A stable partitioned FSI algorithm for incompressible flow and deforming beams

An added-mass partitioned (AMP) algorithm is described for solving fluid-structure interaction (FSI) problems coupling incompressible flows with thin elastic structures undergoing finite deformations. The new AMP scheme is fully second-order accurate and stable, without sub-time-step iterations, even for very light structures when added-mass effects are strong. The fluid, governed by the incompressible Navier-Stokes equations, is solved in velocity-pressure form using a fractional-step method; large deformations are treated with a mixed Eulerian-Lagrangian approach on deforming composite grids. The motion of the thin structure is governed by a generalized Euler-Bernoulli beam model, and these equations are solved in a Lagrangian frame using two approaches, one based on finite differences and the other on finite elements. Special treatment of the AMP condition is required to couple the finite-element beam solver with the finite-difference-based fluid solver, and two coupling approaches are described. A normal-mode stability analysis is performed for a linearized model problem involving a beam separating two fluid domains, and it is shown that the AMP scheme is stable independent of the ratio of the mass of the fluid to that of the structure. A traditional partitioned (TP) scheme using a Dirichlet-Neumann coupling for the same model problem is shown to be unconditionally unstable if the added mass of the fluid is too large. A series of benchmark problems of increasing complexity are considered to illustrate the behavior of the AMP algorithm, and to compare the behavior with that of the TP scheme. The results of all these benchmark problems verify the stability and accuracy of the AMP scheme. Results for one benchmark problem modeling blood flow in a deforming artery are also compared with corresponding results available in the literature.

==> fig/exact.beamPistonRhos0p1.pc.flexiblePartition.ins.order2.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  & N & $p$ & r &  $v_1$ & r & $v_2$ & r & $\uv$ & r & $\grad\cdot\uv$  & r \\ \hline 
   flexiblePartiton1 &     1 & \num{1.3}{-3} &      & \num{6.9}{-6} &      & \num{1.0}{-3} &      & \num{1.0}{-3} &      & \num{3.9}{-5} &       \\ \hline
   flexiblePartiton2 &     2 & \num{5.2}{-5} & 25.0 & \num{2.8}{-7} & 24.7 & \num{7.4}{-6} &134.8 & \num{7.4}{-6} &134.8 & \num{1.9}{-6} & 20.6  \\ \hline
   flexiblePartiton4 &     4 & \num{3.8}{-6} & 13.9 & \num{1.9}{-9} &147.9 & \num{8.2}{-9} &903.8 & \num{8.2}{-9} &903.8 & \num{1.9}{-8} & 96.9  \\ \hline
    rate             &       &  $4.22$       &      &  $5.92$       &      &  $8.45$       &      &  $8.45$       &      &  $5.48$       &       \\ \hline
\end{tabular}
\caption{Cgins, beamPiston, ins, exact.beamPistonRhos0p1.pc.flexiblePartition.ins.order2, ts=pc, $t=.5$, $\nu=.05$, dtMax=0.1, aftol=1e-10, axialAxis=2, kp=1, , cfl=0.9, -rhoBeam=0.1 -E=1.e-4 -tension=1.e-2 -thickness=.1 -K0=10 -p0=1 -addedMass=1 -fluidOnTwoSides=1  -ampProjectVelocity=1 -option=beamPiston -sideBC=slipWall, Sat Jan 31 16:07:05 2015}\label{table:exact.beamPistonRhos0p1.pc.flexiblePartition.ins.order2}
\end{center}
\end{table}


==> fig/exact.beamPistonRhos10p0.pc.flexiblePartition.ins.order2.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  & N & $p$ & r &  $v_1$ & r & $v_2$ & r & $\uv$ & r & $\grad\cdot\uv$  & r \\ \hline 
   flexiblePartiton1 &     1 & \num{1.0}{-4} &      & \num{4.9}{-7} &      & \num{4.4}{-5} &      & \num{4.4}{-5} &      & \num{6.4}{-5} &       \\ \hline
   flexiblePartiton2 &     2 & \num{8.5}{-6} & 12.2 & \num{2.8}{-8} & 17.6 & \num{3.2}{-6} & 13.7 & \num{3.2}{-6} & 13.7 & \num{2.3}{-6} & 27.7  \\ \hline
   flexiblePartiton4 &     4 & \num{6.1}{-7} & 13.8 & \num{1.1}{-9} & 26.1 & \num{2.2}{-7} & 14.4 & \num{2.2}{-7} & 14.4 & \num{7.5}{-8} & 30.5  \\ \hline
    rate             &       &  $3.70$       &      &  $4.42$       &      &  $3.81$       &      &  $3.81$       &      &  $4.86$       &       \\ \hline
\end{tabular}
\caption{Cgins, beamPiston, ins, exact.beamPistonRhos10p0.pc.flexiblePartition.ins.order2, ts=pc, $t=.5$, $\nu=.05$, dtMax=0.1, aftol=1e-10, axialAxis=2, kp=1, , cfl=0.9, -rhoBeam=10.0 -E=1.e-4 -tension=1.e-2 -thickness=.1 -K0=10 -p0=1 -addedMass=1 -fluidOnTwoSides=1  -ampProjectVelocity=1 -option=beamPiston -sideBC=slipWall, Sat Jan 31 16:04:51 2015}\label{table:exact.beamPistonRhos10p0.pc.flexiblePartition.ins.order2}
\end{center}
\end{table}


==> flexibleChannel/exact.beamPistonRhos0p1.pc.flexiblePartition.ins.order2.vector.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid &     N &    $p$   & r & $\vv$ & r & $\grad\cdot\uv$ & r &      $\eta$ & r &    $\eta_t$ & r \\ \hline 
  flexiblePartition1 &     1 & \num{1.5}{-4} &      & \num{1.1}{-3} &      & \num{9.0}{-4} &      & \num{2.9}{-5} &      & \num{1.1}{-3} &       \\ \hline
  flexiblePartition2 &     2 & \num{1.6}{-5} &  9.6 & \num{4.1}{-5} & 26.9 & \num{1.2}{-4} &  7.2 & \num{3.1}{-6} &  9.4 & \num{5.3}{-5} & 21.4  \\ \hline
  flexiblePartition4 &     4 & \num{5.2}{-7} & 30.7 & \num{2.1}{-6} & 19.7 & \num{3.8}{-6} & 32.6 & \num{8.7}{-8} & 36.2 & \num{2.2}{-6} & 24.4  \\ \hline
  flexiblePartition8 &     8 & \num{8.2}{-9} & 62.8 & \num{1.2}{-7} & 16.6 & \num{5.2}{-8} & 73.0 & \num{1.0}{-9} & 83.5 & \num{1.3}{-7} & 17.1  \\ \hline
    rate             &       &  $4.75$       &      &  $4.36$       &      &  $4.72$       &      &  $4.95$       &      &  $4.40$       &       \\ \hline
\end{tabular}
\caption{Cgins, beamPiston, ins, exact.beamPistonRhos0p1.pc.flexiblePartition.ins.order2.vector, ts=pc, $t=1.$, $\nu=.02$, dtMax=0.1, aftol=1e-10, axialAxis=2, kp=1, , cfl=0.9, -rhoBeam=0.1 -E=1.e-4 -tension=1.e-2 -thickness=.1 -K0=10 -p0=1 -addedMass=1 -fluidOnTwoSides=1  -ampProjectVelocity=1 -projectNormalComponent=1 -nis=16 -option=beamPiston -sideBC=slipWall, Thu Jun 11 20:55:53 2015}\label{table:exact.beamPistonRhos0p1.pc.flexiblePartition.ins.order2.vector}
\end{center}
\end{table}


==> flexibleChannel/exact.beamPistonRhos100p0.pc.flexiblePartition.ins.order2.vector.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid &     N &    $p$   & r & $\vv$ & r & $\grad\cdot\uv$ & r &      $\eta$ & r &    $\eta_t$ & r \\ \hline 
  flexiblePartition1 &     1 & \num{5.5}{-6} &      & \num{1.2}{-5} &      & \num{1.0}{-5} &      & \num{7.9}{-6} &      & \num{9.6}{-6} &       \\ \hline
  flexiblePartition2 &     2 & \num{6.7}{-7} &  8.3 & \num{1.2}{-6} & 10.2 & \num{8.2}{-7} & 12.5 & \num{8.8}{-7} &  9.0 & \num{1.1}{-6} &  8.9  \\ \hline
  flexiblePartition4 &     4 & \num{6.2}{-8} & 10.8 & \num{1.1}{-7} & 10.5 & \num{4.9}{-8} & 16.7 & \num{8.8}{-8} & 10.0 & \num{1.1}{-7} & 10.0  \\ \hline
  flexiblePartition8 &     8 & \num{4.0}{-9} & 15.2 & \num{7.5}{-9} & 14.6 & \num{1.8}{-9} & 28.0 & \num{6.1}{-9} & 14.4 & \num{7.5}{-9} & 14.5  \\ \hline
    rate             &       &  $3.47$       &      &  $3.52$       &      &  $4.16$       &      &  $3.43$       &      &  $3.43$       &       \\ \hline
\end{tabular}
\caption{Cgins, beamPiston, ins, exact.beamPistonRhos100p0.pc.flexiblePartition.ins.order2.vector, ts=pc, $t=.7$, $\nu=.02$, dtMax=0.1, aftol=1e-10, axialAxis=2, kp=1, , cfl=0.9, -rhoBeam=100.0 -E=1.e-3 -tension=1.e-1 -thickness=.1 -K0=10 -p0=1 -addedMass=1 -fluidOnTwoSides=1  -ampProjectVelocity=1 -projectNormalComponent=1 -nis=4 -option=beamPiston -sideBC=slipWall -cfls=1., Thu Jun 18 15:26:22 2015}\label{table:exact.beamPistonRhos100p0.pc.flexiblePartition.ins.order2.vector}
\end{center}
\end{table}


==> flexibleChannel/exact.beamPistonRhosp1.pc.flexiblePartition.ins.order2.vector.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid &     N &    $p$   & r & $\vv$ & r & $\grad\cdot\uv$ & r &      $\eta$ & r &    $\eta_t$ & r \\ \hline 
  flexiblePartition1 &     1 & \num{3.1}{-4} &      & \num{1.7}{-4} &      & \num{4.2}{-5} &      & \num{4.8}{-5} &      & \num{9.1}{-5} &       \\ \hline
  flexiblePartition2 &     2 & \num{1.3}{-5} & 22.8 & \num{5.1}{-6} & 34.1 & \num{8.4}{-7} & 49.7 & \num{2.1}{-6} & 22.8 & \num{4.8}{-6} & 19.0  \\ \hline
  flexiblePartition4 &     4 & \num{9.2}{-7} & 14.6 & \num{3.3}{-7} & 15.3 & \num{2.7}{-8} & 30.8 & \num{1.4}{-7} & 14.6 & \num{3.3}{-7} & 14.5  \\ \hline
  flexiblePartition8 &     8 & \num{5.8}{-8} & 15.9 & \num{2.1}{-8} & 16.1 & \num{1.3}{-9} & 20.6 & \num{8.9}{-9} & 16.0 & \num{2.1}{-8} & 15.9  \\ \hline
    rate             &       &  $4.10$       &      &  $4.30$       &      &  $4.98$       &      &  $4.10$       &      &  $4.02$       &       \\ \hline
\end{tabular}
\caption{Cgins, beamPiston, ins, exact.beamPistonRhosp1.pc.flexiblePartition.ins.order2.vector, ts=pc, $t=.7$, $\nu=.02$, dtMax=0.1, aftol=1e-10, axialAxis=2, kp=1, , cfl=0.9, -rhoBeam=.1 -E=1.e-3 -tension=1.e-1 -thickness=.1 -K0=10 -p0=1 -addedMass=1 -fluidOnTwoSides=1  -ampProjectVelocity=1 -projectNormalComponent=1 -nis=4 -option=beamPiston -sideBC=slipWall -cfls=2., Thu Jun 18 15:08:39 2015}\label{table:exact.beamPistonRhosp1.pc.flexiblePartition.ins.order2.vector}
\end{center}
\end{table}


==> texFiles/algorithm-5-5-15.tex <==
\section{Added-Mass Partitioning} \label{sec:AMPalgorithm}

\textcolor{red}{[This lead paragraph may be repeating ideas from the Introduction.  Want to return to this at a later time.]}
In the traditional approach to partitioned fluid-structure interaction, the kinematic condition~\eqref{eq:kinematicII}
is satisfied by imposing the motion of the solid as an interface condition on the fluid. This inherently
one-sided approach is one root cause leading to added-mass instabilities for partitioned fluid-structure
interaction. Various avenues to
more symmetric imposition of~\eqref{eq:kinematicII} have been taken with various degrees of
success. Here we pursue the Added Mass Partitioned (AMP) approach to coupling. 
The core AMP algorithm for coupling a linear incompressible fluid with a thin shell or beam
was described in~\cite{fis2014}. In that work a simplified model was considered where 
linearized equations of motion were used to describe infinitesimal amplitude perturbations
from the specific geometry of fluid in a box with a beam on one of the faces of the box.
This manuscript considers the more general case of the nonlinear Navier-Stokes equations
with finite amplitude deformations applied to more general geometries. 
% (although we continue to use a beam model only valid for small amplitude deformations)
For example, we consider the case of a beam with fluid on two sides and the case of a beam
with a free end immersed in a fluid.
% can be immersed within the fluid. 
%The AMP interface conditions for this more general situation are derived below. 
%The primary 
%difference for beams with fluid on two sides is that the Robin interface condition for the pressure
%now involves the pressure at opposite sides of the beam. 
% are basically the same as those given in~\cite{fis2014}. 
%  with a few minor differences. 
%
% The kinematic interface condition~\eqref{eq:kinematic} can be written using the EB approximation to
% relate the velocity of the fluid and the velocity of the beam by 
% \begin{align}
%     \vv(\xsv_\pm(\ss,t),t) &= \frac{\partial}{\partial t}\xsv_{\pm}(\ss,t) 
%                               = \vsv(\ss,t) \pm (\hs/2) \partialt\nsv(\ss,t) , \nonumber  \\
%                           &= \vsv(\ss,t) \pm \wsv,   \label{eq:velocityInterface}
% \end{align} 
% where we have defined $\wsv \equiv (\hs/2) \partialt\nsv(\ss,t)$. 
%

\subsection{Continuous AMP Interface Condition}
The AMP interface condition can be derived at a continuous level by first 
taking the time derivative of the kinematic interface condition~\eqref{eq:kinematicII} and using
the definition of the velocity on the surface of the beam~\eqref{eq:beamSurfaceVelocity} to give
\begin{align}
  \frac{D}{Dt}\vv(\xsv_\pm(\sv,t),t)  & = \partialt \vsv(\sv,t) + \partialt\wsv_\pm(\sv,t)  \nonumber\\
     & = \frac{\partial^2 \uvs}{\partial t^2}(\sv,t) + \partialt\wsv_\pm(\sv,t), \label{eq:interfaceAcceleration}
\end{align}
where $D/Dt$ is the material derivative.
%From~\eqref{eq:interfaceAcceleration}, it follows that acceleration of the beam is 
%\begin{align}
%    \frac{\partial^2 \uvs}{\partial t^2} = \partialt \vsv(\ss,t) = \frac{D}{Dt}\vv(\xsv_\pm(\ss,t),t) - \partialt\wsv_\pm . \label{eq:beamAccel}
%\end{align}
% Solving for $\partial_t \vsv(\ss,t)$ from ~\eqref{eq:interfaceAcceleration} and sub
% Replacing $\partial^2\usv/\partial^2 t$ in the beam equation~\eqref{eq:beamEquation} with the expression for
% Substituting~\eqref{eq:interfaceAcceleration} into the beam equation~\eqref{eq:beamEquation} gives the following
% interface condition on the fluid, 
The fluid acceleration, $D\vv/Dt$, is given by the fluid momentum equation~\eqref{eq:fluidMomentum},
while the acceleration of the structure, $\partial^2 \uvs / \partial t^2$, is given by the beam equation~\eqref{eq:beamEquation}. Substituting
these definitions into~\eqref{eq:interfaceAcceleration} gives 
\begin{equation}
  \frac{\rhos\As}{\rho}\grad\cdot\sigmav(\xsv_\pm(\sv,t),t)  = \Lsv\bigl(\uvs,\vsv\bigr) + \rhos\As \partialt \wsv_\pm(\sv,t)  + \fsv(\sv,t),
          \qquad \sv\in\OmegaSbar.
    \label{eq:AMPconditionSigma}
\end{equation}
%
%Substituting~\eqref{eq:beamAccel} into the beam equation~\eqref{eq:beamEquation} results in the following relation,
%\begin{align}
%&  \rhos\As \frac{D}{Dt}\vv(\xsv_\pm(\ss,t),t)  = \Lsv(\usv,\vsv)  
%                 + \rhos\As \partialt \wsv_\pm(\ss,t)  + \fsv(\ss,t) ,    \qquad \ss\in\Gammas.  \label{eq:AMPcondition}
%\end{align}
%Using the fluid momentum equation~\eqref{eq:fluidMomentum} to replace $D\vv/Dt$ in~\eqref{eq:AMPcondition} gives
%\begin{equation}
%  \frac{\rhos\As}{\rho}\grad\cdot\sigmav(\xsv_\pm(\ss,t),t)  = \Lsv\bigl(\uvs,\vsv\bigr) + \rhos\As \partialt \wsv_\pm(\ss,t)  + \fsv(\ss,t),
%          \qquad \ss\in\Gammas.
%    \label{eq:AMPconditionSigma}
%\end{equation}
Finally, using~\eqref{eq:dynamic} for the force $\fsv$ yields the continuous AMP interface condition 
\begin{equation}
    (\sigmav\nv)_+(\sv,t) + (\sigmav\nv)_-(\sv,t) + 
\frac{\rhos\As}{\rho}\grad\cdot\sigmav(\xsv_\pm(\sv,t),t)  
         = \Lsv\bigl(\uvs,\vsv\bigr) + \rhos\As \partialt \wsv_\pm(\sv,t) , \qquad \sv\in\OmegaSbar,
    \label{eq:AMP_ContinuousConditions}
\end{equation}
which can be interpreted as a mixed Robin condition along the upper and lower surfaces of the beam coupling the behaviors of the fluid and structure.

\subsection{Partitioned Schemes Using the AMP Condition}
Following the approach used in~\cite{fis2014}, we employ the AMP interface condition in~\eqref{eq:AMP_ContinuousConditions} as a stable condition for a {\em partitioned} scheme coupling incompressible fluids and thin structural beams.  Assuming that {\em predicted} values
for the solid variables $\usv^{(p)}$, $\vsv^{(p)}$ and $\wsv^{(p)}_\pm$ are obtained in a first step of the partitioned scheme and used to evaluate the right-hand side of~\eqref{eq:AMP_ContinuousConditions}, the interface condition then becomes a mixed Robin condition for the fluid in a subsequent step of the scheme.  This is the primary AMP interface condition:
% ---------------------------------------------------------------------------------------------------------------
\begin{condition}
The AMP interface condition for the fluid is 
\begin{equation}
    (\sigmav\nv)_+(\sv,t) + (\sigmav\nv)_-(\sv,t) + 
\frac{\rhos\As}{\rho}\grad\cdot\sigmav(\xsv_\pm(\sv,t),t)  
         = \Lsv\bigl(\uvs^{(p)},\vsv^{(p)}\bigr) + \rhos\As \partialt \wsv^{(p)}_\pm(\sv,t) , \qquad \sv\in\OmegaSbar,
    \label{eq:AMP_CombinedConditions}
\end{equation}
where $\usv^{(p)}$, $\vsv^{(p)}$ and $\wsv^{(p)}_\pm$ are predicted solid variables.
For a beam with fluid on only one side the condition is
\begin{equation}
    \sigmav\nv(\sv,t) + 
\frac{\rhos\As}{\rho}\grad\cdot\sigmav(\xsv(\sv,t),t)
         = \Lsv\bigl(\uvs^{(p)},\vsv^{(p)}\bigr) + \rhos\As \partialt \wsv^{(p)}(\sv,t) , \qquad \sv\in\OmegaSbar,
    \label{eq:AMP_CombinedConditionsOneSide}
\end{equation}
% This is used with partitioned FSI schemes by using predicted values for the beam operators that appear on the 
% right-hand-side of~\eqref{eq:AMP_CombinedConditions}.
\end{condition}
% ---------------------------------------------------------------------------------------------------------------
% When the beam has fluid on two sides, the two 
% conditions ($\pm$) in~\eqref{eq:AMP_CombinedConditions} are generalized Robin interface conditions that
% involve the fluid traction at points
% on opposite sides of the beam. For a beam with fluid on only one side, there will be only one condition applied,
% with the traction term on the opposite side set to zero, or some specified value. 

The essential philosophy in this approach is to embed the local behavior of solutions of the FSI problem
to define the interface dynamics.
Therefore, in a partitioned scheme the solid would be advanced first to a new time step, providing the predicted
values used in the interface conditions~\eqref{eq:AMP_CombinedConditions} or~\eqref{eq:AMP_CombinedConditionsOneSide}
for the subsequent fluid solve. This process can be viewed as 
computing the solution of a generalized fluid-solid Riemann problem at the interface, thus extending the approach used in the AMP
scheme for elastic solids coupled to inviscid compressible fluids discussed in~\cite{BanksSjogreen2011,fsi2012,flunsi2014r}.
In these previous studies, the FSI problems were purely hyperbolic and the fluid-solid Riemann problem involved local, piecewise constant states of the fluid and solid on either side of the interface.  The solution was then computed using the method of characteristics, giving interface values that are impedance-weighted averages of the fluid and solid states. 
In the present case involving an incompressible fluid, the initial states 
for the solid domain are $\usv^{(p)}$, $\vsv^{(p)}$ and $\wsv^{(p)}_\pm$, while the solution of the generalized
fluid-solid Riemann problem requires the solution of an elliptic problem in the entire fluid domain with~\eqref{eq:AMP_CombinedConditions} or~\eqref{eq:AMP_CombinedConditionsOneSide} providing the appropriate condition along the interface.





%  (there are two equations, one applied onat a point on the lower surface and one on the corresponding point on the upper surface). 

%- Noting that $\sigmav\nv_\pm = -p(\xsv_+(\ss,t),t)\nv_\pm + \tauv\nv_\pm$ 
%- leads to the AMP condition written in terms of the fluid pressure.  *CHECK ME*
%- % ---------------------------------------------------------------------------------------------------------------
%- \begin{condition}
%- The AMP interface condition for the fluid written in terms of the pressure is 
%- \begin{equation}
%-    -(p\nv)_+ +  (p\nv)_-  -  
%- \frac{\rhos\As}{\rho} \grad p(\xsv_\pm(\ss,t),t)  
%-          = \Lsv\bigl(\uvs^{(p)},\vsv^{(p)}\bigr) + \rhos\As \partialt \wsv^{(p)}_\pm(\ss,t) - (\tauv\nv)_+ - (\tauv\nv)_- , \qquad \ss\in\Gammas.
%-     \label{eq:AMP_CombinedConditionsPressure}
%- \end{equation}
%- % This is used with partitioned FSI schemes by using predicted values for the beam operators that appear on the 
%- % right-hand-side of~\eqref{eq:AMP_CombinedConditionsPressure}.
%- % and with fractional-step fluid solvers by
%- % using predicted values for the fluid stress terms that appear on the 
%- % right-hand-side of~\eqref{eq:AMP_CombinedConditionsPressure}.
%- \end{condition}
%- % ---------------------------------------------------------------------------------------------------------------
%- 

If a fractional-step scheme is used to integrate the fluid equations, then suitable boundary conditions can be derived by
decomposing~\eqref{eq:AMP_CombinedConditions} or~\eqref{eq:AMP_CombinedConditionsOneSide} into normal and tangential components.  The normal component gives a boundary condition for the pressure, while the tangential components, along with the continuity equation~\eqref{eq:fluidDiv3d}, provide boundary conditions for the velocity. 
% ---------------------------------------------------------------------------------------------------------------
\begin{condition}
The AMP interface conditions for the pressure equation~\eqref{eq:fluidPressure} are given by
\begin{align}
    p_+ -  p_-  
     +  \frac{\rhos\As}{\rho} \frac{\partial}{\partial n_+}p_+ 
       =  - \nv_+^T\Lsv^{(p)} - \rhos\As \nv_{+}^T \partialt \wsv^{(p)}_\pm
          +   \frac{\mu\rhos\As}{\rho}\nv_{+}^T\Delta \vv
       +   \nv_+^T(\tauv\nv)_+  - \nv_+^T(\tauv\nv)_- \,,  \label{eq:AMPpressureBCI} \\
% 
   - p_+ +   p_-  
     +  \frac{\rhos\As}{\rho} \frac{\partial}{\partial n_-}p_- 
       =  - \nv_-^T\Lsv^{(p)} - \rhos\As \nv_{-}^T \partialt \wsv^{(p)}_\pm
           +   \frac{\mu\rhos\As}{\rho}\nv_{-}^T\Delta \vv
        -  \nv_-^T (\tauv\nv)_+  + \nv_-^T(\tauv\nv)_- \,,  \label{eq:AMPpressureBCII}
\end{align}
or for a beam with fluid on only one side
\begin{align}
    p
     +  \frac{\rhos\As}{\rho} \frac{\partial}{\partial n}p 
       =  - \nv^T\Lsv^{(p)} - \rhos\As \nv^T \partialt \wsv^{(p)}_\pm
       +   \nv^T\tauv\nv,   \label{eq:AMPpressureBCIII}
\end{align}
where $\Lsv^{(p)}\equiv \Lsv\bigl(\uvs^{(p)},\vsv^{(p)}\bigr)$ and for $\sv\in\OmegaSbar$.
\end{condition}

\bigskip
% ---------------------------------------------------------------------------------------------------------------
\begin{condition}
The AMP interface conditions for the velocity when integrating the momentum equation~\eqref{eq:fluidMomentum}
are given by
\begin{align}
  \tanv_{m,+}^T\left[(\tauv\nv)_+ +  (\tauv\nv)_- +   \frac{\mu\rhos\As}{\rho}\Delta \vv\right]
     = \tanv_{m,+}^T\left[\frac{\rhos\As}{\rho}\grad p  
               + \Lsv^{(p)}
        +  \rhos\As \partialt \wsv^{(p)}_+\right]
          , \qquad m=1,2 ,    \label{eq:AMPtangentialVelocityBCI} \\
  \tanv_{m,-}^T\left[(\tauv\nv)_+ +  (\tauv\nv)_- +   \frac{\mu\rhos\As}{\rho}\Delta \vv\right]
     = \tanv_{m,-}^T\left[\frac{\rhos\As}{\rho}\grad p  
               + \Lsv^{(p)}
        +  \rhos\As \partialt \wsv^{(p)}_-\right]
          , \qquad m=1,2 , \label{eq:AMPtangentialVelocityBCII}
\end{align}
%\begin{align}
%  \tanv_{m,+}^T(\tauv\nv)_+ +  \tanv_{m,+}^T(\tauv\nv)_- +   \frac{\mu\rhos\As}{\rho}\tanv_{m,+}^T\Delta \vv
%     = \frac{\rhos\As}{\rho}\tanv_{m,+}^T\grad p  
%               + \tanv_{m,+}^T\Lsv^{(p)}
%        +  \rhos\As \tanv_{m,+}^T \partialt \wsv^{(p)}_+(\ss,t)
%          , \quad m=1,2 ,    \label{eq:AMPtangentialVelocityBCI} \\
%  \tanv_{m,-}^T(\tauv\nv)_+ +  \tanv_{m,-}^T(\tauv\nv)_- +   \frac{\mu\rhos\As}{\rho}\tanv_{m,-}^T\Delta \vv
%     = \frac{\rhos\As}{\rho}\tanv_{m,-}^T\grad p  
%               + \tanv_{m,-}^T\Lsv^{(p)}
%        +  \rhos\As \tanv_{m,-}^T \partialt \wsv^{(p)}_-(\ss,t)
%          , \quad m=1,2 , \label{eq:AMPtangentialVelocityBCII}
%\end{align}
or for a beam with fluid on only one side:
\begin{align}
  \tanv_{m}^T\left[\tauv\nv +  \frac{\mu\rhos\As}{\rho}\Delta \vv\right]
     = \tanv_{m}^T\left[\frac{\rhos\As}{\rho}\grad p  
               + \Lsv^{(p)}
        +  \rhos\As \partialt \wsv^{(p)}\right]
          , \qquad m=1,2 ,    \label{eq:AMPtangentialVelocityBCIII}
\end{align}
%\begin{align}
%  \tanv_{m}^T\tauv\nv +  \frac{\mu\rhos\As}{\rho}\tanv_{m}^T\Delta \vv
%     = \frac{\rhos\As}{\rho}\tanv_{m}^T\grad p  
%               + \tanv_{m}^T\Lsv^{(p)}
%        +  \rhos\As \tanv_{m}^T \partialt \wsv^{(p)}(\ss,t)
%          , \quad m=1,2 ,    \label{eq:AMPtangentialVelocityBCIII}
%\end{align}
where $\tanv_{m,\pm}=\tanv_{m,\pm}(\sv,t)$, $m=1,2$,  denote mutually orthonormal tangent vectors and $\sv\in\OmegaSbar$. %  on $\GammaI_\pm$ (DEFINE $\GammaI_\pm$ ?).
\end{condition}




% Let the fluid normals on the upper and lower surfaces 
% be denoted by $\nv_+=\nv(\xsv_+(\ss,t),t)$ and $\nv_-=\nv(\xsv_-(\ss,t),t)$, respectively.

We note that if the beam model only supports motion in the direction normal to the beam reference surface,
then only~\eqref{eq:AMPpressureBCI}--\eqref{eq:AMPpressureBCIII} are 
valid and~\eqref{eq:AMPtangentialVelocityBCI}--\eqref{eq:AMPtangentialVelocityBCIII} should be replaced with a
standard condition on the tangential velocity. For example, \eqref{eq:AMPtangentialVelocityBCI}--\eqref{eq:AMPtangentialVelocityBCIII}
can be replaced by setting the tangential component of the fluid velocity equal to the
tangential component of the velocity on the beam surface, i.e.~a {\em no-slip} type condition on the tangential velocity,
\begin{equation}
  \tv_\pm^T\vv(\xsv_\pm(\sv,t),t) = \tv_\pm^T\vsv(\sv,t)+\tv_\pm^T\wsv_\pm(\sv,t), \qquad \sv\in\OmegaSbar,
    \label{eq:TangentialVelocityNoSlip}
\end{equation}
or by setting the tangential component of the traction to zero, i.e.~a {\em slip wall} condition,
\begin{equation}
  (\tv^T\tauv\nv)_\pm(\sv,t) = 0 ,\qquad \sv\in\OmegaSbar.
    \label{eq:TangentialVelocitySlip}
\end{equation}

% -------------------------
\subsection{Velocity projection} 
The velocity at the interface in the AMP scheme is defined to be a weighted average of the predicted velocities from
the fluid and solid. 
This averaging can be motivated by noting that 
for heavy beams the motion of the interface is primarily determined from the beam and thus the interface velocity should
be nearly equal to that of the structure.  For very light beams, on the other hand, 
% when $\Lsv$ is also small, 
the fluid interface
approaches a free surface where the motion of the interface is primarily determined by the fluid itself.
The weighted average given in~\cite{fis2014} correctly accounts for these two limits, and this average is extended here
to account for beams of finite thickness and for beams with fluid on two sides.
% Thus in this limit the fluid-beam interface is primarily determined by the fluid
%Note that the velocity projection given here extends the one given in~\cite{fis2014}
%by considering beams of finite thickness and beams with fluid on two sides.
 

% The algorithm for projecting the interface velocities is as follows.
\textcolor{red}{I would like to discuss this.  It confused me in several places.}
\begin{algorithmVP}\small
~

% Velocity projection algorithm.
\begin{enumerate}
   \item Compute the projected surface velocities $\vv_\pm^I$ on the beam as a weighted average of the predicted
        fluid surface velocities $\vv_\pm$ and beam surface velocities $\vsv_\pm$,
\begin{align}
    \vv_\pm^I = \gamma \vv_\pm + (1-\gamma) \vsv_\pm ,  \qquad  \gamma=\frac{1}{1 + (\rhos\As)/(\rho \Af)},\label{eq:velocityProjection}
\end{align}
   Note that the algorithm appears to be insensitive to the choice of $\Af$ and we pick $\Af=??$.  \textcolor{red}{I'm confused here.  In 2D I would think that $\rhos\As$ is the mass per unit length per unit breadth of the beam and in 3D it is a mass per unit area.  (Ultimately, a mass per unit area in either case and so $\As$ has units of length.)  So, $\rho\Af$ should also have units of mass per unit area, and thus $\Af$ has units of length as well.  In FIS we used $h_f$ here and were similarly vague on its definition.  Can we say something more???}
   \item Transfer the interface velocities $\vv_\pm^I$ onto the beam reference surface.  \textcolor{red}{Can we give more details on how this is done?} 
         % using the algorithm  described in Section~\ref{sec:beamSolverNumerical}. CHECK ME
   \item Redefine the beam reference-surface velocity $\vsv(s,t)$ to be the velocity obtained from step 2, 
           or a density weighted average of the two velocities from step 2 when the beam has fluid on two sides.
   \item For beams with fluid on two sides we ensure that fluid velocities on opposite sides of the beam remain consistent with a single
       beam reference-surface velocity. Thus the fluid surface velocities $\vv_\pm$ 
       on the two beam surfaces is recomputed using~\eqref{eq:beamSurfaceVelocity}
       and the beam reference-surface velocity from step 3.
\end{enumerate}
\end{algorithmVP}

From the perspective of numerical stability, this velocity projection appears to be needed only when the 
beam is quite {\em light}. Otherwise the fluid velocity on the interface could be taken as the velocity of the beam.
This observation is supported by a linear stability analysis as well as numerical experiments. However, in practice we
find that the velocity projection is never harmful and we therefore advocate its use. In addition, for very light beams the
interface acts as a free surface with no surface tension (assuming $\Lsv$ is also very small). 
In this case, the fluid interface velocity is smoothed using a few steps of a fourth-order filter
to remove oscillations that can be excited on the interface, see Section~\ref{sec:velocityFilter} for
more details. Finally note that for cases where the beam supports motion only in the normal direction to the beam, only the 
normal component of the fluid velocity is projected, 
\begin{align}
   (\nv^T\vv)_\pm^I = \gamma (\nv^T\vv)_\pm + (1-\gamma) (\nv^T\vsv)_\pm  .  \label{eq:velocityProjectionNormalComponent}
\end{align}

%\medskip
%\noindent{Notes.}
%\begin{enumerate}
%  \item The weighting parameter $\gamma$ is taken to be 
%\begin{align*}
%    \gamma = \frac{1}{1 + (\rhos\As)/(\rho \Af)}.
%\end{align*}
%where $\Af$ is a measure of the volume of the fluid domain. The algorithm appears to be quite insensitive to the
%choice of $\Af$. 
%% 
%\item Step 4 will
%       ensure that the fluid velocities on opposite sides on the beam will remain consistent with a single
%       beam reference-line velocity.
%%
% \item The velocity projection appears to be generally only needed when the beam is quite {\em light}. 
%Otherwise the fluid velocity on the interface can be taken from the velocity of the beam.
%%
%  \item For very light beams the
%interface acts a free surface with no surface tension (assuming $\Lsv$ is also very small). 
%In this case, the fluid interface velocity is smoothed with a few steps of a fourth-order filter
%to remove oscillations that can be excited on the interface, see Section~\ref{sec:velocityFilter} for
%more details.
%% 
% \item For beams with fluid on two-sides, and where the fluid densities are different 
%on the two sides it may be appropriate to use a fluid density weighted average in step 3. We have not as yet evaluated
%this situation. 
%% 
%\item  For the case when the beam only supports motion in the normal direction to the beam, only the 
%normal component of the velocity is projected, 
%\begin{align}
%   (\nv^T\vv)_\pm^I = \gamma (\nv^T\vv)_\pm + (1-\gamma) (\nv^T\vsv)_\pm  .  \label{eq:velocityProjectionNormalComponent}
%\end{align}
%\end{enumerate}

% 
% Following~\cite{fis2014}, the interface velocity $\vv^I$ is defined to be a weighted average of the predicted velocities from
% the fluid and solid. For example, if the fluid velocity on a point on the top or bottom surface $\xsv_\pm$ is $\vv_\pm$
% then we take the interface velocity to be 
% \begin{align}
%     \vv_\pm^I = \gamma \vv_\pm + (1-\gamma) \vsv_\pm   \label{eq:velocityProjection}
% \end{align}
% where from~\eqref{eq:kinematicII}, $\vsv_\pm$ is the velocity of a point on the surface of the beam
% \begin{align*}
%   \vsv_\pm = \vsv(s,t) \pm \wsv_\pm(s,t)
% \end{align*}
% and where
% \begin{align*}
%     \gamma = \frac{1}{1 + (\rhos\As)/(\rho h_f)}.
% \end{align*}
% The parameter $h_f$  is ... FINISH ME. 
% Equation~\eqref{eq:velocityProjection} defines the projected velocity on the surface(s) of the beam. 
% Given values on the beam surface(s) we need to determine a projected beam velocity $\vsv(s,t)$ on the beam reference-line. 
% Note that velocity values on the beam surface correspond to velocity values on the beam reference line according
% to the transformation~\eqref{eq:kinematicII}, 
% Therefore we transfer the surface velocities to the beam reference line
% using~\eqref{eq:kinematicII} to determine the projected beam velocity. For a beam with fluid on two surfaces, we
% take some average value of the two projected velocities (THIS COULD CHANGE if the fluid densities on the two
% sides are not the same). 
% 
% 
% Note that for the case when the beam only supports motion in the normal direction to the beam we only project the
% normal component of the velocity,
% \begin{align}
%    (\nv^T\vv)_\pm^I = \gamma (\nv^T\vv)_\pm + (1-\gamma) (\nv^T\vsv)_\pm   \label{eq:velocityProjectionNormalComponent}
% \end{align}



% 
% Since beam model may have it's own discretization and degrees of freedom it is not straightfoward to 
% adjust the beam velocity on the reference-line to match the values of $\vv^I$ on the beam surfaces. 
% For ease of implementation we thus
% use a relaxation procedure to force the beam reference-line velocity $\vsv$ to approximately match the
% interface velocities $\vv_\pm^I$. We do this by adding an extra relaxation term proportional to the beam velocity 
% to the right-hand side
% of the beam equation~\eqref{eq:beamEquation}
% \begin{alignat}{3}
%      - K_I \vsv
% %   \rhos \As \frac{\partial^2 \uvs}{\partial t^2} =& \Lvs(\uvs,\vvs) +\fsv(s,t), \quad && \ss\in[0,\ls], \quad t\ge 0,
% \end{alignat}
% and adjust the fluid force on the beam surfaces to be 
% \begin{alignat}{3}
%    \sigmav\nv \rightarrow \sigmav\nv + K_I \vv_\pm^I 
% \end{alignat}
% Roughly speaking, this will add a term of the form $-K_I ( \vsv - \vv^I)$ to the beam equation. 
% When $K_I/(\rhos\As)$ is large this will cause the beam velocity to be consistent with the chosen interface velocities.
% When the beam is {\em heavy} this term should have little affect since $K_I/(\rhos\As)$ will be small
% and also since the interface velocity will be primarily determined by the beam velocity, $\vsv \approx \vv^I$,
% from the velocity projection~\eqref{eq:velocityProjection}.


==> texFiles/algorithm-orig.tex <==
\section{Added-Mass Partitioning} \label{sec:AMPalgorithm}

In the traditional approach to partitioned fluid-structure interaction, the kinematic condition~\eqref{eq:kinematicII}
is satisfied by imposing the motion of the solid as an interface condition on the fluid. This inherently
one-sided approach is one root cause leading to added-mass instabilities for partitioned fluid-structure
interaction. Various avenues to
more symmetric imposition of~\eqref{eq:kinematicII} have been taken with various degrees of
success. Here we pursue the Added Mass Partitioned (AMP) approach to coupling. 
The core AMP algorithm for coupling a linear incompressible fluid with a thin shell or beam
was described in~\cite{fis2014}. In that work a simplified model was considered where 
linearized equations of motion were used to describe infinitesimal amplitude perturbations
from the specific geometry of fluid in a box with a beam on one of the faces of the box.
This manuscript considers the more general case of the nonlinear Navier-Stokes equations
with finite amplitude deformations applied to more general geometries. 
% (although we continue to use a beam model only valid for small amplitude deformations)
For example, we consider the case of a beam with fluid on two sides and the case of a beam
with a free end immersed in a fluid.
% can be immersed within the fluid. 
%The AMP interface conditions for this more general situation are derived below. 
%The primary 
%difference for beams with fluid on two sides is that the Robin interface condition for the pressure
%now involves the pressure at opposite sides of the beam. 
% are basically the same as those given in~\cite{fis2014}. 
%  with a few minor differences. 
%
% The kinematic interface condition~\eqref{eq:kinematic} can be written using the EB approximation to
% relate the velocity of the fluid and the velocity of the beam by 
% \begin{align}
%     \vv(\xsv_\pm(\ss,t),t) &= \frac{\partial}{\partial t}\xsv_{\pm}(\ss,t) 
%                               = \vsv(\ss,t) \pm (\hs/2) \partialt\nsv(\ss,t) , \nonumber  \\
%                           &= \vsv(\ss,t) \pm \wsv,   \label{eq:velocityInterface}
% \end{align} 
% where we have defined $\wsv \equiv (\hs/2) \partialt\nsv(\ss,t)$. 
%

\subsection{Continuous AMP Interface Condition}
The AMP interface condition can be derived at a continuous level by first 
taking the time derivative of the kinematic interface condition~\eqref{eq:kinematicII} and using
the definition of the velocity on the surface of the beam~\eqref{eq:beamSurfaceVelocity} to give
\begin{align}
  \frac{D}{Dt}\vv(\xsv_\pm(\ss,t),t)  & = \partialt \vsv(\ss,t) + \partialt\wsv_\pm  \nonumber\\
     & = \frac{\partial^2 \uvs}{\partial t^2} + \partialt\wsv_\pm, \label{eq:interfaceAcceleration}
\end{align}
where $D/Dt$ is the total time derivative (i.e. $\frac{D\vv}{Dt} = \vv_t + (\vv\cdot\grad)\vv$).
%From~\eqref{eq:interfaceAcceleration}, it follows that acceleration of the beam is 
%\begin{align}
%    \frac{\partial^2 \uvs}{\partial t^2} = \partialt \vsv(\ss,t) = \frac{D}{Dt}\vv(\xsv_\pm(\ss,t),t) - \partialt\wsv_\pm . \label{eq:beamAccel}
%\end{align}
% Solving for $\partial_t \vsv(\ss,t)$ from ~\eqref{eq:interfaceAcceleration} and sub
% Replacing $\partial^2\usv/\partial^2 t$ in the beam equation~\eqref{eq:beamEquation} with the expression for
% Substituting~\eqref{eq:interfaceAcceleration} into the beam equation~\eqref{eq:beamEquation} gives the following
% interface condition on the fluid, 
The fluid acceleration, $D\vv/Dt$, is given from the fluid momentum equation~\eqref{eq:fluidMomentum},
while the acceleration of the beam, $\partial^2 \uvs / \partial t^2$,  is given by equation~\eqref{eq:beamEquation}. Substituting
these definitions into~\eqref{eq:interfaceAcceleration} gives 
\begin{equation}
  \frac{\rhos\As}{\rho}\grad\cdot\sigmav(\xsv_\pm(\ss,t),t)  = \Lsv\bigl(\uvs,\vsv\bigr) + \rhos\As \partialt \wsv_\pm(\ss,t)  + \fsv(\ss,t),
          \qquad \ss\in\Gammas.
    \label{eq:AMPconditionSigma}
\end{equation}
%
%Substituting~\eqref{eq:beamAccel} into the beam equation~\eqref{eq:beamEquation} results in the following relation,
%\begin{align}
%&  \rhos\As \frac{D}{Dt}\vv(\xsv_\pm(\ss,t),t)  = \Lsv(\usv,\vsv)  
%                 + \rhos\As \partialt \wsv_\pm(\ss,t)  + \fsv(\ss,t) ,    \qquad \ss\in\Gammas.  \label{eq:AMPcondition}
%\end{align}
%Using the fluid momentum equation~\eqref{eq:fluidMomentum} to replace $D\vv/Dt$ in~\eqref{eq:AMPcondition} gives
%\begin{equation}
%  \frac{\rhos\As}{\rho}\grad\cdot\sigmav(\xsv_\pm(\ss,t),t)  = \Lsv\bigl(\uvs,\vsv\bigr) + \rhos\As \partialt \wsv_\pm(\ss,t)  + \fsv(\ss,t),
%          \qquad \ss\in\Gammas.
%    \label{eq:AMPconditionSigma}
%\end{equation}
Finally, substituting the expression~\eqref{eq:dynamic} for the force $\fsv$ yields the continuous AMP interface condition 
\begin{equation}
    (\sigmav\nv)_+ + (\sigmav\nv)_- + 
\frac{\rhos\As}{\rho}\grad\cdot\sigmav(\xsv_\pm(\ss,t),t)  
         = \Lsv\bigl(\uvs,\vsv\bigr) + \rhos\As \partialt \wsv_\pm(\ss,t) , \qquad \ss\in\Gammas,
    \label{eq:AMP_ContinuousConditions}
\end{equation}
which can be interpreted as a mixed condition along the interface separating the fluid and beam.

\subsection{Partitioned Solvers Using the AMP Condition}
Equation~\eqref{eq:AMP_ContinuousConditions} appears to be a condition that couples
fluid and solid values on the interface. However, a critical observation made in~\cite{fis2014} is
that~\eqref{eq:AMP_ContinuousConditions}
can be used as a stable condition for {\em partitioned} schemes by using {\em predicted} values
for the solid variables $\usv^{(p)}$, $\vsv^{(p)}$ and $\wsv^{(p)}$ when evaluating the right-hand-side 
of~\eqref{eq:AMP_ContinuousConditions}.  
% Note that the fluid traction terms on the left-hand side of~\eqref{eq:AMP_ContinuousConditions}, which orginally appeared in the beam equations, 
% 
This leads to the primary AMP interface condition:
% ---------------------------------------------------------------------------------------------------------------
\begin{condition}
The AMP interface condition for the fluid is 
\begin{equation}
    (\sigmav\nv)_+ + (\sigmav\nv)_- + 
\frac{\rhos\As}{\rho}\grad\cdot\sigmav(\xsv_\pm(\ss,t),t)  
         = \Lsv\bigl(\uvs^{(p)},\vsv^{(p)}\bigr) + \rhos\As \partialt \wsv^{(p)}_\pm(\ss,t) , \qquad \ss\in\Gammas,
    \label{eq:AMP_CombinedConditions}
\end{equation}
where $\usv^{(p)}$, $\vsv^{(p)}$ and $\wsv^{(p)}$ are predicted solid values.
For a beam with fluid on only one side the condition is
\begin{equation}
    \sigmav\nv + 
\frac{\rhos\As}{\rho}\grad\cdot\sigmav
         = \Lsv\bigl(\uvs^{(p)},\vsv^{(p)}\bigr) + \rhos\As \partialt \wsv^{(p)}(\ss,t) , \qquad \xv\in\Gamma, ~~\ss\in\Gammas,
    \label{eq:AMP_CombinedConditionsOneSide}
\end{equation}
% This is used with partitioned FSI schemes by using predicted values for the beam operators that appear on the 
% right-hand-side of~\eqref{eq:AMP_CombinedConditions}.
\end{condition}
% ---------------------------------------------------------------------------------------------------------------
% When the beam has fluid on two sides, the two 
% conditions ($\pm$) in~\eqref{eq:AMP_CombinedConditions} are generalized Robin interface conditions that
% involve the fluid traction at points
% on opposite sides of the beam. For a beam with fluid on only one side, there will be only one condition applied,
% with the traction term on the opposite side set to zero, or some specified value. 

The essential philosophy in this approach is to embed the local behavior of solutions to the fluid-solid system
to define the interface dynamics.
Therefore, in a partitioned scheme the solid would first be advanced to the new time step, providing the predicted
values used in the interface conditions~\eqref{eq:AMP_CombinedConditions} 
that are used when solving for the fluid values. This process can be viewed as 
computing the solution to a generalized Riemann problem at the interface and generalizes the AMP
scheme for compressible fluids and compressible solids~\cite{BanksSjogreen2011,fsi2012}.
In that case the FSI problem was purely hyperbolic and 
the Riemann problem had piecewise constant initial conditions. The solution is then computed
using characteristics, giving interface values that are impedance weighted averages of the fluid and solid states. 
In the present case the initial conditions for the Riemann problem 
for the solid domain are $\usv^{(p)}$, $\vsv^{(p)}$. %In the fluid domain the velocity can also be predicted when 
%using a fractional step scheme. 
The solution to the Riemann problem then requires the solution of
an elliptic equation for the pressure using Robin boundary conditions derived from the normal
component of~\eqref{eq:AMP_CombinedConditions}.




%  (there are two equations, one applied onat a point on the lower surface and one on the corresponding point on the upper surface). 

%- Noting that $\sigmav\nv_\pm = -p(\xsv_+(\ss,t),t)\nv_\pm + \tauv\nv_\pm$ 
%- leads to the AMP condition written in terms of the fluid pressure.  *CHECK ME*
%- % ---------------------------------------------------------------------------------------------------------------
%- \begin{condition}
%- The AMP interface condition for the fluid written in terms of the pressure is 
%- \begin{equation}
%-    -(p\nv)_+ +  (p\nv)_-  -  
%- \frac{\rhos\As}{\rho} \grad p(\xsv_\pm(\ss,t),t)  
%-          = \Lsv\bigl(\uvs^{(p)},\vsv^{(p)}\bigr) + \rhos\As \partialt \wsv^{(p)}_\pm(\ss,t) - (\tauv\nv)_+ - (\tauv\nv)_- , \qquad \ss\in\Gammas.
%-     \label{eq:AMP_CombinedConditionsPressure}
%- \end{equation}
%- % This is used with partitioned FSI schemes by using predicted values for the beam operators that appear on the 
%- % right-hand-side of~\eqref{eq:AMP_CombinedConditionsPressure}.
%- % and with fractional-step fluid solvers by
%- % using predicted values for the fluid stress terms that appear on the 
%- % right-hand-side of~\eqref{eq:AMP_CombinedConditionsPressure}.
%- \end{condition}
%- % ---------------------------------------------------------------------------------------------------------------
%- 

If a fractional-step algorithm is used to integrate the fluid equations, then suitable boundary conditions can be derived by
decomposing~\eqref{eq:AMP_CombinedConditions} into normal and tangential components.  The normal component gives a boundary condition
for the pressure, while the tangential components, along with the continuity equation~\eqref{eq:fluidDiv3d}, provide boundary conditions
for the velocity. 
% ---------------------------------------------------------------------------------------------------------------
\begin{condition}
The AMP interface conditions for the pressure equation~\eqref{eq:fluidPressure} are given by
\begin{align}
    p_+ -  p_-  
     +  \frac{\rhos\As}{\rho} \frac{\partial}{\partial n_+}p_+ 
       =  - \nv_+^T\Lsv^{(p)} - \rhos\As \nv_{+}^T \partialt \wsv^{(p)}_\pm
          +   \frac{\mu\rhos\As}{\rho}\nv_{+}^T\Delta \vv
       +   \nv_+^T(\tauv\nv)_+  - \nv_+^T(\tauv\nv)_- , \quad \ss\in\Gammas,  \label{eq:AMPpressureBCI} \\
% 
   - p_+ +   p_-  
     +  \frac{\rhos\As}{\rho} \frac{\partial}{\partial n_-}p_- 
       =  - \nv_-^T\Lsv^{(p)} - \rhos\As \nv_{-}^T \partialt \wsv^{(p)}_\pm
           +   \frac{\mu\rhos\As}{\rho}\nv_{-}^T\Delta \vv
        -  \nv_-^T (\tauv\nv)_+  + \nv_-^T(\tauv\nv)_- , \quad \ss\in\Gammas,  \label{eq:AMPpressureBCII}
\end{align}
or for a beam with fluid on only one side:
\begin{align}
    p
     +  \frac{\rhos\As}{\rho} \frac{\partial}{\partial n}p 
       =  - \nv^T\Lsv^{(p)} - \rhos\As \nv^T \partialt \wsv^{(p)}_\pm
       +   \nv^T\tauv\nv, \qquad \qquad \xv\in\Gamma, ~~\ss\in\Gammas,   \label{eq:AMPpressureBCIII}
\end{align}
where $\Lsv^{(p)}\equiv \Lsv\bigl(\uvs^{(p)},\vsv^{(p)}\bigr)$.
\end{condition}

\bigskip
% ---------------------------------------------------------------------------------------------------------------
\begin{condition}
The AMP interface conditions for the velocity to be used when integrating the momentum equation~\eqref{eq:fluidMomentum}
are given by
\begin{align}
  \tanv_{m,+}^T(\tauv\nv)_+ +  \tanv_{m,+}^T(\tauv\nv)_- +   \frac{\mu\rhos\As}{\rho}\tanv_{m,+}^T\Delta \vv
     = \frac{\rhos\As}{\rho}\tanv_{m,+}^T\grad p  
               + \tanv_{m,+}^T\Lsv^{(p)}
        +  \rhos\As \tanv_{m,+}^T \partialt \wsv^{(p)}_+(\ss,t)
          , \quad m=1,2 ,    \label{eq:AMPtangentialVelocityBCI} \\
  \tanv_{m,-}^T(\tauv\nv)_+ +  \tanv_{m,-}^T(\tauv\nv)_- +   \frac{\mu\rhos\As}{\rho}\tanv_{m,-}^T\Delta \vv
     = \frac{\rhos\As}{\rho}\tanv_{m,-}^T\grad p  
               + \tanv_{m,-}^T\Lsv^{(p)}
        +  \rhos\As \tanv_{m,-}^T \partialt \wsv^{(p)}_-(\ss,t)
          , \quad m=1,2 , \label{eq:AMPtangentialVelocityBCII}
\end{align}
or for a beam with fluid on only one side:
\begin{align}
  \tanv_{m}^T\tauv\nv +  \frac{\mu\rhos\As}{\rho}\tanv_{m}^T\Delta \vv
     = \frac{\rhos\As}{\rho}\tanv_{m}^T\grad p  
               + \tanv_{m}^T\Lsv^{(p)}
        +  \rhos\As \tanv_{m}^T \partialt \wsv^{(p)}(\ss,t)
          , \quad m=1,2 ,    \label{eq:AMPtangentialVelocityBCIII}
\end{align}
where $\tanv_{m,\pm}$, $m=1,2$  denote mutually orthonormal tangent vectors. %  on $\GammaI_\pm$ (DEFINE $\GammaI_\pm$ ?).
\end{condition}




% Let the fluid normals on the upper and lower surfaces 
% be denoted by $\nv_+=\nv(\xsv_+(\ss,t),t)$ and $\nv_-=\nv(\xsv_-(\ss,t),t)$, respectively.

\noindent Note: If the beam model only supports motion in the direction normal to the beam reference-line,
then only~\eqref{eq:AMPpressureBCI}-\eqref{eq:AMPpressureBCIII} are 
valid and~\eqref{eq:AMPtangentialVelocityBCI}-\eqref{eq:AMPtangentialVelocityBCIII} should be replaced with a
standard condition on the tangential velocity. For example, equation~\eqref{eq:AMPpressureBCI}-\eqref{eq:AMPpressureBCIII}
can be replaced by setting the tangential component of the fluid velocity equal to the
tangential component of the velocity on the beam surface (i.e. a {\em no-slip} type condition on the tangential velocity),
\begin{equation}
  \tv_\pm^T\vv(\xsv_\pm(\ss,t),t) = \tv_\pm^T\vsv(s,t)+\tv_\pm^T\wsv_\pm(\ss,t), \qquad \ss\in\Gammas,
    \label{eq:TangentialVelocityNoSlip}
\end{equation}
or by setting the tangential component of the traction to zero,  (i.e. a {\em slip wall} condition),
\begin{equation}
  (\tv^T\tauv\nv)_\pm = 0 .
    \label{eq:TangentialVelocitySlip}
\end{equation}

% -------------------------
\subsection{Velocity projection} 
The velocity in the AMP scheme is defined to be a weighted average of the predicted velocities from
the fluid and solid following~\cite{fis2014}. 
This averaging can be motivated by noting that 
for heavy beams the motion of the interface is primarily determined from the beam, however, 
for very light beams 
% when $\Lsv$ is also small, 
the fluid interface
approaches a free surface where the motion of the interface is primarily determined by the fluid itself.
The weighted average correctly accounts for these two limits. 
% Thus in this limit the fluid-beam interface is primarily determined by the fluid
Note that the velocity projection given here extends the one given in~\cite{fis2014}
by considering beams of finite thickness and beams with fluid on two sides.
 

% The algorithm for projecting the interface velocities is as follows.
\begin{algorithmVP}\small
~

% Velocity projection algorithm.
\begin{enumerate}
   \item Compute the projected surface velocities $\vv_\pm^I$ on the beam as a weighted average of the predicted
        fluid surface velocities $\vv_\pm$ and beam surface velocities $\vsv_\pm$,
\begin{align}
    \vv_\pm^I = \gamma \vv_\pm + (1-\gamma) \vsv_\pm ,  \qquad  \gamma=\frac{1}{1 + (\rhos\As)/(\rho \Af)}\label{eq:velocityProjection}
\end{align}
   Note that the algorithm appears to be insensitive to the choice of $\Af$ and we pick $\Af=??$.
   \item Project the surface velocities $\vv_\pm^I$ onto the beam reference line. 
         % using the algorithm  described in Section~\ref{sec:beamSolverNumerical}. CHECK ME
   \item Redefine the beam reference-line velocity $\vsv(s,t)$ to be the velocity obtained from step 2, 
           (or a density weighted average of the two velocities from step 2 when the beam has fluid on two sides).
   \item For beams with fluid on two sides we ensure that fluid velocities on opposite sides of the beam remain consistent with a single
       beam reference-line velocity. Thus the fluid surface velocities $\vv_\pm$ 
       on the two beam surfaces is recomputed using~\eqref{eq:beamSurfaceVelocity}
       and the beam reference-line velocity from step 3.
\end{enumerate}
\end{algorithmVP}

From the perspective of numerical stability, this velocity projection appears to be needed only when the 
beam is quite {\em light}. Otherwise the fluid velocity on the interface could be taken as the velocity of the beam.
This observation is supported by a linear stability analysis as well as numerical experiments. However, in practice we
find that the velocity projection is never harmful and we therefore advocate its use. In addition, for very light beams the
interface acts as a free surface with no surface tension (assuming $\Lsv$ is also very small). 
In this case, the fluid interface velocity is smoothed using a few steps of a fourth-order filter
to remove oscillations that can be excited on the interface, see Section~\ref{sec:velocityFilter} for
more details. Finally note that for cases where the beam supports motion only in the normal direction to the beam, only the 
normal component of the fluid velocity is projected, 
\begin{align}
   (\nv^T\vv)_\pm^I = \gamma (\nv^T\vv)_\pm + (1-\gamma) (\nv^T\vsv)_\pm  .  \label{eq:velocityProjectionNormalComponent}
\end{align}

%\medskip
%\noindent{Notes.}
%\begin{enumerate}
%  \item The weighting parameter $\gamma$ is taken to be 
%\begin{align*}
%    \gamma = \frac{1}{1 + (\rhos\As)/(\rho \Af)}.
%\end{align*}
%where $\Af$ is a measure of the volume of the fluid domain. The algorithm appears to be quite insensitive to the
%choice of $\Af$. 
%% 
%\item Step 4 will
%       ensure that the fluid velocities on opposite sides on the beam will remain consistent with a single
%       beam reference-line velocity.
%%
% \item The velocity projection appears to be generally only needed when the beam is quite {\em light}. 
%Otherwise the fluid velocity on the interface can be taken from the velocity of the beam.
%%
%  \item For very light beams the
%interface acts a free surface with no surface tension (assuming $\Lsv$ is also very small). 
%In this case, the fluid interface velocity is smoothed with a few steps of a fourth-order filter
%to remove oscillations that can be excited on the interface, see Section~\ref{sec:velocityFilter} for
%more details.
%% 
% \item For beams with fluid on two-sides, and where the fluid densities are different 
%on the two sides it may be appropriate to use a fluid density weighted average in step 3. We have not as yet evaluated
%this situation. 
%% 
%\item  For the case when the beam only supports motion in the normal direction to the beam, only the 
%normal component of the velocity is projected, 
%\begin{align}
%   (\nv^T\vv)_\pm^I = \gamma (\nv^T\vv)_\pm + (1-\gamma) (\nv^T\vsv)_\pm  .  \label{eq:velocityProjectionNormalComponent}
%\end{align}
%\end{enumerate}

% 
% Following~\cite{fis2014}, the interface velocity $\vv^I$ is defined to be a weighted average of the predicted velocities from
% the fluid and solid. For example, if the fluid velocity on a point on the top or bottom surface $\xsv_\pm$ is $\vv_\pm$
% then we take the interface velocity to be 
% \begin{align}
%     \vv_\pm^I = \gamma \vv_\pm + (1-\gamma) \vsv_\pm   \label{eq:velocityProjection}
% \end{align}
% where from~\eqref{eq:kinematicII}, $\vsv_\pm$ is the velocity of a point on the surface of the beam
% \begin{align*}
%   \vsv_\pm = \vsv(s,t) \pm \wsv_\pm(s,t)
% \end{align*}
% and where
% \begin{align*}
%     \gamma = \frac{1}{1 + (\rhos\As)/(\rho h_f)}.
% \end{align*}
% The parameter $h_f$  is ... FINISH ME. 
% Equation~\eqref{eq:velocityProjection} defines the projected velocity on the surface(s) of the beam. 
% Given values on the beam surface(s) we need to determine a projected beam velocity $\vsv(s,t)$ on the beam reference-line. 
% Note that velocity values on the beam surface correspond to velocity values on the beam reference line according
% to the transformation~\eqref{eq:kinematicII}, 
% Therefore we transfer the surface velocities to the beam reference line
% using~\eqref{eq:kinematicII} to determine the projected beam velocity. For a beam with fluid on two surfaces, we
% take some average value of the two projected velocities (THIS COULD CHANGE if the fluid densities on the two
% sides are not the same). 
% 
% 
% Note that for the case when the beam only supports motion in the normal direction to the beam we only project the
% normal component of the velocity,
% \begin{align}
%    (\nv^T\vv)_\pm^I = \gamma (\nv^T\vv)_\pm + (1-\gamma) (\nv^T\vsv)_\pm   \label{eq:velocityProjectionNormalComponent}
% \end{align}



% 
% Since beam model may have it's own discretization and degrees of freedom it is not straightfoward to 
% adjust the beam velocity on the reference-line to match the values of $\vv^I$ on the beam surfaces. 
% For ease of implementation we thus
% use a relaxation procedure to force the beam reference-line velocity $\vsv$ to approximately match the
% interface velocities $\vv_\pm^I$. We do this by adding an extra relaxation term proportional to the beam velocity 
% to the right-hand side
% of the beam equation~\eqref{eq:beamEquation}
% \begin{alignat}{3}
%      - K_I \vsv
% %   \rhos \As \frac{\partial^2 \uvs}{\partial t^2} =& \Lvs(\uvs,\vvs) +\fsv(s,t), \quad && \ss\in[0,\ls], \quad t\ge 0,
% \end{alignat}
% and adjust the fluid force on the beam surfaces to be 
% \begin{alignat}{3}
%    \sigmav\nv \rightarrow \sigmav\nv + K_I \vv_\pm^I 
% \end{alignat}
% Roughly speaking, this will add a term of the form $-K_I ( \vsv - \vv^I)$ to the beam equation. 
% When $K_I/(\rhos\As)$ is large this will cause the beam velocity to be consistent with the chosen interface velocities.
% When the beam is {\em heavy} this term should have little affect since $K_I/(\rhos\As)$ will be small
% and also since the interface velocity will be primarily determined by the beam velocity, $\vsv \approx \vv^I$,
% from the velocity projection~\eqref{eq:velocityProjection}.


==> texFiles/algorithmOld.tex <==
\section{AMP algorithm} \label{sec:AMPalgorithm}

The AMP algorithm for coupling an incompressible fluid and a shell or beam
was described in~\cite{fis2014} where a simplified situtation was considered with the
equations of motion linearized about infinitesimal amplitude perturbations
and applied to a specific geometry of a fluid in a box with a
beam on one of the faces of the box.
Here the more general case of finite amplitude deformations is considered 
% (although we continue to use a beam model only valid for small amplitude deformations) 
and more general geometries where, for example, the beam may have fluid on two sides or the
beam may have one end immersed in the fluid.
% can be immersed within the fluid. 
The AMP interface conditions for this more general situation are derived below. 
The primary 
difference for beams with fluid on two sides is that the Robin interface condition for the pressure
now involves the pressure at opposite sides of the beam. 
% are basically the same as those given in~\cite{fis2014}. 
%  with a few minor differences. 
%
% The kinematic interface condition~\eqref{eq:kinematic} can be written using the EB approximation to
% relate the velocity of the fluid and the velocity of the beam by 
% \begin{align}
%     \vv(\xsv_\pm(\ss,t),t) &= \frac{\partial}{\partial t}\xsv_{\pm}(\ss,t) 
%                               = \vsv(\ss,t) \pm (\hs/2) \partialt\nsv(\ss,t) , \nonumber  \\
%                           &= \vsv(\ss,t) \pm \wsv,   \label{eq:velocityInterface}
% \end{align} 
% where we have defined $\wsv \equiv (\hs/2) \partialt\nsv(\ss,t)$. 
%

From the time derivative of the kinematic interface condition~\eqref{eq:kinematicII} combined with~\eqref{eq:beamSurfaceVelocity},
we obtain
\begin{align}
&  \frac{D}{Dt}\vv(\xsv_\pm(\ss,t),t)  = \partialt \vsv(\ss,t) + \partialt\wsv_\pm , \label{eq:interfaceAcceleration}
\end{align}
where $D/Dt$ is the total time derivative, 
\begin{align}
   \frac{D\vv}{Dt} = \vv_t + (\vv\cdot\grad)\vv. 
\end{align}
From~\eqref{eq:interfaceAcceleration}, it follows that acceleration of the beam is 
\begin{align}
    \frac{\partial^2 \uvs}{\partial t^2} = \partialt \vsv(\ss,t) = \frac{D}{Dt}\vv(\xsv_\pm(\ss,t),t) - \partialt\wsv_\pm . \label{eq:beamAccel}
\end{align}
% Solving for $\partial_t \vsv(\ss,t)$ from ~\eqref{eq:interfaceAcceleration} and sub
% Replacing $\partial^2\usv/\partial^2 t$ in the beam equation~\eqref{eq:beamEquation} with the expression for
% Substituting~\eqref{eq:interfaceAcceleration} into the beam equation~\eqref{eq:beamEquation} gives the following
% interface condition on the fluid, 
Substituting~\eqref{eq:beamAccel} into the beam equation~\eqref{eq:beamEquation} results in the following relation,
\begin{align}
&  \rhos\As \frac{D}{Dt}\vv(\xsv_\pm(\ss,t),t)  = \Lsv(\usv,\vsv)  
                 + \rhos\As \partialt \wsv_\pm(\ss,t)  + \fsv(\ss,t) ,    \qquad \ss\in\Gammas.  \label{eq:AMPcondition}
\end{align}
Using the fluid momentum equation~\eqref{eq:fluidMomentum} to replace $D\vv/Dt$ in~\eqref{eq:AMPcondition} gives
\begin{equation}
  \frac{\rhos\As}{\rho}\grad\cdot\sigmav(\xsv_\pm(\ss,t),t)  = \Lsv\bigl(\uvs,\vsv\bigr) + \rhos\As \partialt \wsv_\pm(\ss,t)  + \fsv(\ss,t),
          \qquad \ss\in\Gammas.
    \label{eq:AMPconditionSigma}
\end{equation}
Substituting the expression~\eqref{eq:dynamic} for $\fsv$ 
gives 
\begin{equation}
    (\sigmav\nv)_+ + (\sigmav\nv)_- + 
\frac{\rhos\As}{\rho}\grad\cdot\sigmav(\xsv_\pm(\ss,t),t)  
         = \Lsv\bigl(\uvs,\vsv\bigr) + \rhos\As \partialt \wsv_\pm(\ss,t) , \qquad \ss\in\Gammas.
    \label{eq:AMP_ContinuousConditions}
\end{equation}
Equation~\eqref{eq:AMP_ContinuousConditions} appears to be a condition that fully couples the
fluid and solid values on the interface. However, the critical observation is that~\eqref{eq:AMP_ContinuousConditions}
can be used as a stable  condition for {\em partitioned} schemes by using {\em predicted} values
for the solid variables $\usv^{(p)}$, $\vsv^{(p)}$ and $\wsv^{(p)}$ when evaluating the right-hand-side 
terms in~\eqref{eq:AMP_ContinuousConditions}.
% Note that the fluid traction terms on the left-hand side of~\eqref{eq:AMP_ContinuousConditions}, which orginally appeared in the beam equations, 
% 
This leads to the primary AMP interface condition:
% ---------------------------------------------------------------------------------------------------------------
\begin{condition}
The AMP interface condition for the fluid is 
\begin{equation}
    (\sigmav\nv)_+ + (\sigmav\nv)_- + 
\frac{\rhos\As}{\rho}\grad\cdot\sigmav(\xsv_\pm(\ss,t),t)  
         = \Lsv\bigl(\uvs^{(p)},\vsv^{(p)}\bigr) + \rhos\As \partialt \wsv^{(p)}_\pm(\ss,t) , \qquad \ss\in\Gammas,
    \label{eq:AMP_CombinedConditions}
\end{equation}
where $\usv^{(p)}$, $\vsv^{(p)}$ and $\wsv^{(p)}$ are predicted solid values.
For a beam with fluid on only one side the condition is
\begin{equation}
    \sigmav\nv + 
\frac{\rhos\As}{\rho}\grad\cdot\sigmav
         = \Lsv\bigl(\uvs^{(p)},\vsv^{(p)}\bigr) + \rhos\As \partialt \wsv^{(p)}(\ss,t) , \qquad \xv\in\Gamma, ~~\ss\in\Gammas,
    \label{eq:AMP_CombinedConditionsOneSide}
\end{equation}
% This is used with partitioned FSI schemes by using predicted values for the beam operators that appear on the 
% right-hand-side of~\eqref{eq:AMP_CombinedConditions}.
\end{condition}
% ---------------------------------------------------------------------------------------------------------------
% When the beam has fluid on two sides, the two 
% conditions ($\pm$) in~\eqref{eq:AMP_CombinedConditions} are generalized Robin interface conditions that
% involve the fluid traction at points
% on opposite sides of the beam. For a beam with fluid on only one side, there will be only one condition applied,
% with the traction term on the opposite side set to zero, or some specified value. 

In a partitioned scheme the solid would first be advanced to the new time step, providing the predicted
values used in the interface conditions~\eqref{eq:AMP_CombinedConditions} 
that are used when solving for the fluid values. This process can be viewed as 
computing the solution to a generalized Riemann problem at the interface and generalizes the AMP
scheme for compressible fluids and compressible solids~\cite{BanksSjogreen2011,fsi2012}.
In the purely hyperbolic
problem the Riemann problem has piecewise constant initial conditions and the solution is computed
using characteristics, giving interface values that are impedance weighted averages of the fluid and solid states. 
In the present case the initial conditions for the Riemann problem 
for the solid domain are $\usv^{(p)}$, $\vsv^{(p)}$. In the fluid domain the velocity can also be predicted when 
using a fractional step scheme. The solution to the Riemann problem then requires the solution of
an elliptic equation for the pressure using Robin boundary conditions derived from the normal
component of~\eqref{eq:AMP_CombinedConditions}.




%  (there are two equations, one applied onat a point on the lower surface and one on the corresponding point on the upper surface). 

%- Noting that $\sigmav\nv_\pm = -p(\xsv_+(\ss,t),t)\nv_\pm + \tauv\nv_\pm$ 
%- leads to the AMP condition written in terms of the fluid pressure.  *CHECK ME*
%- % ---------------------------------------------------------------------------------------------------------------
%- \begin{condition}
%- The AMP interface condition for the fluid written in terms of the pressure is 
%- \begin{equation}
%-    -(p\nv)_+ +  (p\nv)_-  -  
%- \frac{\rhos\As}{\rho} \grad p(\xsv_\pm(\ss,t),t)  
%-          = \Lsv\bigl(\uvs^{(p)},\vsv^{(p)}\bigr) + \rhos\As \partialt \wsv^{(p)}_\pm(\ss,t) - (\tauv\nv)_+ - (\tauv\nv)_- , \qquad \ss\in\Gammas.
%-     \label{eq:AMP_CombinedConditionsPressure}
%- \end{equation}
%- % This is used with partitioned FSI schemes by using predicted values for the beam operators that appear on the 
%- % right-hand-side of~\eqref{eq:AMP_CombinedConditionsPressure}.
%- % and with fractional-step fluid solvers by
%- % using predicted values for the fluid stress terms that appear on the 
%- % right-hand-side of~\eqref{eq:AMP_CombinedConditionsPressure}.
%- \end{condition}
%- % ---------------------------------------------------------------------------------------------------------------
%- 

If a fractional-step algorithm is used to integrate the fluid equations, then suitable boundary conditions can be derived by
decomposing~\eqref{eq:AMP_CombinedConditions} into normal and tangential components.  The normal component gives a boundary condition
for the pressure, while the tangential components, along with the continuity equation~\eqref{eq:fluidDiv3d}, provide boundary conditions
for the velocity. 
% ---------------------------------------------------------------------------------------------------------------
\begin{condition}
The AMP interface conditions that can be used when solving the pressure equation~\eqref{eq:fluidPressure} are given by
\begin{align}
    p_+ -  p_-  
     +  \frac{\rhos\As}{\rho} \frac{\partial}{\partial n_+}p_+ 
       =  - \nv_+^T\Lsv^{(p)} - \rhos\As \nv_{+}^T \partialt \wsv^{(p)}_\pm
          +   \frac{\mu\rhos\As}{\rho}\nv_{+}^T\Delta \vv
       +   \nv_+^T(\tauv\nv)_+  - \nv_+^T(\tauv\nv)_- , \quad \ss\in\Gammas,  \label{eq:AMPpressureBCI} \\
% 
   - p_+ +   p_-  
     +  \frac{\rhos\As}{\rho} \frac{\partial}{\partial n_-}p_- 
       =  - \nv_-^T\Lsv^{(p)} - \rhos\As \nv_{-}^T \partialt \wsv^{(p)}_\pm
           +   \frac{\mu\rhos\As}{\rho}\nv_{-}^T\Delta \vv
        -  \nv_-^T (\tauv\nv)_+  + \nv_-^T(\tauv\nv)_- , \quad \ss\in\Gammas,  \label{eq:AMPpressureBCII}
\end{align}
or for a beam with fluid on only one side:
\begin{align}
    p
     +  \frac{\rhos\As}{\rho} \frac{\partial}{\partial n}p 
       =  - \nv^T\Lsv^{(p)} - \rhos\As \nv^T \partialt \wsv^{(p)}_\pm
       +   \nv^T\tauv\nv, \qquad \qquad \xv\in\Gamma, ~~\ss\in\Gammas,   \label{eq:AMPpressureBCIII}
\end{align}
where $\Lsv^{(p)}\equiv \Lsv\bigl(\uvs^{(p)},\vsv^{(p)}\bigr)$.
\end{condition}

\bigskip
% ---------------------------------------------------------------------------------------------------------------
\begin{condition}
The AMP interface conditions for the velocity that can be used when integrating the momentum equation~\eqref{eq:fluidMomentum}
are given by
\begin{align}
  \tanv_{m,+}^T(\tauv\nv)_+ +  \tanv_{m,+}^T(\tauv\nv)_- +   \frac{\mu\rhos\As}{\rho}\tanv_{m,+}^T\Delta \vv
     = \frac{\rhos\As}{\rho}\tanv_{m,+}^T\grad p  
               + \tanv_{m,+}^T\Lsv^{(p)}
        +  \rhos\As \tanv_{m,+}^T \partialt \wsv^{(p)}_+(\ss,t)
          , \quad m=1,2 ,    \label{eq:AMPtangentialVelocityBCI} \\
  \tanv_{m,-}^T(\tauv\nv)_+ +  \tanv_{m,-}^T(\tauv\nv)_- +   \frac{\mu\rhos\As}{\rho}\tanv_{m,-}^T\Delta \vv
     = \frac{\rhos\As}{\rho}\tanv_{m,-}^T\grad p  
               + \tanv_{m,-}^T\Lsv^{(p)}
        +  \rhos\As \tanv_{m,-}^T \partialt \wsv^{(p)}_-(\ss,t)
          , \quad m=1,2 , \label{eq:AMPtangentialVelocityBCII}
\end{align}
or for a beam with fluid on only one side:
\begin{align}
  \tanv_{m}^T\tauv\nv +  \frac{\mu\rhos\As}{\rho}\tanv_{m}^T\Delta \vv
     = \frac{\rhos\As}{\rho}\tanv_{m}^T\grad p  
               + \tanv_{m}^T\Lsv^{(p)}
        +  \rhos\As \tanv_{m}^T \partialt \wsv^{(p)}(\ss,t)
          , \quad m=1,2 ,    \label{eq:AMPtangentialVelocityBCIII}
\end{align}
where $\tanv_{m,\pm}$, $m=1,2$  denote mutually orthonormal tangent vectors. %  on $\GammaI_\pm$ (DEFINE $\GammaI_\pm$ ?).
\end{condition}




% Let the fluid normals on the upper and lower surfaces 
% be denoted by $\nv_+=\nv(\xsv_+(\ss,t),t)$ and $\nv_-=\nv(\xsv_-(\ss,t),t)$, respectively.

\noindent Note: If the beam model only supports motion in the direction normal to the beam reference-line,
then only~\eqref{eq:AMPpressureBCI}-\eqref{eq:AMPpressureBCIII} are 
valid and~\eqref{eq:AMPtangentialVelocityBCI}-\eqref{eq:AMPtangentialVelocityBCIII} should be replaced with a
standard condition on the tangential velocity. For example, equation~\eqref{eq:AMPpressureBCI}-\eqref{eq:AMPpressureBCIII}
can be replaced by setting the tangential component of the fluid velocity equal to the
tangential component of the velocity on the beam surface (i.e. a {\em no-slip} type condition on the tangential velocity),
\begin{equation}
  \tv_\pm^T\vv(\xsv_\pm(\ss,t),t) = \tv_\pm^T\vsv(s,t)+\tv_\pm^T\wsv_\pm(\ss,t), \qquad \ss\in\Gammas,
    \label{eq:TangentialVelocityNoSlip}
\end{equation}
or by setting the tangential component of the traction to zero,  (i.e. a {\em slip wall} condition),
\begin{equation}
  (\tv^T\tauv\nv)_\pm = 0 .
    \label{eq:TangentialVelocitySlip}
\end{equation}

% -------------------------
\paragraph{Velocity projection} 
The AMP interface velocity is defined to be a weighted average of the predicted velocities from
the fluid and solid following~\cite{fis2014}. 
This averaging can be motivated by noting that 
for heavy beams the motion of the interface is primarily determined from the beam, however, 
for very light beams 
% when $\Lsv$ is also small, 
the fluid interface
approaches a free surface where the motion of the interface is primarly determined by the fluid itself.
The weighted average correctly accounts for these two limits. 
% Thus in this limit the fluid-beam interface is primarily determined by the fluid
Note that the velocity projection given here extends the one given in~\cite{fis2014}
by considering beams of finite thickness and beams with fluid on two sides.
 

% The algorithm for projecting the interface velocities is as follows.
\begin{algorithmVP}\small
~

% Velocity projection algorithm.
\begin{enumerate}
   \item Compute the projected surface velocities $\vv_\pm^I$ on the beam as a weighted average of the predicted
        fluid surface velocities $\vv_\pm$ and beam surface velocities $\vsv_\pm$,
\begin{align}
    \vv_\pm^I = \gamma \vv_\pm + (1-\gamma) \vsv_\pm ,   \label{eq:velocityProjection}
\end{align}
   where $\gamma$ is defined below.
   \item Project the surface velocities $\vv_\pm^I$ onto the beam reference line. 
         % using the algorithm  described in Section~\ref{sec:beamSolverNumerical}. CHECK ME
   \item Redefine the beam reference-line velocity $\vsv(s,t)$ to be the velocity obtained from step 2, 
           (or a weighted average of the two velocities from step 2, when the beam has fluid on two sides).
   \item For beams with fluid on two-sides, recompute the fluid surface velocities $\vv_\pm$ 
       on the two beam surfaces using~\eqref{eq:beamSurfaceVelocity}
       and then redefined
       reference-line beam velocity from step 3.
\end{enumerate}
\end{algorithmVP}

\medskip
\noindent{Notes.}
\begin{enumerate}
  \item The weighting parameter $\gamma$ is taken to be 
\begin{align*}
    \gamma = \frac{1}{1 + (\rhos\As)/(\rho \Af)}.
\end{align*}
where $\Af$ is a measure of the volume of the fluid domain. The algorithm appears to be quite insensitive to the
choice of $\Af$. 
% 
\item Step 4 will
       ensure that the fluid velocities on opposite sides on the beam will remain consistent with a single
       beam reference-line velocity.
%
 \item The velocity projection appears to be generally only needed when the beam is quite {\em light}. 
Otherwise the fluid velocity on the interface can be taken from the velocity of the beam.
%
  \item For very light beams the
interface acts a free surface with no surface tension (assuming $\Lsv$ is also very small). 
In this case, the fluid interface velocity is smoothed with a few steps of a fourth-order filter
to remove oscillations that can be excited on the interface, see Section~\ref{sec:velocityFilter} for
more details.
% 
 \item For beams with fluid on two-sides, and where the fluid densities are different 
on the two sides it may be appropriate to use a fluid density weighted average in step 3. We have not as yet evaluated
this situation. 
% 
\item  For the case when the beam only supports motion in the normal direction to the beam, only the 
normal component of the velocity is projected, 
\begin{align}
   (\nv^T\vv)_\pm^I = \gamma (\nv^T\vv)_\pm + (1-\gamma) (\nv^T\vsv)_\pm  .  \label{eq:velocityProjectionNormalComponent}
\end{align}
\end{enumerate}

% 
% Following~\cite{fis2014}, the interface velocity $\vv^I$ is defined to be a weighted average of the predicted velocities from
% the fluid and solid. For example, if the fluid velocity on a point on the top or bottom surface $\xsv_\pm$ is $\vv_\pm$
% then we take the interface velocity to be 
% \begin{align}
%     \vv_\pm^I = \gamma \vv_\pm + (1-\gamma) \vsv_\pm   \label{eq:velocityProjection}
% \end{align}
% where from~\eqref{eq:kinematicII}, $\vsv_\pm$ is the velocity of a point on the surface of the beam
% \begin{align*}
%   \vsv_\pm = \vsv(s,t) \pm \wsv_\pm(s,t)
% \end{align*}
% and where
% \begin{align*}
%     \gamma = \frac{1}{1 + (\rhos\As)/(\rho h_f)}.
% \end{align*}
% The parameter $h_f$  is ... FINISH ME. 
% Equation~\eqref{eq:velocityProjection} defines the projected velocity on the surface(s) of the beam. 
% Given values on the beam surface(s) we need to determine a projected beam velocity $\vsv(s,t)$ on the beam reference-line. 
% Note that velocity values on the beam surface correspond to velocity values on the beam reference line according
% to the transformation~\eqref{eq:kinematicII}, 
% Therefore we transfer the surface velocities to the beam reference line
% using~\eqref{eq:kinematicII} to determine the projected beam velocity. For a beam with fluid on two surfaces, we
% take some average value of the two projected velocities (THIS COULD CHANGE if the fluid densities on the two
% sides are not the same). 
% 
% 
% Note that for the case when the beam only supports motion in the normal direction to the beam we only project the
% normal component of the velocity,
% \begin{align}
%    (\nv^T\vv)_\pm^I = \gamma (\nv^T\vv)_\pm + (1-\gamma) (\nv^T\vsv)_\pm   \label{eq:velocityProjectionNormalComponent}
% \end{align}



% 
% Since beam model may have it's own discretization and degrees of freedom it is not straightfoward to 
% adjust the beam velocity on the reference-line to match the values of $\vv^I$ on the beam surfaces. 
% For ease of implementation we thus
% use a relaxation procedure to force the beam reference-line velocity $\vsv$ to approximately match the
% interface velocities $\vv_\pm^I$. We do this by adding an extra relaxation term proportional to the beam velocity 
% to the right-hand side
% of the beam equation~\eqref{eq:beamEquation}
% \begin{alignat}{3}
%      - K_I \vsv
% %   \rhos \As \frac{\partial^2 \uvs}{\partial t^2} =& \Lvs(\uvs,\vvs) +\fsv(s,t), \quad && \ss\in[0,\ls], \quad t\ge 0,
% \end{alignat}
% and adjust the fluid force on the beam surfaces to be 
% \begin{alignat}{3}
%    \sigmav\nv \rightarrow \sigmav\nv + K_I \vv_\pm^I 
% \end{alignat}
% Roughly speaking, this will add a term of the form $-K_I ( \vsv - \vv^I)$ to the beam equation. 
% When $K_I/(\rhos\As)$ is large this will cause the beam velocity to be consistent with the chosen interface velocities.
% When the beam is {\em heavy} this term should have little affect since $K_I/(\rhos\As)$ will be small
% and also since the interface velocity will be primarily determined by the beam velocity, $\vsv \approx \vv^I$,
% from the velocity projection~\eqref{eq:velocityProjection}.


==> texFiles/analysis-5-20-15.tex <==
%---------------------------------------------------------------------
\section{Analysis of a model problem for a two-dimensional beam} \label{sec:analysis}
{% ------ linearizedTwoSidedBeam ------
\newcommand{\figWidth}{8cm}
\newcommand{\trimfig}[2]{\trimFig{#1}{#2}{0}{0}{0}{0}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.0,0) rectangle (8cm,8cm);  % set the bounding box (so we have less surrounding white space)
%   \draw(0.0,4.4) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/fc2Gridt0p010}{\figWidth}};
  \draw(0.0,0.0) node[anchor=south west,xshift=0pt,yshift=0pt] {\trimfig{fig/linearizedTwoSidedBeam.pdf}{\figWidth}};
% grid:
%  \draw[step=1cm,gray] (0,0) grid (16,5);
\end{tikzpicture}
\end{center}
  \caption{The geometry of the linearized model  for  a beam with fluid on two sides.}
  \label{fig:linearizedTwoSidedBeam}
\end{figure}
}

Notes: 

-wdh: Fig. 2: do you have the latex source we can use instead if the pdf? need to change L to $\ls$

In this section, the stability of the AMP algorithm is investigated for a linearized model problem consisting of a EB beam coupled to inviscid, incompressible fluids with different constant fluid densities in the regions above and below the beam as shown in
Figure~\ref{fig:linearizedTwoSidedBeam}.  For comparitive purposes, we also consider the stability of a traditional partitioned (TP) scheme for the same model problem.  We begin by obtaining the exact solution of the model problem to explicitly identify the contribution of the
added mass of the fluid for two different choices of the boundary conditions on the fluid. The stability of the discrete AMP and TP schemes is then investigated using a mode analysis that
extends the theory for the case of a beam with fluid on one side only presented in~\cite{fis2014}.
 For both the AMP and TP schemes, the fluid
equations are advanced using a backward-Euler time integrator as opposed to the predictor-corrector integrator
described in Section~\ref{sec:AMPalgorithm}.  While this simplifies the analysis somewhat, the essential results are unaffected.  It is found,
in agreement with~\cite{fis2014}, that the AMP scheme is stable for arbitrarily light structures provided the usual convective time-step restriction is satisfied.  The TP scheme without sub-time step iteration, on the other hand, becomes unconditionally unstable for light structures.  Note that the TP scheme has been analyzed previously by Causin, Gerbeau
and Nobile~\cite{CausinGerbeauNobile2005}, among others, and the results presented here extend those works.


In the following analysis the two fluids
% are assumed to be inviscid and incompressible, and
are coupled to an
EB beam with constant thickness $\hs$ and without damping terms. The equations describing the evolution of the fluid-structure system are then linearized 
about flat undeflected beam surfaces at $y=-\hs/2$ and $\hs/2$ as shown in Figure~\ref{fig:linearizedTwoSidedBeam}.
Let $\rho^+(x,y,t)$, $\vv^+(x,y,t)$ and $p^+(x,y,t)$, denote the fluid density, velocity and pressure, respectively, in the upper domain, $\OmegaF_{+}=[0,\ls]\times[\hs/2,\Hf^{+}]$, 
and $\rho^-(x,y,t)$, $\vv^-(x,y,t)$ and $p^-(x,y,t)$, the corresponding quantities in the lower domain $\OmegaF_{-}=[0,\ls]\times[\Hf^{-},-\hs/2]$, where $\ls$ is the length of the beam.
The governing equations and boundary conditions for this model are 
\begin{equation}
\begin{array}{rl}
\text{Fluid:} &
\displaystyle{
 \left\{ 
   \begin{alignedat}{3}
  &  \rho^{\pm}\frac{\partial\vv^{\pm}}{\partial t} 
                 + \grad p^{\pm} =0, \qquad&& \xv\in\OmegaF_{\pm} ,  \\
  & \grad\cdot\vv^{\pm} =0,  \qquad&& \xv\in\OmegaF_{\pm} ,   \\
  & v_2^\pm=0\text{ or } p^{\pm}=0  , \qquad&& x\in(0,\ls), \quad y=\Hf^{\pm}
   \end{alignedat}  \right. % \label{eq:MP1v}
} 
\medskip\\
\text{Beam:} &
\displaystyle{
  \left\{
   \begin{alignedat}{3}
  &  \rhos\hs\frac{\partial^2\eta}{\partial t^2}  = -\Ks_0 \eta + \Ts\frac{\partial^2\eta}{\partial x^2} - \Es\Is\frac{\partial^4\eta}{\partial x^4} + f(x,t), \qquad&&  x\in(0,\ls),
   \end{alignedat}
   \right.
}
\medskip\\
\text{Interface:} &
\displaystyle{
  \left\{
   \begin{alignedat}{3}
  & v_2^{\pm}=\frac{\partial\eta}{\partial t}, \qquad && x\in(0,\ls), \quad y=\pm\hs/2, \\ % x\in\OmegaS .
  & f(x,t)=p^{-}(x,-\hs/2,t) - p^{+}(x,\hs/2,t),\qquad &&  x\in(0,\ls),
   \end{alignedat}  \right.
}
% 
\end{array}
  \label{eq:MP1}
\end{equation}
with periodic boundary conditions in the $x$-direction. 
Initial conditions for $\vv^\pm$, $\eta$ and $\partial\eta/\partial t$ are needed to complete the specification of the problem, but these are not required in the subsequent analysis. 
% 
% To begin the analysis, the solution is expanded in a finite Fourier series in $x$ (i.e.~a pseudo-spectral approximation), which gives 


%%%%%
%% slip wall BCs
%%%%%
\subsection{Exact solution of the continuous model problem} \label{subsec:slipWallBCs}

It is instructive to first examine the behavior of the exact solution of the FSI problem in~\eqref{eq:MP1}.  Since this model problem is a linear constant-coefficient system of equations with periodic boundary conditions in the $x$-direction, the solution can be expressed in terms of a Fourier series in~$x$, e.g.
\[
\vv^{\pm}(x,y,t)=\sum_{k=-\infty}\sp\infty \vvh^{\pm}(k,y,t)\exp(-i\kx x),\qquad \kx = 2\pi k/\ls,
\]
and similar expressions for $p\sp\pm$ and $\eta\sp\pm$.  Here, $\kx$ identifies the wave number of the Fourier mode.  Transforming the equations for the fluid to Fourier space gives
\begin{equation}
\left. \begin{array}{r}
\displaystyle{
  \rho^{\pm} \frac{\partial \vh_1^{\pm}}{\partial t} - i\kx \ph^{\pm} =0
} \smallskip\\
\displaystyle{
  \rho^{\pm} \frac{\partial \vh_2^{\pm}}{\partial t} + \frac{\partial \ph^{\pm}}{\partial y} =0
} \smallskip\\
\displaystyle{
  -i\kx\vh_1^{\pm}+{\partial\vh_2^{\pm}\over\partial y} =0
}
\end{array}
\right\},\qquad
\begin{array}{l}
  \hbox{$y \in (\Hf^{-},-\hs/2)$ for the lower fluid},\medskip\\
  \hbox{$y \in (\hs/2,\Hf^{+})$ for the upper fluid}.\\
\end{array}
\label{eq:modelFluidEquationFT}
\end{equation}
The transformed equation for the beam is
\begin{equation}
  \rhos\hs \frac{\partial ^2\etah}{\partial t^2} = - \Lt \etah + \ph^{-}(-\hs/2,t)-\ph^{+}(\hs/2,t),
\label{eq:modelShellEquationFT}
\end{equation}
where $\Lt=\Ks_0+\Ts\kx^2+\Es\Is\kx^4$, 
and for notational brevity we have suppressed the functional dependence on the wave number.

The transformed equations for the fluid in~\eqref{eq:modelFluidEquationFT} can be manipulated to derive an equation for the pressure of the form
\begin{equation}
{\partial\sp2\ph\sp\pm\over\partial y\sp2}+\kx\sp2\ph\sp\pm=0.
\label{eq:modelPressureEquationFT}
\end{equation}
It is assumed that $\kx\ne0$ in the present analysis while the special case when $\kx=0$ is considered later.  For the case of the rigid-wall boundary condition $\vh_2^{\pm}=0$ at $y=\Hf^{\pm}$, we use the $y$-momentum equation in~\eqref{eq:modelFluidEquationFT} to derive the Neumann condition for the pressure,
\begin{equation}
  \frac{\partial \ph^{\pm}}{\partial y}(\Hf^{\pm},t)=0.
  \label{eq:modelBCFT}
\end{equation}
A general solution of the pressure equation in~\eqref{eq:modelPressureEquationFT} satisfying the homogeneous boundary condition in~\eqref{eq:modelBCFT}~is
\begin{equation}
  \ph^{\pm} = a^{\pm}\cosh\left(\kx(y-H^{\pm})\right), \label{eq:pSolution}
\end{equation}
where $a^{\pm}$ is a time-dependent coefficient function.  Similarly, the kinematic condition at the interface,
\[
\vh_2^{\pm}(\pm\hs/2,t)=\frac{\partial\etah}{\partial t},
\]
together with the $y$-momentum equation in~\eqref{eq:modelFluidEquationFT} gives the interface condition
\begin{equation}
  \frac{\partial \ph^{\pm}}{\partial y}(\pm\hs/2,t)=  -\rho^{\pm}\frac{\partial^2\etah}{\partial t^2}.
  \label{eq:modelInterfaceFTpy}
\end{equation}
The general solution in~\eqref{eq:pSolution} and the interface condition in~\eqref{eq:modelInterfaceFTpy} imply
\begin{equation}
  a^{\pm} = \pm\frac{\rho^{\pm}}{\kx}\left(\frac{\partial^2\etah}{\partial t^2}\right){\rm csch}\left(\kx\mathcal{D}\sp\pm\right),
\label{eq:acoeffs}
\end{equation}
where $\mathcal{D}^{\pm}=\pm\Hf^{+}-\hs/2$ measures the vertical extent of the upper and lower fluid domains.  Using~\eqref{eq:pSolution} and~\eqref{eq:acoeffs},
the applied force appearing in the beam equation~\eqref{eq:modelShellEquationFT} takes the form
\begin{equation}
 \ph^{-}(-\hs/2,t)-\ph^{+}(\hs/2,t) =-\hat{M}_a^{-}\frac{\partial^2\etah}{\partial t^2}-\hat{M}_{a}^{+}\frac{\partial^2\etah}{\partial t^2},
 \label{eq:appliedForceFT}
\end{equation}
where
\begin{equation}
  \hat{M}_a^\pm =\rho^\pm\mathcal{D}^\pm\left[{\coth(\kx\mathcal{D}^\pm)\over\kx\mathcal{D}^\pm}\right] ,\qquad\hbox{(rigid-wall BCs),}
  \label{eq:addedMass}
\end{equation}
are the added masses from the upper and lower fluids for the case of rigid-wall boundary conditions at $y=\Hf^{\pm}$.  For the alternate case of the pressure boundary condition, $\ph^{\pm}=0$ at $y=\Hf^{\pm}$, a similar analysis leads to the added masses given by
\begin{equation}
  \hat{M}_a^\pm =\rho^\pm\mathcal{D}^\pm\left[{\tanh(\kx\mathcal{D}^\pm)\over\kx\mathcal{D}^\pm}\right] ,\qquad\hbox{(pressure BCs).}
  \label{eq:addedMassPressure}
\end{equation}
Finally, using the applied force (\ref{eq:appliedForceFT}) in the equation of motion
for the beam (\ref{eq:modelShellEquationFT}) gives
\begin{equation}
 \Big( \rhos\hs+\hat{M}_a^{-}+\hat{M}_a^{+}\Big) \frac{\partial ^2\etah}{\partial t^2} = - \Lt \etah,
 \label{eq:beamMotionFT}
\end{equation}
which explicitly identifies the contribution of the added mass of the fluid in the beam equation. A solution
to~\eqref{eq:beamMotionFT} satisfying initial conditions for $\etah$ and $\partial\etah/\partial t$ can be found easily to complete the solution of the model problem in Fourier space.



\textcolor{red}{Putting this interpretation of the solution aside for now.}
Note that $\hat{M}_a^{\pm} >0$ and so the added mass associated with the fluids always tends to suppress 
beam acceleration. Indeed, $\hat{M}_a^{\pm}\to\infty$ as $k\to 0$ which indicates that the $k=0$ mode will be the most sensitive
to added-mass effects. In fact for $k=0$ the solution is independent of time and takes the form {\bf check this}
\begin{align}
  & \vh_2(k=0,y,t)^{\pm}=0,\qquad \ph^{\pm}(k=0,y,t) = p_0^\pm,   \label{eq:kZeroContinuous} \\
  & \Ks_0\etah(k=0,t) = p_0^- - p_0^+,  \label{eq:kZeroPressureDiff}
\end{align}
where $p_0^\pm$ are constants (not independent) that balance the initial displacement of the beam through 
through~\eqref{eq:kZeroPressureDiff}. 
The solution is thus determined up to a single constant in the pressure which has no consequential effect on the answer. 
To define a unique solution one additional constraint is needed
such as requiring the mean value of the pressure to be zero.

%%%%%
%% partitioned numerics
%%%%%
\subsection{Stability analysis of the AMP and TP schemes}
The stability of a partitioned scheme for an FSI problem depends crucially on the treatment of the interface and the resulting boundary conditions applied to the fluid and structure on either side.  AMP interface conditions have been developed and used in the AMP FSI time-stepping algorithm, and the purpose of this section is to analyze the stability of a form of this algorithm applied to the model problem in~\eqref{eq:MP1}.  A starting point for this analysis is the system of equations in~\eqref{eq:modelFluidEquationFT} and~\eqref{eq:modelShellEquationFT} already written in Fourier space.  For this system, we consider a discretization in time, but let the dependence on $y$ remain continuous.  This approach reveals the stability of the partitioned algorithm, while keeping the algebraic details as simple as possible.
%We note that a discretization in $y$ could also be considered, but this only makes the analysis messier without providing additional significant information on the main issue of stability.

We begin with an analysis of the AMP algorithm, and then compare the results with a traditional partitioned (TP) in the end.  For both cases, let
\[
\vvh^{n\pm}(y)\approx\vvh^{\pm}(y,t^n), \qquad \ph^{n\pm}(y)\approx\ph^{\pm}(y,t^n), \qquad \etah^{n}\approx\etah(t^n),
\]
where $t^n=n\dt$. Furthermore, let $D_{+t}$ and $D_{-t}$ denote the forward and backward divided different operators in time 
(e.g. $D_{+t}\etah^n=(\etah^{n+1}-\etah^n)/\dt$ and $D_{-t}\etah^n=(\etah^{n}-\etah^{n-1})/\dt$).

The following AMP scheme is an abbreviated version of the full scheme described in Section~\ref{sec:timeStepping}:

% --------------------------------------------------------------------------------------------------------------------------------------
\begin{algorithm}[H] {\bf AMP scheme:} 

\noindent Stage I: Advance the beam displacement using a leap-frog scheme,
\begin{equation}
  \rhos\hs D_{+t}D_{-t}\etah^n  = -\Lt \etah^n + \ph^{n-}(-\hs/2)-\ph^{n+}(\hs/2) .
\label{eq:etaLeapFrogAM}
\end{equation}
Stage II: Advance the fluid velocity and pressure using a backward-Euler scheme applied to the equations in pressure-velocity form,
\begin{equation}
\left. \begin{array}{r}
\displaystyle{
% \rho^{\pm} \frac{\vh_1^{(n+1)\pm}-\vh_1^{n\pm}}{\dt}  + i\kx \ph^{(n+1)\pm} =0
\rho^{\pm} D_{+t} \vh_1^{n\pm}  + i\kx \ph^{(n+1)\pm} =0
} \smallskip\\
\displaystyle{
% \rho^{\pm} \frac{\vh_2^{(n+1)\pm}-\vh_2^{n\pm}}{\dt} + \frac{\partial \ph^{(n+1)\pm}}{\partial y} =0
\rho^{\pm} D_{+t} \vh_2^{n\pm} + \frac{\partial \ph^{(n+1)\pm}}{\partial y} =0
} \smallskip\\
\displaystyle{
\frac{\partial^2 \ph^{(n+1)\pm}}{\partial y^2} - \kx^2 \ph^{(n+1)\pm} =0
}
\end{array} \right\},
\begin{array}{l}
  \qquad y \in (\Hf^{-},-\hs/2) \hbox{ for the lower fluid},\smallskip\\
  \qquad y \in (\hs/2,\Hf^{+}) \hbox{ for the upper fluid},\\
\end{array}
\label{eq:fluidAMP}
\end{equation}
with the AMP Robin interface conditions derived from \eqref{eq:AMPpressureBCI},
\begin{equation}
\ph^{(n+1)-}(-\hs/2)-\ph^{(n+1)+}(\hs/2) + \frac{\rhos\hs}{\rho^{\pm}} \frac{\partial \ph^{(n+1)\pm}}{\partial y} = \Lt \etah^{n+1},\qquad y=\pm\hs/2,
\label{eq:AMPinterfaceBC}
\end{equation}
and boundary conditions,
\begin{equation}
\frac{\partial \ph^{(n+1)\pm}}{\partial y}=0, \qquad y=\Hf^{\pm}.
\label{eq:rbbcs}
\end{equation}
\label{alg:AMP}
\end{algorithm}
% --------------------------------------------------------------------------------------------------------------------------------------

A key ingredient of the AMP scheme is the 
Robin condition in~\eqref{eq:AMPinterfaceBC} for the fluid pressure. This condition, along with~\eqref{eq:etaLeapFrogAM}, implies
\begin{equation}
\frac{\partial \ph^{(n+1)^{\pm}}}{\partial y} = -\rho^{\pm}  D_{+t}D_{-t}\etah^{n+1},\qquad y=\pm\hs/2,
\label{eq:balance}
\end{equation}
which is a discrete version of the interface condition in~\eqref{eq:modelInterfaceFTpy}.
We observe that the acceleration term on the right-hand side of~\eqref{eq:balance} is evaluated at the {\em same time level} as the pressure gradient term on the left-hand side, and this plays an important role in the stability of the AMP scheme as is noted below.
%This is in contrast to the traditional scheme where the acceleration term in the interface condition \eqref{eq:interfaceTraditional} is lagged by one time step.
After solving the pressure equation for the fluid subject to the boundary condition in~\eqref{eq:rbbcs} and interface condition in~\eqref{eq:balance}, 
the applied force is found to be
%
\begin{equation}
 \ph^{(n+1)^-}(-\hs/2)-\ph^{(n+1)^+}(\hs/2) =-\hat{M}_a^{-}D_{+t}D_{-t}\etah^{n+1}-\hat{M}_{a}^{+}D_{+t}D_{-t}\etah^{n+1},
 \label{eq:appliedForceAMP}
\end{equation}
where the added masses, $\hat{M}_a^\pm$, are given in~\eqref{eq:addedMass}.
%
Substituting the expression for the applied force~\eqref{eq:appliedForceAMP}, with $n+1$ replaced by $n$, into the leap-frog scheme~\eqref{eq:etaLeapFrogAM} gives the difference equation for $\etah^n$, 
\begin{align}
  \left(\rhos\hs+\hat{M}_a^{-}+\hat{M}_a^{+}\right)D_{+t}D_{-t}\etah^{n}& = -\Lt \etah^n,
  \label{eq:etaAMP}
\end{align}
which is analogous to the evolution equation for $\etah(t)$ in~\eqref{eq:beamMotionFT}.  A solution of the form $\etah^n=A^n\etah^0$ is sought which leads to the quadratic polynomial
\begin{align}
  %(A-1)^2(\rhos\hs+\hat{M}_a^{-}+\hat{M}_a^{+})+\dt^2\Lt A=0.
  A^2-2\left(1-\frac{\dt^2\Lt}{2(\rhos\hs+\hat{M}_a^{-}+\hat{M}_a^{+})}\right)A+1=0,
\label{eq:AMP_A} 
\end{align}
%
for the amplitude $A$.  Stability requires $\vert\amp\vert \le 1$ and that the roots be simple, which leads to the following theorem:
% which implies
%$\vert 1-\frac{\Lt\dt^2}{2(\rhos\hs+\hat{M}_a^{+}+\hat{M}_a^{-})} \vert < 1$.
%The following theorem then follows directly.
\begin{theorem}
   The AMP scheme applied to the model problem in~\eqref{eq:MP1} is stable if and only if 
\begin{align}
   \dt <\sqrt{\frac{2(\rhos\hs+\hat{M}_a^{-}+\hat{M}_a^{+})}{\Lt}}, \label{eq:AMPstability}
\end{align}
where $M_a^{\pm}$ is given by~\eqref{eq:addedMass} for case of the rigid-wall BCs and by~\eqref{eq:addedMassPressure} for the case of pressure BCs.  Moreover, if~\eqref{eq:AMPstability} holds, then the roots of~\eqref{eq:AMP_A} satisfy $\vert\amp\vert=1$ and the AMP scheme is non-dissipative.
% When $k=0$, the scheme is non-dissipative. 
\end{theorem}

We note that if a stable time step is chosen for the leap-frog scheme in~\eqref{eq:etaLeapFrogAM} with no external forcing due to the fluid, namely $\dt<\sqrt{2\rhos\hs/\Lt}$, then this value of $\dt$ would be stable for the AMP scheme as well since $M_a^{\pm}\ge0$.
%It is interesting to note that the AMP scheme is stable for a value of $\dt$ satisfying the time-step restriction for the leap-frog scheme for the beam with no fluid present, namely $\dt<\sqrt{2\rhos\hs/\Lt}$.
We also note that a velocity projection has been omitted in the prototype AMP scheme considered in the stability analysis, and thus the fluid and structure velocities 
at the interface would only match to first-order accuracy.  An additional projection step to match the velocities on the interface exactly could be included, but this is not essential for the present analysis.

Having considered the stability of the AMP scheme, we now turn our attention to a TP scheme defined as follows:

% --------------------------------------------------------------------------------------------------------------------------------------
\begin{algorithm}[H] {\bf Traditional partitioned (TP) scheme:}

\noindent Stage I: Advance the beam displacement using~\eqref{eq:etaLeapFrogAM}.

\medskip\noindent
Stage II: Advance the fluid velocity and pressure using~\eqref{eq:fluidAMP} with interface condition,
\begin{equation} 
\frac{\partial \ph^{(n+1)^{\pm}}}{\partial y} = -\rho^{\pm}  D_{+t}D_{-t}\etah^n,  \qquad y=\pm\hs/2, \label{eq:interfaceTraditional}
\end{equation}
and the boundary condition in~\eqref{eq:rbbcs}.
\label{alg:TP}
\end{algorithm}
% --------------------------------------------------------------------------------------------------------------------------------------

The only difference between the AMP scheme and the TP scheme is the coupling at the interface.  For the TP and AMP schemes, the stress from the fluid at time level $t_n$ provides a forcing to the leap-frog scheme in~\eqref{eq:etaLeapFrogAM} to advance the displacement of the beam to time level $t_{n+1}$.  The velocity and pressure in the fluid are then advanced to time level $t_{n+1}$ using the discrete equations in~\eqref{eq:fluidAMP}, the boundary condition in~\eqref{eq:rbbcs} and a coupling condition at the interface.  The AMP scheme uses the coupling condition in~\eqref{eq:AMPinterfaceBC}, whereas the TP scheme uses~\eqref{eq:interfaceTraditional}.  The latter is derived from the time derivative of the kinematic interface condition matching the vertical velocity of the beam to that of the fluid on interface.  We note, however, that a similar interface condition was derived from the leap-frog scheme in~\eqref{eq:etaLeapFrogAM} and the AMP interface coupling condition in~\eqref{eq:AMPinterfaceBC}, which appears in~\eqref{eq:balance}.  The {\em key} difference is that the time level for the vertical acceleration of the beam in~\eqref{eq:interfaceTraditional} lags that of fluid in contrast to~\eqref{eq:balance}, and this is the essential issue leading to the instability of the TP scheme for light structures as the subsequent analysis shows.

Following the steps used in the analysis of the AMP scheme, the pressure equation in \eqref{eq:fluidAMP} is solved with interface conditions in~\eqref{eq:interfaceTraditional} and
boundary conditions in~\eqref{eq:rbbcs} to give the applied force
%
\begin{equation}
 \ph^{(n+1)^-}(-\hs/2)-\ph^{(n+1)^+}(\hs/2) =-\hat{M}_a^{-}D_{+t}D_{-t}\etah^n-\hat{M}_{a}^{+}D_{+t}D_{-t}\etah^n.
 \label{eq:appliedForceTP}
 \end{equation}
Using the beam equation in~\eqref{eq:etaLeapFrogAM} together with~\eqref{eq:appliedForceTP} to eliminate the applied force yields a difference equation for $\etah\sp{n}$ of the form
\begin{align}
  \rhos\hs D_{+t}D_{-t}\etah^{n} +\Big(\hat{M}_a^{-}+\hat{M}_a^{+}\Big)D_{+t}D_{-t}\etah^{n-1}& = -\Lt \etah^n.
\label{eq:etaTraditional} 
\end{align}
Again we observe a time lag in the added-mass terms in~\eqref{eq:etaTraditional} as compated to the previous evolution equation equation for $\etah^n$ in~\eqref{eq:etaAMP} for the AMP scheme. This time-lag is well known and is the primary source of the added-mass instability for the TP scheme.  Using $\etah^n=A^n\etah^0$ in~\eqref{eq:etaTraditional}  leads to the cubic polynomial
\begin{align}
  \rhos\hs A(A-1)^2+\dt^2\Lt A^2+(\hat{M}_a^{-}+\hat{M}_a^{+})(A-1)^2=0.
\label{eq:TP_A} 
\end{align}
The TP scheme is weakly stable if all roots of \eqref{eq:TP_A} satisfy $|A|\le 1$. Using the theory
of von Neumann polynomials \textcolor{red}{(REF???)} leads to the following theorem.
%
\begin{theorem} \label{th:traditional}
  For $\rhos\hs>0$ and $\Lt>0$, the traditional partitioned scheme applied to the model problem in~\eqref{eq:MP1} is weakly stable if and only if
\begin{align}
  \hat{M}_a^{-}+\hat{M}_a^{+} < \rhos\hs \label{eq:TP_addedMassLimit}
\end{align}
  and
\begin{align}
  &  \dt <  2\sqrt{ \frac{\rhos\hs-\hat{M}_a^{-}-\hat{M}_a^{+}}{\Lt}}, \label{eq:traditionalStabLimitII}
\end{align}
where $M_a^{\pm}$ is given by~\eqref{eq:addedMass} for case of the rigid-wall BCs and by~\eqref{eq:addedMassPressure} for the case of pressure BCs.
% when $k\neq 0$ and given by~\eqref{eq:addedMass0modeTP} when $k=0$.
\end{theorem}

\textcolor{red}{Return to the interpretation later}
The condition \eqref{eq:TP_addedMassLimit} implies that the TP scheme is unconditionally unstable if 
the contribution from the added mass is too 
large, i.e.~if $\hat{M}_a^{-}+\hat{M}_a^{+} >\rhos \hs$, regardless of the choice for the time-step, $\dt$.
From~\eqref{eq:addedMass}, we observe that the added-mass is large for large $\rho^{\pm} \ls$, 
small $k$, and/or small $\mathcal{D}^{\pm}/\ls$.  
Thus, the TP scheme has difficulty when the ratio $(\rho \ls)/(\rhos\hs)$ is large, the wave number of 
surface variations is low, and/or the fluid domains are thin.
This is in  agreement with the result of Causin {\it et al.}~\cite{CausinGerbeauNobile2005}, who 
studied a simple beam with fluid on one side.
If the condition $\hat{M}_a^{-}+\hat{M}_a^{+}<\rhos\hs$ is satisfied, then \eqref{eq:traditionalStabLimitII} indicates how the time-step 
must be scaled reduced as the total added-mass increases.


%%%%%
%%%%%
%%%%%


\subsubsection{Regularization of the Pressure Equation for $k=0$}
Note that for both the TP and AMP schemes the limit $k=0$ must be treated with some care.
For this case the pressures are only determined up to an arbitrary constant 
as for the continuous case~\eqref{eq:kZeroContinuous}-\eqref{eq:kZeroPressureDiff}.
However, at the discrete level there is an additional subtlety when $k=0$ in that the pressure equations for $p^+$ and $p^-$ 
are both singular. In a numerical implementation these singularities need to be removed since, due to round-off or truncation
errors the singular systems may have no solution. The specific choice of regularization can effect the overall stability
of the approach. For example, one common regularization would follow the approach in~\cite{splitStep2003},
which for $k=0$ would solve the augmented pressure equation 
\begin{align*}
   & \frac{\partial^2 \ph^{(n+1)\pm}}{\partial y^2} +\alpha^{(n+1)\pm} =0,\\
    &\int_{\Hf^{-}}^{-\hs/2} \ph^{(n+1)-}dy=\int^{\Hf^{+}}_{\hs/2} \ph^{(n+1)+}dy  = 0.
\end{align*}
Here $\alpha^{(n+1)\pm}$ are two additional unknowns which serve to regularize the solution and ensure that the augmented 
system has a unique solution. The effect of regularization can be significant for the $k=0$ mode. For example, using this
regularization the traditional partitioned scheme is found to be stable for the $k=0$ mode under the mollified time-step restriction
\[
  \dt <  2\sqrt{ \frac{\rhos\hs-\frac{1}{3} \rho^{-}\mathcal{D}^{-}-\frac{1}{3} \rho^{+}\mathcal{D}^{+}}{\Lt}}.
\]
This is significant difference from \eqref{eq:traditionalStabLimitII} which requires $\dt\to 0$ when
$k\to 0$. This less severe time-step restriction is a result of the pressure regularization
and applies only to the $k=0$ mode. All other
small $k$ modes in the system must satisfy \eqref{eq:traditionalStabLimitII}. Similarly, 
using the same pressure regularization in the AMP scheme it can be shown that 
for $k=0$ the AMP scheme is stable under the restriction
\[
  \dt <2 \sqrt{\frac{\rhos\hs+\frac{1}{3} \rho^{-}\mathcal{D}^{-}+\frac{1}{3} \rho^{+}\mathcal{D}^{+}}{\Lt}}.
\]
Other choices of pressure regularization are likely to result in different behavior for the $k=0$ mode.  

%%%%%
%%%%%
\subsection{Pressure Boundary Condition}
The analysis of the model problem with pressure boundary conditions at $y=\Hf^{\pm}$ is quite similar to the
slip wall case in Section~\ref{subsec:slipWallBCs}. In fact, the only substantive difference is that the
analytic form of the added-mass changes. The analysis uses the same Fourier decomposition
in the $x$ direction to yield the model \eqref{eq:modelFluidEquationFT} and \eqref{eq:modelShellEquationFT}. 
In this case we seek solutions to the pressure equation using the form 
\begin{equation}
  \ph^{\pm} = a^{\pm}\sinh\left(k_x(y-H^{\pm})\right) +b^{\pm}\sinh\left(k_x(y\mp h/2)\right). \label{eq:pSolutionN}
\end{equation}
The pressure boundary condition $p^{\pm}(y=\Hf^{\pm})=0$ implies $b^{\pm}=0$, and the two interface conditions
\eqref{eq:modelInterfaceFTpy} are then used to give 
\[
  a^{\pm} = -\frac{\rho^{\pm}}{k_x}\frac{\partial^2\etah}{\partial t^2}\frac{1}{\cosh\left(k_x(\pm h/2-H^{\pm})\right)}.
\]
This leads directly to \eqref{eq:appliedForceFT} but where the added masses are now given as 
\begin{equation}
  \hat{M}_a^{-} =\frac{\rho^{-}}{k_x}\tanh(k_x\mathcal{D}^{-}),~{\rm and}~ \hat{M}_a^{+} =\frac{\rho^{+}}{k_x}\tanh(k_x\mathcal{D}^{+}).
  \label{eq:addedMassN}
\end{equation}
The remainder of the analysis and the two theorems regarding stability of the TP and AMP schemes then follow without further
modification. The form of the added mass in \eqref{eq:addedMassN} shows that pressure boundary conditions
at the fluid extremities are in some sense easier than the slip wall BCs since in \eqref{eq:addedMassN} the
added mass approaches zero as the wave number goes to zero while in \eqref{eq:addedMass} the added
mass increases in an unbounded manner. This result has been observed in the literature
where it is well documented that the most difficult case for partitioned FSI is when a long beam is placed
near a rigid wall. 

==> texFiles/analysis-orig.tex <==
%---------------------------------------------------------------------
\section{Analysis of a model problem for a beam with fluid on two sides} \label{sec:analysis}
{% ------ linearizedTwoSidedBeam ------
\newcommand{\figWidth}{8cm}
\newcommand{\trimfig}[2]{\trimFig{#1}{#2}{0}{0}{0}{0}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.0,0) rectangle (8cm,8cm);  % set the bounding box (so we have less surrounding white space)
%   \draw(0.0,4.4) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/fc2Gridt0p010}{\figWidth}};
  \draw(0.0,0.0) node[anchor=south west,xshift=0pt,yshift=0pt] {\trimfig{fig/linearizedTwoSidedBeam.pdf}{\figWidth}};
% grid:
%  \draw[step=1cm,gray] (0,0) grid (16,5);
\end{tikzpicture}
\end{center}
  \caption{The geometry of the linearized model  for  a beam with fluid on two sides.}
  \label{fig:linearizedTwoSidedBeam}
\end{figure}
}

Notes: 

-wdh: Fig. 2: do you have the latex source we can use instead if the pdf? need to change L to $\ls$

In this section, the stability of a traditional partitioned (TP) and the new added-mass
partitioned schemes are investigated for a linearized model problem consisting of a beam coupled to two fluid domains as shown in
Figure~\ref{fig:linearizedTwoSidedBeam}. The problem is first analysed 
at the continuous level to explicitly identify the 
added-mass. The stability of the discrete schemes is then investigated using a mode analysis that
extends the theory presented in~\cite{fis2014} for the case of a beam with fluid on only one side.
 For both the TP and AMP schemes, the fluid
equations are advanced using a backward-Euler time integrator as opposed to the predictor-corrector integrator
described in Section~\ref{sec:AMPalgorithm}.  While this simplifies the analysis somewhat, the essential results are unaffected.  As
expected, it is found that the traditional scheme without iteration becomes unconditionally unstable for light structures.  The AMP scheme, in contrast,
remains stable for arbitrarily light structures provided the usual convective time-step restriction is satisfied.  Note that the traditional partitioned scheme has been analyzed previously by Causin, Gerbeau
and Nobile~\cite{CausinGerbeauNobile2005}, among others, and the results presented here extend those works.


In the following analysis the two fluids are assumed to be inviscid and incompressible, and are coupled to a
simple acoustic beam. The equations describing the evolution of the fluid-structure system are then linearized 
about a flat interface as shown in Figure~\ref{fig:linearizedTwoSidedBeam}.
Let $\rho^+$, $\vv^+$ and $p^+$, denote the fluid density, velocity and pressure in the upper domain, $\OmegaF_{+}$, 
and $\rho^-$, $\vv^-$ and $p^-$, the corresponding values in the lower domain $\OmegaF_{-}$.
The governing equations and boundary conditions for this model are 
\begin{equation*}
\begin{aligned}
& \text{Fluid:} \quad \left\{ 
   \begin{alignedat}{3}
  &  \rho^{\pm}\frac{\partial\vv^{\pm}}{\partial t} 
                 + \grad p^{\pm} =0, \qquad&& \xv\in\OmegaF_{\pm} ,  \\
  & \grad\cdot\vv^{\pm} =0,  \qquad&& \xv\in\OmegaF_{\pm} ,   \\
  & v_2^{\pm}(y=\Hf^{\pm})=0~~\text{or}~~ p^{\pm}(y=\Hf^{\pm})=0  , \quad&& x\in(0,\ls), 
   \end{alignedat}  \right. % \label{eq:MP1v}
%
\\ 
& \text{Beam:}\quad  \left\{ 
   \begin{alignedat}{3}
  &  \rhos\hs\frac{\partial^2\eta}{\partial t^2}  = -\Ks_0 \eta + \Ts\frac{\partial^2\eta}{\partial x^2} - \Es\Is\frac{\partial^4\eta}{\partial x^4} + p^{-}(y=-\hs/2) - p^{+}(y=\hs/2), \qquad&&  x\in(0,\ls), % x\in\OmegaS,
   \end{alignedat}  \right. \\
& \text{Interface:}\quad   v_2^{\pm}(y=\pm\hs/2)=\frac{\partial\eta}{\partial t}, \qquad  x\in(0,\ls), % x\in\OmegaS .
% 
\end{aligned}
  \label{eq:MP1}
\end{equation*}
with periodic boundary conditions in the $x$-direction. 
The beam has length $\ls$ and constant thickness $\hs$, breadth $\bs=1$, and has reference-line along $y=0$. 
The fluid in the lower domain occupies the region $\OmegaF_-=[0,\ls]\times[\Hf^{-},-\hs/2]$, while the domain of the  fluid
in the upper part  is $\OmegaF_+=[0,\ls]\times[\hs/2,\Hf^{+}]$. 
Here  $y=\pm\hs/2$ are the locations of the interfaces separating the beam from the
upper and lower fluid, respectively.
Initial conditions for $\vv^\pm$, $\eta$ and $\eta_t$ complete the specification of the problem. 
% 
% To begin the analysis, the solution is expanded in a finite Fourier series in $x$ (i.e.~a pseudo-spectral approximation), which gives 


%%%%%
%% slip wall BCs
%%%%%
\subsection{Slip Wall Boundary Conditions}
\label{subsec:slipWallBCs}
Let us first examine the case of slip wall boundary conditions on the top and bottom at $y=H^{\pm}$.
The solution to this linearized FSI model can be obtained by expansion in Fourier series in the periodic direction. 
Note that the transformed quantity will be denoted using a hat (e.g. $\vvh^{\pm}(k,y,t)=\int_{-\infty}^{\infty}\vv^{\pm}(x,y,t)\exp[-2\pi i k x]\, dx$).
The governing equations for the Fourier components corresponding to a given wavenumber $k$ are
\begin{equation}
\left. \begin{array}{r}
\displaystyle{
  \rho^{\pm} \frac{\partial \vh_1^{\pm}}{\partial t} + i\kx \ph^{\pm} =0
} \smallskip\\
\displaystyle{
  \rho^{\pm} \frac{\partial \vh_2^{\pm}}{\partial t} + \frac{\partial \ph^{\pm}}{\partial y} =0
} \smallskip\\
\displaystyle{
  \frac{\partial^2 \ph^{\pm}}{\partial y^2} - \kx^2 \ph^{\pm} =0
}
\end{array}
\right\},
\begin{array}{l}
  \qquad y \in (\Hf^{-},-\frac{\hs}{2})\ \hbox{ for the lower fluid},\\
  \qquad y \in (\frac{\hs}{2},\Hf^{+}) \hbox{ \hspace{0.165in}for the upper fluid},\\
\end{array}
\label{eq:modelFluidEquationFT}
\end{equation}
 and
\begin{equation}
  \rhos\hs \frac{\partial ^2\etah}{\partial t^2} = - \Lt \etah + \ph^{-}(y=-\hs/2)-\ph^{+}(y=\hs/2),  \mathrm{~ for~the~beam}.
\label{eq:modelShellEquationFT}
\end{equation}
Here $\kx = 2\pi k/\ls$, $\Lt=\Ks_0+\Ts\kx^2+\Es\Is\kx^4$, 
and for notational brevity we have suppress functional dependence on wavenumber $k$.
 
The solution of the pressure equation in the fluid system (\ref{eq:modelFluidEquationFT}) can be written
\begin{equation}
  \ph^{\pm} = a^{\pm}\cosh\left(k_x(y-H^{\pm})\right) +b^{\pm}\cosh\left(k_x(y\mp h/2)\right), \label{eq:pSolution}
\end{equation}
with time-dependent coefficients $a^{\pm}$ and $b^{\pm}$ that  are determined
by the boundary and interface conditions. 
The slip wall boundary conditions for the fluids at $y=\Hf^{\pm}$ are $\vh_2^{\pm}=0$,
which in combination with the momentum equation implies
\begin{equation}
  \frac{\partial \ph^{\pm}}{\partial y}(y=\Hf^{\pm})=0.
  \label{eq:modelBCFT}
\end{equation}
It follow that $b^{\pm}=0$. The kinematic condition at the fluid-structure interfaces, 
$\vh_2^{\pm}(y=\pm\hs/2)=\frac{\partial\etah}{\partial t}$, implies the acceleration condition
$\frac{\partial \vh_2^{\pm}}{\partial t}(y=\pm\hs/2)=\frac{\partial^2\etah}{\partial t^2}.$
Using the fluid momentum equation in the $y$ direction then gives the two interface conditions
\begin{equation}
  \frac{\partial \ph^{\pm}}{\partial y}(y=\pm\hs/2)=  -\rho^{\pm}\frac{\partial^2\etah}{\partial t^2}.
  \label{eq:modelInterfaceFTpy}
\end{equation}
Therefore $a^{\pm}$ are given as
\[
  a^{\pm} = -\frac{\rho^{\pm}}{k_x}\frac{\partial^2\etah}{\partial t^2}\frac{1}{\sinh\left(k_x(\pm h/2-H^{\pm})\right)}.
\]
The applied force appearing in the beam equation can then be written in the form
\begin{equation}
 \ph^{-}(y=-\hs/2)-\ph^{+}(y=\hs/2) =-\hat{M}_a^{-}\frac{\partial^2\etah}{\partial t^2}-\hat{M}_{a}^{+}\frac{\partial^2\etah}{\partial t^2},
 \label{eq:appliedForceFT}
\end{equation}
where $\hat{M}_{a}^{\pm}$ are the added-mass coefficients for the upper and lower fluids defined as
\begin{equation}
  \hat{M}_a^{-} =\frac{\rho^{-}}{k_x}\coth(k_x\mathcal{D}^{-}),~{\rm and}~ \hat{M}_a^{+} =\frac{\rho^{+}}{k_x}\coth(k_x\mathcal{D}^{+}).
  \label{eq:addedMass}
\end{equation}
Here $\mathcal{D}^{-}=-\hs/2-\Hf^{-}$ and $\mathcal{D}^{+}=\Hf^{+}-\hs/2$ are the extents of the lower and upper fluid domains, respectively.  
Finally, using the applied force (\ref{eq:appliedForceFT}) in the equation of motion
for the beam (\ref{eq:modelShellEquationFT}) gives
\begin{equation}
 \Big( \rhos\hs+\hat{M}_a^{-}+\hat{M}_a^{+}\Big) \frac{\partial ^2\etah}{\partial t^2} = - \Lt \etah,
 \label{eq:beamMotionFT}
\end{equation}
which explicitly identifies the effect of the added-mass in the beam equation. Equation \eqref{eq:beamMotionFT} can easily be solved
in concert with the initial conditions for $\etah$ and $\etah_t$ to complete the Fourier space solution to the model problem.
Note that $\hat{M}_a^{\pm} >0$ and so the added mass associated with the fluids always tends to suppress 
beam acceleration. Indeed, $\hat{M}_a^{\pm}\to\infty$ as $k\to 0$ which indicates that the $k=0$ mode will be the most sensitive
to added-mass effects. In fact for $k=0$ the solution is independent of time and takes the form {\bf check this}
\begin{align}
  & \vh_2(k=0,y,t)^{\pm}=0,\qquad \ph^{\pm}(k=0,y,t) = p_0^\pm,   \label{eq:kZeroContinuous} \\
  & \Ks_0\etah(k=0,t) = p_0^- - p_0^+,  \label{eq:kZeroPressureDiff}
\end{align}
where $p_0^\pm$ are constants (not independent) that balance the initial displacement of the beam through 
through~\eqref{eq:kZeroPressureDiff}. 
The solution is thus determined up to a single constant in the pressure which has no consequential effect on the answer. 
To define a unique solution one additional constraint is needed
such as requiring the mean value of the pressure to be zero.

%%%%%
%% partitioned numerics
%%%%%
\subsubsection{Stability of Discrete Coupling Schemes}
To isolate the effect of different discrete treatments of the interface conditions, and in particular the existence or nonexistence
of added-mass type instabilities, the governing system (\ref{eq:modelFluidEquationFT})-(\ref{eq:modelShellEquationFT}) 
is discretized in time with spatial coordinate $y$  left continuous.
Note that the analysis presented here can be extended to fully discrete in $y$ without undue conceptual difficulty but at the cost
of increased algebraic complexity. Note also that the details of the stability analysis may depend somewhat on the 
particulars of the spatial discretization. Let
\[
\vvh^{n\pm}\approx\vvh^{\pm}(t=t^n), \qquad \ph^{n\pm}\approx\ph^{\pm}(t=t^n), \qquad \etah^{n}\approx\etah(t=t^n),
\]
 where $t^n=n\dt$. Furthermore, let $D_{+t}$ and $D_{-t}$ denote the forward and backward divided different operators in time 
(e.g. $D_{+t}\etah^n=(\etah^{n+1}-\etah^n)/\dt$ and $D_{-t}\etah^n=(\etah^{n}-\etah^{n-1})/\dt$).  

% --------------------------------------------------------------------------------------------------------------------------------------
\begin{algorithm}[H] {\bf Traditional partitioned (TP) scheme:}

\noindent Stage I: Advance the shell displacements using a leap-frog scheme:
\begin{align}
  \rhos\hs D_{+t}D_{-t}\etah^n & = -\Lt \etah^n + \ph^{n-}(y=-\hs/2)-\ph^{n+}(y=\hs/2) . \label{eq:etaLeapFrog}
%  \rhos\hs\frac{\etah^{n+1}-2\etah^n+\etah^{n-1}}{\dt^2} & = -\Lt \hs \etah^n + \ph^n(k,H) , \label{eq:etaLeapFrog}
\end{align}
Stage II: Advance the fluid velocity and pressure using a backward-Euler scheme,
\begin{equation}
\left. \begin{array}{r}
\displaystyle{
% \rho^{\pm} \frac{\vh_1^{(n+1)\pm}-\vh_1^{n\pm}}{\dt}  + i\kx \ph^{(n+1)\pm} =0
\rho^{\pm} D_{+t}\vh_1^{n\pm}  + i\kx \ph^{(n+1)\pm} =0
} \smallskip\\
\displaystyle{
% \rho^{\pm} \frac{\vh_2^{(n+1)\pm}-\vh_2^{n\pm}}{\dt} + \frac{\partial \ph^{(n+1)\pm}}{\partial y} =0
\rho^{\pm} D_{+t}\vh_2^{n\pm} + \frac{\partial \ph^{(n+1)\pm}}{\partial y} =0
} \smallskip\\
\displaystyle{
\frac{\partial^2 \ph^{(n+1)\pm}}{\partial y^2} - \kx^2 \ph^{(n+1)\pm} =0
}
\end{array} \right\},
\begin{array}{l}
  \qquad y \in (\Hf^{-},-\frac{\hs}{2}) \hbox{ for the lower fluid},\\
  \qquad y \in (\frac{\hs}{2},\Hf^{+}) \hbox{ \hspace{0.13in}for the upper fluid},\\
\end{array}
\label{eq:fhat}
\end{equation}
with interface condition,
\begin{equation} 
\frac{\partial \ph^{(n+1)^{\pm}}}{\partial y}(y=\pm\hs/2) = -\rho^{\pm}  D_{+t}D_{-t}\etah^n,  \label{eq:interfaceTraditional}
\end{equation}
and boundary condition,
\begin{equation} 
\frac{\partial \ph^{(n+1)\pm}}{\partial y}(y=\Hf^{\pm})=0.  \label{eq:pressureBCTraditional}
\end{equation}
\label{alg:TP}
\end{algorithm}
% --------------------------------------------------------------------------------------------------------------------------------------
\noindent
{\bf Traditional Partitioned Scheme:} Solutions to the TP scheme can be determined following similar steps to those used above for the continuous-in-time solution.
Solving the pressure equation in \eqref{eq:fhat} with interface conditions \eqref{eq:interfaceTraditional} and
boundary conditions \eqref{eq:pressureBCTraditional} yields the applied force
%
\begin{equation}
 \ph^{(n+1)^-}(y=-\hs/2)-\ph^{(n+1)^+}(y=\hs/2) =-\hat{M}_a^{-}D_{+t}D_{-t}\etah^n-\hat{M}_{a}^{+}D_{+t}D_{-t}\etah^n.
 \label{eq:appliedForceTP}
 \end{equation}
A difference equation for $\etah$ can therefore be written as
\begin{align}
  \rhos\hs D_{+t}D_{-t}\etah^{n} +\Big(\hat{M}_a^{+}+\hat{M}_a^{-}\Big)D_{+t}D_{-t}\etah^{n-1}& = -\Lt \etah^n.
\label{eq:etaTraditional} 
\end{align}
The stability of the TP scheme 
is encapsulated in the stability of~\eqref{eq:etaTraditional}.
Notice that the application of the discrete TP interface condition~\eqref{eq:interfaceTraditional} results
in the added mass term being applied with a one time-step lag. This time-lag is well known and turns out to 
be the primary source of the added-mass instability for the TP algorithm. As in~\cite{fis2014}, solutions
to \eqref{eq:etaTraditional} of the form $\etah^n=A^n\etah^0$ are sought which leads to the cubic polynomial
\begin{align}
  \rhos\hs A(A-1)^2+\dt^2\Lt A^2+(\hat{M}_a^{-}-\hat{M}_a^{+})(A-1)^2=0.
\label{eq:TP_A} 
\end{align}
The TP scheme is weakly stable if all roots of \eqref{eq:TP_A} satisfy $|A|\le 1$. Using the theory
of von Neumann polynomials leads to the following theorem.
%
\begin{theorem} \label{th:traditional}
  For $\rhos\hs>0$ and $\Lt>0$, the traditional partitioned scheme is weakly stable if and only if
\begin{align}
  \hat{M}_a^{+}+\hat{M}_a^{-} < \rhos\hs \label{eq:TP_addedMassLimit}
\end{align}
  and
\begin{align}
  &  \dt <  2\sqrt{ \frac{\rhos\hs-\hat{M}_a^{-}-\hat{M}_a^{+}}{\Lt}}, \label{eq:traditionalStabLimitII}
\end{align}
where $\hat{M}_a^{\pm}$ are given by~\eqref{eq:addedMass} .% when $k\neq 0$ and given by~\eqref{eq:addedMass0modeTP} when $k=0$.
\end{theorem}

The condition \eqref{eq:TP_addedMassLimit} implies that the TP scheme is unconditionally unstable if 
the contribution from the added mass is too 
large, i.e.~if $\hat{M}_a^{-}+\hat{M}_a^{+} >\rhos \hs$, regardless of the choice for the time-step, $\dt$.
From~\eqref{eq:addedMass}, we observe that the added-mass is large for large $\rho^{\pm} \ls$, 
small $k$, and/or small $\mathcal{D}^{\pm}/\ls$.  
Thus, the TP scheme has difficulty when the ratio $(\rho \ls)/(\rhos\hs)$ is large, the wave number of 
surface variations is low, and/or the fluid domains are thin.
This is in  agreement with the result of Causin {\it et al.}~\cite{CausinGerbeauNobile2005}, who 
studied a simple beam with fluid on one side.
If the condition $\hat{M}_a^{-}+\hat{M}_a^{+}<\rhos\hs$ is satisfied, then \eqref{eq:traditionalStabLimitII} indicates how the time-step 
must be scaled reduced as the total added-mass increases.


%%%%%
%%%%%
%%%%%

% --------------------------------------------------------------------------------------------------------------------------------------
\begin{algorithm}[H] {\bf AMP scheme:} 

\noindent Stage I: Advance the shell displacement using a leap-frog scheme (as in the traditional scheme),
\begin{equation}
  \rhos\hs D_{+t}D_{-t}\etah^n  = -\Lt \etah^n + \ph^{n-}(y=-\hs/2)-\ph^{n+}(y=\hs/2) .
\label{eq:etaLeapFrogAM}
\end{equation}
Stage II: Advance the fluid velocity and pressure using a backward-Euler scheme (as in the traditional scheme),
\[
\left. \begin{array}{r}
\displaystyle{
% \rho^{\pm} \frac{\vh_1^{(n+1)\pm}-\vh_1^{n\pm}}{\dt}  + i\kx \ph^{(n+1)\pm} =0
\rho^{\pm} D_{+t} \vh_1^{n\pm}  + i\kx \ph^{(n+1)\pm} =0
} \smallskip\\
\displaystyle{
% \rho^{\pm} \frac{\vh_2^{(n+1)\pm}-\vh_2^{n\pm}}{\dt} + \frac{\partial \ph^{(n+1)\pm}}{\partial y} =0
\rho^{\pm} D_{+t} \vh_2^{n\pm} + \frac{\partial \ph^{(n+1)\pm}}{\partial y} =0
} \smallskip\\
\displaystyle{
\frac{\partial^2 \ph^{(n+1)\pm}}{\partial y^2} - \kx^2 \ph^{(n+1)\pm} =0
}
\end{array} \right\},
\begin{array}{l}
  \qquad y \in (\Hf^{-},-\frac{\hs}{2}) \hbox{ for the lower fluid},\\
  \qquad y \in (\frac{\hs}{2},\Hf^{+}) \hbox{ \hspace{0.125in}for the upper fluid},\\
\end{array}
\]
with the AMP Robin interface condition, derived from \eqref{eq:AMPpressureBCI} and \eqref{eq:AMPpressureBCII},
\begin{equation}
\ph^{(n+1)-}(y=-\hs/2)-\ph^{(n+1)+}(y=+\hs/2) + \frac{\rhos\hs}{\rho^{\pm}} \frac{\partial \ph^{(n+1)\pm}}{\partial y}(y=\pm\hs/2) = \Lt \etah^{n+1},
\label{eq:AMPinterfaceBC}
\end{equation}
and boundary conditions.
\[
\frac{\partial \ph^{(n+1)\pm}}{\partial y}(y=\Hf^{\pm})=0.
\]
\label{alg:AMP}
\end{algorithm}
% --------------------------------------------------------------------------------------------------------------------------------------
\noindent
{\bf Added-Mass Partitioned Scheme:} The stability of the AMP coupling scheme is now investigated. One key ingredient of the AMP scheme is the 
Robin condition in~\eqref{eq:AMPinterfaceBC} for the fluid pressure. This condition implies
\[
\frac{\partial \ph^{(n+1)^{\pm}}}{\partial y}(y=\pm\hs/2) = -\rho^{\pm}  D_{+t}D_{-t}\etah^{n+1},
\]
where the acceleration term on the right-hand-side is at the same time level as the left-hand-side.
This is in contrast to the traditional scheme where the acceleration term in the interface condition \eqref{eq:interfaceTraditional}
is lagged by one time step. As a result, after solving the pressure equation with interface conditions \eqref{eq:AMPinterfaceBC} 
the applied force is found to be
%
\begin{equation}
 \ph^{(n+1)^-}(y=-\hs/2)-\ph^{(n+1)^+}(y=\hs/2) =-\hat{M}_a^{-}D_{+t}D_{-t}\etah^{n+1}-\hat{M}_{a}^{+}D_{+t}D_{-t}\etah^{n+1}.
 \label{eq:appliedForceAMP}
\end{equation}
%
Therefore, the difference equation for $\etah$ is 
\begin{align}
  \rhos\hs D_{+t}D_{-t}\etah^n +\Big(\hat{M}_a^{-}+\hat{M}_a^{+}\Big)D_{+t}D_{-t}\etah^{n}& = -\Lt \etah^n.
  \label{eq:etaAMP}
\end{align}
As before, solution of the form $\etah^n=A^n\etah^0$ are sought which leads to the quadratic polynomial
\begin{align}
  %(A-1)^2(\rhos\hs+\hat{M}_a^{-}+\hat{M}_a^{+})+\dt^2\Lt A=0.
  A^2-2\left(1-\frac{\dt^2\Lt}{2(\rhos\hs+\hat{M}_a^{-}-\hat{M}_a^{+})}\right)A+1=0.
\label{eq:AMP_A} 
\end{align}
%
Stability requires $\vert\amp\vert \le 1$ and that the roots be simple which implies
$\vert 1-\frac{\Lt\dt^2}{2(\rhos\hs+\hat{M}_a^{+}+\hat{M}_a^{-})} \vert < 1$.  
The following theorem then follows directly.
\begin{theorem}
   The added-mass partitioned scheme is stable if and only if 
\begin{align}
   \dt <2 \sqrt{\frac{\rhos\hs+\hat{M}_a^{+}+\hat{M}_a^{-}}{\Lt}}. \label{eq:AMPstability}
\end{align}
%where $M_a^{\pm}$ is given by~\eqref{eq:addedMass}. 
% When $k=0$, the scheme is non-dissipative. 
\end{theorem}

It is interesting to realize that the AMP algorithm  is stable when using the time-step restriction that arises when advancing the shell with no 
fluid present (i.e.~taking $\hat{M}_a^{+}+\hat{M}_a^{-}=0$ in~\eqref{eq:AMPstability}).  For this case the amplification factor 
satisfies $\vert\amp\vert=1$ and the scheme is non-dissipative.  Finally, for this simple AMP scheme, the fluid and shell velocities 
at the interface only match to first-order accuracy. As noted previously, one
could include an additional projection step to match the velocities on the interface exactly.

\subsubsection{Regularization of the Pressure Equation for $k=0$}
Note that for both the TP and AMP schemes the limit $k=0$ must be treated with some care.
For this case the pressures are only determined up to an arbitrary constant 
as for the continuous case~\eqref{eq:kZeroContinuous}-\eqref{eq:kZeroPressureDiff}.
However, at the discrete level there is an additional subtlety when $k=0$ in that the pressure equations for $p^+$ and $p^-$ 
are both singular. In a numerical implementation these singularities need to be removed since, due to round-off or truncation
errors the singular systems may have no solution. The specific choice of regularization can effect the overall stability
of the approach. For example, one common regularization would follow the approach in~\cite{splitStep2003},
which for $k=0$ would solve the augmented pressure equation 
\begin{align*}
   & \frac{\partial^2 \ph^{(n+1)\pm}}{\partial y^2} +\alpha^{(n+1)\pm} =0,\\
    &\int_{\Hf^{-}}^{-\hs/2} \ph^{(n+1)-}dy=\int^{\Hf^{+}}_{\hs/2} \ph^{(n+1)+}dy  = 0.
\end{align*}
Here $\alpha^{(n+1)\pm}$ are two additional unknowns which serve to regularize the solution and ensure that the augmented 
system has a unique solution. The effect of regularization can be significant for the $k=0$ mode. For example, using this
regularization the traditional partitioned scheme is found to be stable for the $k=0$ mode under the mollified time-step restriction
\[
  \dt <  2\sqrt{ \frac{\rhos\hs-\frac{1}{3} \rho^{-}\mathcal{D}^{-}-\frac{1}{3} \rho^{+}\mathcal{D}^{+}}{\Lt}}.
\]
This is significant difference from \eqref{eq:traditionalStabLimitII} which requires $\dt\to 0$ when
$k\to 0$. This less severe time-step restriction is a result of the pressure regularization
and applies only to the $k=0$ mode. All other
small $k$ modes in the system must satisfy \eqref{eq:traditionalStabLimitII}. Similarly, 
using the same pressure regularization in the AMP scheme it can be shown that 
for $k=0$ the AMP scheme is stable under the restriction
\[
  \dt <2 \sqrt{\frac{\rhos\hs+\frac{1}{3} \rho^{-}\mathcal{D}^{-}+\frac{1}{3} \rho^{+}\mathcal{D}^{+}}{\Lt}}.
\]
Other choices of pressure regularization are likely to result in different behavior for the $k=0$ mode.  

%%%%%
%%%%%
\subsection{Pressure Boundary Condition}
The analysis of the model problem with pressure boundary conditions at $y=\Hf^{\pm}$ is quite similar to the
slip wall case in Section~\ref{subsec:slipWallBCs}. In fact, the only substantive difference is that the
analytic form of the added-mass changes. The analysis uses the same Fourier decomposition
in the $x$ direction to yield the model \eqref{eq:modelFluidEquationFT} and \eqref{eq:modelShellEquationFT}. 
In this case we seek solutions to the pressure equation using the form 
\begin{equation}
  \ph^{\pm} = a^{\pm}\sinh\left(k_x(y-H^{\pm})\right) +b^{\pm}\sinh\left(k_x(y\mp h/2)\right). \label{eq:pSolutionN}
\end{equation}
The pressure boundary condition $p^{\pm}(y=\Hf^{\pm})=0$ implies $b^{\pm}=0$, and the two interface conditions
\eqref{eq:modelInterfaceFTpy} are then used to give 
\[
  a^{\pm} = -\frac{\rho^{\pm}}{k_x}\frac{\partial^2\etah}{\partial t^2}\frac{1}{\cosh\left(k_x(\pm h/2-H^{\pm})\right)}.
\]
This leads directly to \eqref{eq:appliedForceFT} but where the added masses are now given as 
\begin{equation}
  \hat{M}_a^{-} =\frac{\rho^{-}}{k_x}\tanh(k_x\mathcal{D}^{-}),~{\rm and}~ \hat{M}_a^{+} =\frac{\rho^{+}}{k_x}\tanh(k_x\mathcal{D}^{+}).
  \label{eq:addedMassN}
\end{equation}
The remainder of the analysis and the two theorems regarding stability of the TP and AMP schemes then follow without further
modification. The form of the added mass in \eqref{eq:addedMassN} shows that pressure boundary conditions
at the fluid extremities are in some sense easier than the slip wall BCs since in \eqref{eq:addedMassN} the
added mass approaches zero as the wave number goes to zero while in \eqref{eq:addedMass} the added
mass increases in an unbounded manner. This result has been observed in the literature
where it is well documented that the most difficult case for partitioned FSI is when a long beam is placed
near a rigid wall. 

==> texFiles/analysisOld.tex <==
%---------------------------------------------------------------------
\section{Analysis of a model problem for a beam with fluid on two sides} \label{sec:analysis}
{% ------ linearizedTwoSidedBeam ------
\newcommand{\figWidth}{8cm}
\newcommand{\trimfig}[2]{\trimFig{#1}{#2}{0}{0}{0}{0}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.0,0) rectangle (8cm,8cm);  % set the bounding box (so we have less surrounding white space)
%   \draw(0.0,4.4) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/fc2Gridt0p010}{\figWidth}};
  \draw(0.0,0.0) node[anchor=south west,xshift=0pt,yshift=0pt] {\trimfig{fig/linearizedTwoSidedBeam.pdf}{\figWidth}};
% grid:
%  \draw[step=1cm,gray] (0,0) grid (16,5);
\end{tikzpicture}
\end{center}
  \caption{The geometry of the linearized model  for  a beam with fluid on two sides.}
  \label{fig:linearizedTwoSidedBeam}
\end{figure}
}

Notes: 

-wdh: Fig. 2: do you have the latex source we can use instead if the pdf? need to change L to $\ls$

%-wdh: Jeff does not like first person ``we'' and I have been removing these

In this section, a mode analysis is used to study the stability of a traditional partitioned (TP) scheme and the new added-mass
partitioned scheme for a linearized model problem consisting of a beam coupled to two fluid domains as shown in
Figure~\ref{fig:linearizedTwoSidedBeam}. The problem is first analysed 
at the continuous level to explicitly identify the added-mass
term, and then the stability of the discrete schemes is investigated.
This analysis is an
extension of that developed in~\cite{fis2014} for the case of a beam with fluid on one side. 
 For both schemes, the fluid
equations are advanced using a backward-Euler scheme as opposed to the predictor-corrector 
time-stepping scheme used in the AMP algorithm
described in Section~\ref{sec:AMPalgorithm}.  While this simplifies the analysis somewhat, the essential results are unaffected.  As
expected, it is found that the traditional scheme becomes unconditionally unstable for light structures.  The AMP scheme, in contrast,
remains stable for arbitrarily light structures provided a time-step restriction is satisfied.  The traditional partitioned scheme has been analyzed previously by Causin, Gerbeau
and Nobile~\cite{CausinGerbeauNobile2005}, among others. The results here extend that work.


The fluids, assumed to be inviscid and incompressible, are coupled to a
simple beam. The equations are linearized about a flat interface as shown in Figure~\ref{fig:linearizedTwoSidedBeam}.
Let $\rho^+$, $\vv^+$ and $p^+$, denote the fluid density, velocity and pressure in the upper domain, $\OmegaF_{+}$, 
and $\rho^-$, $\vv^-$ and $p^-$, the corresponding values in the lower domain $\OmegaF_{-}$.
The governing equations and boundary conditions are 
\begin{equation*}
\begin{aligned}
& \text{Fluid:} \quad \left\{ 
   \begin{alignedat}{3}
  &  \rho^{\pm}\frac{\partial\vv^{\pm}}{\partial t} 
                 + \grad p^{\pm} =0, \qquad&& \xv\in\OmegaF_{\pm} ,  \\
  & \grad\cdot\vv^{\pm} =0,  \qquad&& \xv\in\OmegaF_{\pm} ,   \\
  & v_2^{\pm}(x,\Hf^{\pm},t)=0~~\text{or}~~ p^{\pm}(x,\Hf^{\pm},t)=0  , \quad&& x\in(0,\ls), 
   \end{alignedat}  \right. % \label{eq:MP1v}
%
\\ 
& \text{Beam:}\quad  \left\{ 
   \begin{alignedat}{3}
  &  \rhos\hs\frac{\partial^2\eta}{\partial t^2}  = -\Ks_0 \eta + \Ts\frac{\partial^2\eta}{\partial x^2} - \Es\Is\frac{\partial^4\eta}{\partial x^4} + p^{-}(x,-\hs/2,t) - p^{+}(x,+\hs/2,t), \qquad&&  x\in(0,\ls), % x\in\OmegaS,
   \end{alignedat}  \right. \\
& \text{Interface:}\quad   v_2^{\pm}(x,\pm\hs/2,t)=\frac{\partial\eta}{\partial t}(x,t), \qquad  x\in(0,\ls), % x\in\OmegaS .
% 
\end{aligned}
  \label{eq:MP1}
\end{equation*}
with periodic boundary conditions in the $x$-direction. 
The beam has length $\ls$ and constant thickness $\hs$, breadth $\bs=1$, and has reference-line along $y=0$. 
The fluid in the lower domain occupies the region $\OmegaF_-=[0,\ls]\times[\Hf^{-},-\hs/2]$, while the domain of the  fluid
in the upper part  is $\OmegaF_+=[0,\ls]\times[\hs/2,\Hf^{+}]$. 
Here  $y=\pm\hs/2$ are the heights of the interfaces of the beam in the
upper and lower fluid, respectively.
Initial conditions for $\vv^\pm$, $\eta$ and $\eta_t$ are also
needed to complete the specification of the problem. 
% 
% To begin the analysis, the solution is expanded in a finite Fourier series in $x$ (i.e.~a pseudo-spectral approximation), which gives 

The solution is expanded as a Fourier series in $x$, 
\[
 \vv^{\pm}(x,y,t) \approx \sum_{k=-\infty}^{\infty} \vvh^{\pm}(k,y,t) e^{2\pi i k x/\ls} , \qquad
    p^{\pm}(x,y,t) \approx \sum_{k=-\infty}^{\infty} \ph^{\pm}(k,y,t) e^{2\pi i k x/\ls} ,
\]
and
\[
  \eta(x,t) \approx \sum_{k=-\infty}^{\infty} \etah(k,t) e^{2\pi i k x/\ls} . 
\]
The governing equations for the Fourier components corresponding to a given wavenumber $k$ are
\begin{equation}
\left. \begin{array}{r}
\displaystyle{
  \rho^{\pm} \frac{\partial \vh_1^{\pm}}{\partial t} + i\kx \ph^{\pm} =0
} \smallskip\\
\displaystyle{
  \rho^{\pm} \frac{\partial \vh_2^{\pm}}{\partial t} + \frac{\partial \ph^{\pm}}{\partial y} =0
} \smallskip\\
\displaystyle{
  \frac{\partial^2 \ph^{\pm}}{\partial y^2} - \kx^2 \ph^{\pm} =0
}
\end{array}
\right\},
\begin{array}{l}
  \qquad y \in (\Hf^{-},-\frac{\hs}{2}) \mathrm{~ for~the~ lower ~fluid},\\
  \qquad y \in (\frac{\hs}{2},\Hf^{+}) \mathrm{~ for~the~ upper~ fluid},\\
\end{array}
\label{eq:modelFluidEquationFT}
\end{equation}
 and
\begin{equation}
  \rhos\hs \frac{\partial ^2\etah}{\partial t^2} = - \Lt \etah + \ph^{-}(k,-\hs/2,t)-\ph^{+}(k,\hs/2,t),  \mathrm{~ for~the~beam},
\label{eq:modelShellEquationFT}
\end{equation}
 where $\vvh=(\vh_1,\vh_2)$, $\kx = 2\pi k/\ls$, and  $\Lt=\Ks_0+\Ts\kx^2+\Es\Is\kx^4$.
The boundary conditions on the fluid at $y=\Hf^{\pm}$ are first 
taken as solid {\em slip} walls (equivalent to a symmetry boundary condition), which implies
$\vh_2^{\pm}(k,\Hf^{\pm},t)=0$.  It then follows from the fluid momentum equation that
\begin{equation}
  \frac{\partial \ph^{\pm}}{\partial y}(k,\Hf^{\pm},t)=0.
  \label{eq:modelBCFT}
  \end{equation}
At the discrete level, the choice of interface condition, either matching the velocity (traditional scheme)
or the acceleration (AMP scheme),
is critical to the stability of the scheme. 
At the continuous level, both conditions are valid: 
the interface
condition on the velocity, $\vh_2^{\pm}(k,\pm\hs/2,t)=\frac{\partial\etah}{\partial t}(k,t)$, implies the acceleration condition,
\begin{equation*}
  \frac{\partial \vh_2^{\pm}}{\partial t}(k,\pm\hs/2,t)=\frac{\partial^2\etah}{\partial t^2}(k,t).
\end{equation*}
Using the fluid momentum equation in the $y$ direction, gives the additional relation
\begin{equation}
  \frac{\partial \ph^{\pm}}{\partial y}(k,\pm\hs/2,t)=  -\rho^{\pm}\frac{\partial^2\etah}{\partial t^2}(k,t).
  \label{eq:modelInterfaceFTpy}
\end{equation}
% 
For $k\neq0$, the solution of the pressure equation in the fluid system (\ref{eq:modelFluidEquationFT}) is 
\begin{equation}
\ph^{\pm}(k,y,t) = a^{\pm}e^{k_x y} +b^{\pm}e^{-k_xy}, \label{eq:pSolution}
\end{equation}
with time-dependent coefficients $a^{\pm}$ and $b^{\pm}$ that  are determined
by the boundary condition (\ref{eq:modelBCFT}) and  the interface  condition (\ref{eq:modelInterfaceFTpy}), that is,
\begin{align}
  &a^{+}e^{k_x \Hf^{+}} -b^{+}e^{-k_x\Hf^{+}}=0,\label{eq:BC1}\\
  &a^{-}e^{k_x \Hf^{-}} -b^{-}e^{-k_x\Hf^{-}}=0,\label{eq:BC2}\\
  &\left(a^{+}e^{k_x \hs/2} -b^{+}e^{-k_x\hs/2}\right)k_x= -\rho^{+}\frac{\partial^2\etah}{\partial t^2}(k,t),\label{eq:BC3}\\
  &\left(a^{-}e^{-k_x \hs/2} -b^{+}e^{k_x\hs/2}\right)k_x= -\rho^{-}\frac{\partial^2\etah}{\partial t^2}(k,t).\label{eq:BC4}
\end{align}
Using (\ref{eq:pSolution})--(\ref{eq:BC4}), it follows that
\begin{equation}
 \ph^{-}(k,-\hs/2,t)-\ph^{+}(k,\hs/2,t) =-M_a^{-}(k)\frac{\partial^2\etah}{\partial t^2}(k,t)-M_{a}^{+}(k)\frac{\partial^2\etah}{\partial t^2}(k,t),
\end{equation}
where $M_{a}^{\pm}(k)$ are the added-mass coefficients for the upper and lower fluids defined as
\begin{equation}
  M_a^{-}(k) =\frac{\rho^{-}\left[1+e^{-2k_x\mathcal{D}^{-}}\right]}{k_x\left[1-e^{-2k_x\mathcal{D}^{-}}\right]},~{\rm and}~ M_a^{+}(k) =\frac{\rho^{+}\left[1+e^{-2k_x\mathcal{D}^{+}}\right]}{k_x\left[1-e^{-2k_x\mathcal{D}^{+}}\right]},~~(k\neq0).
  \label{eq:addedMass}
\end{equation}
Here $\mathcal{D}^{-}=-\hs/2-\Hf^{-}$ and $\mathcal{D}^{+}=\Hf^{+}-\hs/2$ are the depths of the lower and upper fluid domains, respectively, and it is  noted that $M_a^{\pm}(k) >0$. The added-mass terms are now  explicitly identified  in   the beam equation (\ref{eq:modelShellEquationFT}),
\begin{equation}
 \Big( \rhos\hs+M_a^{-}(k)+M_a^{+}(k)\Big) \frac{\partial ^2\etah}{\partial t^2} = - \Lt \etah.
\end{equation}
% 
For $k=0$, solution is independent of time and takes the form
%the fluid pressure and shell displacement satisfy
% equations~\eqref{eq:modelFluidEquationFT}--\eqref{eq:modelShellEquationFT} 
% for fluid pressure and shell displacement are  
{\bf wdh: I think this is the form:} 
\begin{align}
% \ph^{\pm}(0,y,t) = p_0^\pm, ~{\rm and} ~ \etah(0,t) = 0,
  & \vv(0,t)=0, ~~ \ph^{\pm}(0,y,t) = p_0^\pm,   \label{eq:kZeroContinuous} \\
  & \Ks_0\etah(0,t) = p_0^- - p_0^+,  \label{eq:kZeroPressureDiff}
\end{align}
where $p_0^\pm$ are constants (not independent) that balance the initial displacement of the beam through 
through~\eqref{eq:kZeroPressureDiff}. 
The solution is thus determined up to a single constant in the pressure which has no consequential effect on the answer. 
To define a unique solution one additional constraint is needed
such as requiring the mean value of the pressure to be zero.
% The pressures are constant in each domain and match the
% To define a unique solution one additional constraint is needed, 
% such as requiring the mean value of the pressure to be zero in both domains which would imply $p_0^\pm=0$ and $\etah(0,t)=0$.
% However, at the discrete level, we  note that the equation for $\ph(0,y)$ becomes 
% 1D laplace equation subject to Neumann boundary condition on all the boundarys. 
% Therefore, we need a compatiblity condition to solve this  otherwise singular system following the work in \cite{splitStep2003}.



To see how the stability of a specific partitioned scheme is affected by the added-mass effect,
the governing system (\ref{eq:modelFluidEquationFT})-(\ref{eq:modelShellEquationFT}) is discretized
in time but, for clarity, leave the spatial coordinate $y$ continuous 
(the analysis can be easily extended to fully discrete in $y$). 
Let
\[
\vvh^{n\pm}(k,y)\approx\vvh^{\pm}(k,y,t^n), \qquad \ph^{n\pm}(k,y)\approx\ph^{\pm}(k,y,t^n), \qquad \etah^{n}(k)\approx\etah(k,t^n),
\]
 where $t^n=n\dt$. 
Let $D_{+t}$ and $D_{-t}$ denote the forward and backward divided different operators in time,
defined by $D_{+t}\etah^n=(\etah^{n+1}-\etah^n)/\dt$ and $D_{-t}\etah^n=(\etah^{n}-\etah^{n-1})/\dt$.

Firstly,  an analysis for the traditional partitioned scheme, described in  Algorithm \ref{alg:TP}, is conducted.

% --------------------------------------------------------------------------------------------------------------------------------------
\begin{algorithm}[H] {\bf Traditional partitioned (TP) scheme:}

\noindent Stage I: Advance the shell displacement using a leap-frog scheme:
\begin{align}
  \rhos\hs D_{+t}D_{-t}\etah^n & = -\Lt \etah^n + \ph^{n-}(k,-\hs/2)-\ph^{n+}(k,\hs/2) . \label{eq:etaLeapFrog}
%  \rhos\hs\frac{\etah^{n+1}-2\etah^n+\etah^{n-1}}{\dt^2} & = -\Lt \hs \etah^n + \ph^n(k,H) , \label{eq:etaLeapFrog}
\end{align}
Stage II: Advance the fluid velocity and pressure using a backward-Euler scheme,
\begin{equation}
\left. \begin{array}{r}
\displaystyle{
% \rho^{\pm} \frac{\vh_1^{(n+1)\pm}-\vh_1^{n\pm}}{\dt}  + i\kx \ph^{(n+1)\pm} =0
\rho^{\pm} D_{+t}\vh_1^{n\pm}  + i\kx \ph^{(n+1)\pm} =0
} \smallskip\\
\displaystyle{
% \rho^{\pm} \frac{\vh_2^{(n+1)\pm}-\vh_2^{n\pm}}{\dt} + \frac{\partial \ph^{(n+1)\pm}}{\partial y} =0
\rho^{\pm} D_{+t}\vh_2^{n\pm} + \frac{\partial \ph^{(n+1)\pm}}{\partial y} =0
} \smallskip\\
\displaystyle{
\frac{\partial^2 \ph^{(n+1)\pm}}{\partial y^2} - \kx^2 \ph^{(n+1)\pm} =0
}
\end{array} \right\},
\begin{array}{l}
  \qquad y \in (\Hf^{-},-\frac{\hs}{2}) \mathrm{~ for~the~ lower ~fluid},\\
  \qquad y \in (\frac{\hs}{2},\Hf^{+}) \mathrm{~ for~the~ upper~ fluid},\\
\end{array}
\label{eq:fhat}
\end{equation}
with interface condition,
\begin{equation} 
\frac{\partial \ph^{(n+1)^{\pm}}}{\partial y}(k,\pm\hs/2) = -\rho^{\pm}  D_{+t}D_{-t}\etah^n(k),  \label{eq:interfaceTraditional}
\end{equation}
and boundary condition,
\begin{equation} 
\frac{\partial \ph^{(n+1)\pm}}{\partial y}(k,\Hf^{\pm})=0.  \label{eq:pressureBCTraditional}
\end{equation}
\label{alg:TP}
\end{algorithm}
% --------------------------------------------------------------------------------------------------------------------------------------
The solution to the TP scheme can be determined following the steps used above for the continuous-in-time problem.
For $k\ne 0$, this leads to a difference equation for $\etah^n$
% it  follows the arguments for the continuous case that
\begin{align}
  \rhos\hs D_{+t}D_{-t}\etah^n +\Big(M_a^{+}(k)+M_a^{-}(k)\Big)D_{+t}D_{-t}\etah^{n-1}& = -\Lt \etah^n.
\label{eq:etaTraditional} 
\end{align}
Note that interface relation~\eqref{eq:interfaceTraditional} applied in the TP scheme 
uses the acceleration of the beam lagged by one time-level; this time-lag turns out to be 
the primary source of the added-mass instability.
% is inconsistent with
% that~\eqref{eq:modelInterfaceFTpy} of the continuous case in a way that the accelerations are actually matched at different time
% levels, which 
% results the time delayed appearance of the added-mass term in~\eqref{eq:etaTraditional}. 
% We consider this delay as the
% primary source of the added-mass instability.

For $k=0$, the pressures in the TP scheme are only determined up to an arbitrary constant 
as for the continuous case~\eqref{eq:kZeroContinuous}-\eqref{eq:kZeroPressureDiff}.
At the discrete level there is a subtlety for the $k=0$ mode that results in an added-mass effect.
At the discrete level the  pressure equations for $p^+$ and $p^-$ are both singular and these
singularities needs to be removed in a numerical implementation since, due to round-off or truncation
errors the singular systems may have no solution.
To remove the singularity we follow the approach in~\cite{splitStep2003} 
that solves an augmented linear system with one additional unknown and one additional constraint equation.
%
% For $k= 0$, the TP scheme is a singular system since both the interface condition~\eqref{eq:interfaceTraditional} and boundary condition~\eqref{eq:pressureBCTraditional}  are essentially Neuamn boundary condition, and the pressure equation in~\eqref{eq:fhat} becomes 1D laplace equation. 
% Following the idea in
% \cite{splitStep2003}, we introduce an additional parameter $\alpha$ and  a constraint condition  for the pressure to remove the singularity in the system. 
To be specific, instead of the pressure equation described  in~\eqref{eq:fhat}, we solve the an augmented  equation for pressure when $k=0$,
\begin{align*}
   & \frac{\partial^2 \ph^{(n+1)\pm}}{\partial y^2} +\alpha^{(n+1)\pm} =0,\\
    &\int_{\Hf^{-}}^{-\hs/2} \ph^{(n+1)-}dy=\int^{\Hf^{+}}_{\hs/2} \ph^{(n+1)+}dy  = 0.
\end{align*}
where  $\alpha^{(n+1)\pm}$ are two additional unknowns. This new system has a unique solution.
The general solution of the augumented pressure equation is
\begin{equation}
 \ph^{(n+1)\pm}(0,y) = a^{(n+1){\pm}} + b^{(n+1){\pm}}y -\frac{\alpha^{(n+1)\pm}}{2}y^2.
\end{equation}
{\bf wdh: do we want to skip the details here? Longfei: I vote yes.}
With the boundary, interface and constraint conditions, we have the following equations that determine $ a^{(n+1){\pm}},~b^{(n+1){\pm}}$ and $\alpha^{(n+1){\pm}}$,
\begin{align}
  &b^{(n+1){+}} -\alpha^{(n+1)+}\Hf^{+} = 0,\label{eq:BCTP1}\\
  &b^{(n+1){-}} -\alpha^{(n+1)-}\Hf^{-} = 0,\label{eq:BCTP2}\\
  &b^{(n+1){+}} -\alpha^{(n+1)+}\hs/2 = -\rho^{+}  D_{+t}D_{-t}\etah^n(0),\label{eq:BCTP3}\\
  &b^{(n+1){-}} +\alpha^{(n+1)-}\hs/2 = -\rho^{-}  D_{+t}D_{-t}\etah^n(0),\label{eq:BCTP4}\\
  &a^{(n+1){+}}\Big[\Hf^{+}-\frac{\hs}{2}\Big] + \frac{1}{2}b^{(n+1){+}}\Big[{\Hf^{+}}^2-\left(\frac{\hs}{2}\right)^2\Big] -\frac{\alpha^{(n+1)+}}{6}\Big[{\Hf^{+}}^3-\left(\frac{\hs}{2}\right)^3\Big] = 0,\label{eq:BCTP5}\\
    &a^{(n+1){-}}\Big[-\frac{\hs}{2}-\Hf^{-}\Big] + \frac{1}{2}b^{(n+1){-}}\Big[\left(-\frac{\hs}{2}\right)^2-{\Hf^{-}}^2\Big] -\frac{\alpha^{(n+1)-}}{6}\Big[\left(-\frac{\hs}{2}\right)^3-{\Hf^{-}}^3\Big] = 0.\label{eq:BCTP6} 
\end{align}
Solving the system~\eqref{eq:BCTP1}--\eqref{eq:BCTP6}, we have
\begin{align*}
  &\alpha^{(n+1)+} = -\frac{\rho^{+}}{\mathcal{D}^{+}} D_{+t}D_{-t}\etah^n(0),\\
  &\alpha^{(n+1)-} =  \frac{\rho^{+}}{\mathcal{D}^{-}} D_{+t}D_{-t}\etah^n(0),\\
  & b^{(n+1){+}} = \alpha^{(n+1)+}\Hf^{+},\\
  & b^{(n+1){-}} =\alpha^{(n+1)-}\Hf^{-} ,\\
  & a^{(n+1){+}} =\alpha^{(n+1)+}\Big[-\frac{1}{3}{\Hf^{+}}^2 -\frac{1}{3}\left(\frac{\hs}{2}\right)\Hf^{+}+\frac{1}{6}\left(\frac{\hs}{2}\right)^2\Big], \\
  & a^{(n+1){-}} =\alpha^{(n+1)-}\Big[-\frac{1}{3}{\Hf^{-}}^2 +\frac{1}{3}\left(\frac{\hs}{2}\right)\Hf^{+}+\frac{1}{6}\left(\frac{\hs}{2}\right)^2\Big]. \\
\end{align*}

Therefore, the force on the beam from the fluid pressure is
\begin{equation}
  \ph^{(n+1)-}(0,-\hs/2)-\ph^{(n+1)+}(0,\hs/2) =- M_a^{+}(0) D_{+t}D_{-t}\etah^n(0) - M_a^{-}(0) D_{+t}D_{-t}\etah^n(0),
  \label{eq:0modeTPdeltaP}
\end{equation}
where the added-mass coeffients are given by
\begin{equation}
  M_a^{-}(0) = \frac{1}{3} \rho^{-}\mathcal{D}^{-},~{\rm and }~ M_a^{+}(0) = \frac{1}{3} \rho^{+}\mathcal{D}^{+}.
  \label{eq:addedMass0modeTP}
\end{equation}
By substituting~\eqref{eq:0modeTPdeltaP} into the shell equation~\eqref{eq:etaLeapFrog}, it is  shown that ~\eqref{eq:etaTraditional} applies when $k=0$ as well. We note that the expressions~\eqref{eq:addedMass0modeTP} may vary depending on how the
pressure system is regularized. 




The stability of the overall scheme is determined by the stability of~\eqref{eq:etaTraditional}. Noting that equation~\eqref{eq:etaTraditional} is actually of the same form as the equation in the analysis for the case of a beam with fluid on one side~\cite{fis2014};  therefore,  the same conclusion is reached,
\begin{theorem} \label{th:traditional}
  Assuming $\rhos\hs>0$, $\Lt>0$ and $M_a>0$, 
the traditional partitioned scheme given in Algorithm~\ref{alg:TP} is weakly stable if and only if 
the following conditions are satisfied:
\begin{align}
%   &  \dt^2 <  2 \, \frac{\rhos\hs}{\Lt} \Big[ \frac{\rhos\hs}{M_a} - \frac{M_a}{\rhos\hs} \Big],  \\
  &  \dt <  2\sqrt{ \frac{\rhos\hs-M_a^{-}(k)-M_a^{+}(k)}{\Lt}}, ~ k  = 0,1,2..., \label{eq:traditionalStabLimitII}
\end{align}
where $M_a^{\pm}(k)$ is given by~\eqref{eq:addedMass}  when $k\neq 0$ and given by~\eqref{eq:addedMass0modeTP} when $k=0$.

\end{theorem}
The condition ~\eqref{eq:traditionalStabLimitII} requires the total added mass $M_a^{-}(k)+M_a^{+}(k)<\rhos\hs$. This is in  agreement with the result of Causin {\it et al.}~\cite{CausinGerbeauNobile2005}, who studied a simple beam with fluid on one side.
 Additionally, the condition~\eqref{eq:traditionalStabLimitII} indicates how the time-step must be reduced as the added-mass effects become larger.
% The proof of this theorem follows from the theory of blah, blah (ref).  
It is noted that the TP scheme is unconditionally unstable if the contribution from the added mass is too large, i.e.~if $M_a^{-}(k)+M_a^{+}(k) >\rhos \hs$, regardless of the choice for the time-step, $\dt$.  From~\eqref{eq:addedMass}, we observe that the added-mass coefficient is large for large $\rho^{\pm} \ls$, small $k$ and/or small $\mathcal{D}^{\pm}/\ls$.  Thus, the TP scheme has difficulty when the mass ratio, $(\rho \ls)/(\rhos\hs)$, is large, the wave number of surface variations is low, and/or the fluid domains are thin.


Secondly, the stability of the  AMP scheme for  the case of a beam with fluid on both sides is analyzed.  The  AMP algorithm is described in Algorithm ~\ref{alg:AMP} {\bf(Longfei: the ref number is not correct)}.
% --------------------------------------------------------------------------------------------------------------------------------------
\begin{algorithm}[H] {\bf AMP scheme:} 

\noindent Stage I: Advance the shell displacement using a leap-frog scheme (as in the traditional scheme),
\begin{equation}
  \rhos\hs D_{+t}D_{-t}\etah^n  = -\Lt \etah^n + \ph^{n-}(k,-\hs/2)-\ph^{n+}(k,\hs/2) .
\label{eq:etaLeapFrogAM}
\end{equation}
Stage II: Advance the fluid velocity and pressure using a backward-Euler scheme (as in the traditional scheme),
\[
\left. \begin{array}{r}
\displaystyle{
% \rho^{\pm} \frac{\vh_1^{(n+1)\pm}-\vh_1^{n\pm}}{\dt}  + i\kx \ph^{(n+1)\pm} =0
\rho^{\pm} D_{+t} \vh_1^{n\pm}  + i\kx \ph^{(n+1)\pm} =0
} \smallskip\\
\displaystyle{
% \rho^{\pm} \frac{\vh_2^{(n+1)\pm}-\vh_2^{n\pm}}{\dt} + \frac{\partial \ph^{(n+1)\pm}}{\partial y} =0
\rho^{\pm} D_{+t} \vh_2^{n\pm} + \frac{\partial \ph^{(n+1)\pm}}{\partial y} =0
} \smallskip\\
\displaystyle{
\frac{\partial^2 \ph^{(n+1)\pm}}{\partial y^2} - \kx^2 \ph^{(n+1)\pm} =0
}
\end{array} \right\},
\begin{array}{l}
  \qquad y \in (\Hf^{-},-\frac{\hs}{2}) \mathrm{~ for~the~ lower ~fluid},\\
  \qquad y \in (\frac{\hs}{2},\Hf^{+}) \mathrm{~ for~the~ upper~ fluid},\\
\end{array}
\]
with the AMP Robin interface condition, derived from~\eqref{eq:AMPpressureBC},
\begin{equation}
\ph^{(n+1)-}(k,-\hs/2)-\ph^{(n+1)+}(k,+\hs/2) + \frac{\rhos\hs}{\rho^{\pm}} \frac{\partial \ph^{(n+1)\pm}}{\partial y}(k,\pm\hs/2) = \Lt \etah^{n+1}(k),
\label{eq:AMPinterfaceBC}
\end{equation}
and boundary conditions.
\[
\frac{\partial \ph^{(n+1)\pm}}{\partial y}(k,\Hf^{\pm})=0.
\]
\label{alg:AMP}
\end{algorithm}
% --------------------------------------------------------------------------------------------------------------------------------------


The key ingredient of the AMP scheme is the Robin condition in~\eqref{eq:AMPinterfaceBC} for the fluid pressure. 
This condition implies
$$
\frac{\partial \ph^{(n+1)^{\pm}}}{\partial y}(k,\pm\hs/2) = -\rho^{\pm}  D_{+t}D_{-t}\etah^{n+1}(k),
$$
where now the acceleration term on the right-hand-side is at the same time level as the left-hand-side.
% which is consistent with the interface condition~\eqref{eq:modelInterfaceFTpy} for the continuous case. 
%
Following the steps of the solution procedure for the continuous case leads to, when $k\neq 0$,
\begin{align}
  \rhos\hs D_{+t}D_{-t}\etah^n +\Big(M_a^{-}(k)+M_a^{+}(k)\Big)D_{+t}D_{-t}\etah^{n}& = -\Lt \etah^n.
  \label{eq:etaAMP}
\end{align}
When $k=0$, the interface condition for the AMP scheme is a Robin condition for pressure, therefore, unlike the TP scheme, the system is not singular, and we are able to solve the pressure, i.e.,
{\bf wdh: I think the coupled pressure system is still singular. Longfei: i need to work on this.}
$$
 \ph^{(n+1)\pm}(0,y) = b^{(n+1)\pm}, 
$$
where $b^{(n+1)\pm}$ are constants.
With the AMP Robin condition~\eqref{eq:AMPinterfaceBC}, we have
$$
 b^{(n+1)-}- b^{(n+1)+} = \Lt \etah^{n+1}(0). 
$$
 Then the shell equation~\eqref{eq:etaLeapFrogAM} becomes
 \begin{align}
  \rhos\hs D_{+t}D_{-t}\etah^n +\Big(M_a^{-}(0)+M_a^{+}(0)\Big)D_{+t}D_{-t}\etah^{n}& =0,
  \label{eq:etaAMP0Mode}
\end{align}
 where
 $$
 M_a^{-}(0)=M_a^{+}(0)=0.
 $$
% We note that~\eqref{eq:etaAMP0Mode} is non-dissipative.
 
\begin{theorem}
   When $k\neq0$, the added-mass partitioned scheme described in Algorithm~\ref{alg:AMP} is stable if and only if 
\begin{align}
   \dt <2 \sqrt{\frac{\rhos\hs+M_a^{+}(k)+M_a^{-}(k)}{\Lt}}, \label{eq:AMPstability}
\end{align}
where $M_a^{\pm}(k)$ is given by~\eqref{eq:addedMass}. 
% When $k=0$, the scheme is non-dissipative. 
\end{theorem}
\begin{proof}
Using $\etah^{n}=\amp^n \etah^{0}$ and substituting into~\eqref{eq:etaAMP} gives
\begin{align*}
&   \amp^2 -(2-\frac{\Lt}{\rhos\hs+M_a(k)}\Delta t^2) \amp + 1 = 0, 
\end{align*}
where $M_a(k) =M_a^{+}(k)+M_a^{-}(k) $ denotes the total added mass.
The requirement that $\vert\amp\vert \le 1$ and that the roots be simple 
implies $\vert (2-\frac{\Lt}{\rhos\hs+M_a(k)}\Delta t^2) /2 \vert < 1$ which leads to~\eqref{eq:AMPstability}.
\end{proof}

It is interesting to note that the AMP algorithm  is stable when using the time-step restriction that arises when advancing the shell with no fluid present (i.e.~taking $M_a=0$ in~\eqref{eq:AMPstability}).  Also, when~\eqref{eq:AMPstability} holds the amplification factor satisfies $\vert\amp\vert=1$ and the scheme is non-dissipative.  Finally, for this simple AMP scheme, the fluid and shell velocities 
at the interface only match to first-order accuracy. As noted previously, one
could include an additional projection step to match the velocities on the interface.

The analysis done in this section so far is for the boundary condition of solid slip walls, i.e., $v_2(x,\Hf^{\pm},t)=0$.  Following a similar argument, it is easily shown that the previous theorems apply also for the boundary condition of free surfaces, i.e., $p^{\pm}(x,\Hf^{\pm},t)=0$. In this case, the added mass coefficients are defined as 
\begin{align}
  k\neq0:\qquad&\tilde{M}_a^{-}(k) =\frac{\rho^{-}\left(1-e^{-2k_x\mathcal{D}^{-}}\right)}{k_x\left(1+e^{-2k_x\mathcal{D}^{-}}\right)},~{\rm and}~ \tilde{M}_a^{+}(k) =\frac{\rho^{+}\left(1-e^{-2k_x\mathcal{D}^{+}}\right)}{k_x\left(1+e^{-2k_x\mathcal{D}^{+}}\right)},\\
    k=0:\qquad&\tilde{M}_a^{-}(0) =\rho^{-}\mathcal{D}^{-},~{\rm and}~ \tilde{M}_a^{+}(0) =\rho^{+}\mathcal{D}^{+},
  \label{eq:addedMass||}
\end{align}
Noting that the $k=0$  case is actually the limit of the $k\neq0$ case.


==> texFiles/beamModels-orig.tex <==
% ----------------------------------------------------------------------------------
\newcommand{\Kt}{\Ks_1}
\newcommand{\Kxxt}{\Ts_1}
\section{An Euler-Bernoulli beam model} \label{sec:beamModels}


For the purposes of this paper we consider a generalized Euler-Bernoulli (EB) beam model.
\old{Although this model is
only valid for small deviations   from an initially flat beam (small {\em slopes}), it will be used to
demonstrate the stability of the AMP algorithm for finite amplitude motions. 
In this section we describe this beam model and also describe
some more details of the AMP algorithm as it applies in this setting.

A generalized Euler-Bernoulli beam model is}
\new{This model is physically relevant when the deviations from an initial beam shape are sufficiently small (small {\em slopes}).
The EB model will be used here to demonstrate the stability and accuracy of the AMP algorithm for finite amplitude beam
motion in coupled FSI problems. The generalized Euler-Bernoulli beam model considered here is}

\begin{align}
  \rhos \As \frac{\partial^2\ww}{\partial t^2} = 
                    & -\Ks_0\ww +
                   \frac{\partial}{\partial s}\left( \Ts \frac{\partial\ww}{\partial s}\right)
                   - \frac{\partial^2}{\partial s^2}\left( \Es \Is \frac{\partial^2\ww}{\partial s^2}\right) 
                  - \Kt \frac{\partial\ww}{\partial t}
                   + \Kxxt \partialt\frac{\partial^2 \ww}{\partial s^2}
                   + f(s,t), 
                  \quad s\in[0,\ls], \quad t\ge 0,  \label{eq:BeamModel}
\end{align}
where $y=\ww(s,t)$ is the displacement of the beam reference line, $\partial\ww/\partial t$ is the velocity,  
$\As=\As(s)$ is the cross-sectional area of the beam\footnote{The cross-section area, $\As=\As(s)$, will in general
vary with $s$ such as near the rounded tip of the free end of a cantilevered beam.}
($\As=\hs\bs$ where $\hs$ is the thickness and $\bs$ the breadth
in the z-direction), 
$\rhos$ is the beam density, $\ls$ is the length of the beam, 
$\Es$ is Young's modulus, $\Is$ is the area-moment of inertial (e.g. $\Is=\frac{1}{12} \hs^3 \bs$ for a rectangular beam),
$\Ts$ is the {\em tension} coefficient and $\Ks_0$ is the linear stiffiness coefficient.
The term with coefficient $\Kt$ is a linear damping term while the term with 
coefficient $\Kxxt$ damps higher spatial frequencies faster than lower frequencies and
serves to smooth the beam. 
%is a {\em visco-elastic} damping term that . 
% 







\input texFiles/beamCartoon

Let $\xbv(\ss,t)=(\ss,\eta(\ss,t))$ denote the position of the reference-line 
of the beam (this is the centerline of the EB beam)
% or {\em neutral-axis}) 
at time $t$ which is given by 
\begin{align*}
  \xbv(\ss,t)= \xbv(\ss,0) + \usv(s,t), 
\end{align*}
% where $\xsv(s)=\xbv(\ss,0)$ is the initial position of the reference-line and 
where $\usv(s,t)=(0,\eta(\ss,t))$ is the beam displacement.
Let $\xsv_+(\ss,t)$ and $\xsv_+(\ss,t)$ denote the points
on the upper and lower surfaces of the beam, respectively.
The geometry for EB beam is illustrated in Figure~\ref{fig:beamCartoon}. 
In this case, lines normal to the mid-line remain straight and 
we have  
\begin{align}
  \xsv_{\pm}(\ss,t)=\xbv(\ss,t)\pm \frac{\hs}{2} \nsv(\ss,t), \label{eq:EBsurface}
\end{align}
where $\hs=\hs(s)$ is the thickness of the beam and $\nsv(\ss,t)$ is the unit normal to the {\em reference-line} 
($\nsv$ is sometimes called the pseudo-normal or director~\cite{Belytschko2005}). 
% Note that in some circumstances we use the simplied approximation $\xsv_{\pm}(\ss,t)=\xbv(\ss,t)$, 
% which is a good approximation for very thin beams. 
For an EB beam the velocity and acceleration on the surface of the beam are given by 
\begin{align}
   \vsv_\pm(s,t) =  \frac{\partial}{\partial t}\xsv_{\pm}(\ss,t) = \vsv(\ss,t) \pm \frac{\hs}{2} \partialt \nsv(\ss,t),
      \label{eq:beamSurfaceVelocityEB} \\
   \asv_\pm(s,t) =  \partialt \vsv(\ss,t) \pm \frac{\hs}{2} \frac{\partial^2}{\partial t^2}\nsv(\ss,t).
      \label{eq:beamSurfaceAccelerationEB}
\end{align} 
Thus for an EB beam the velocity correction in~\eqref{eq:beamSurfaceVelocity} is given by
\begin{align}
   \wsv_\pm(s,t) = \pm \frac{\hs}{2} \partialt \nsv(\ss,t).
\end{align} 

\old{The} \new{In this work the} force $f(s,t)$ on the beam reference-line 
is defined by the normal components of the fluid tractions
on corresponding points on the beam surface,
\begin{align}
    f(s,t) = -\Big[ (\nv^T\sigmav\nv)_+ + (\nv^T\sigmav\nv)_- \Big]. \label{eq:EB_BeamForce}
\end{align}
\old{We take the fluid force to be $\nv^T\sigmav\nv$ instead of $\hat{y}^T\sigmav\nv$ even though
$\ww$ is the motion in the $y$ direction ($\hat{y}$ being the unit vector in the $y-$direction).
This is a modeling approximation and is valid for small beam deflections. 
The force on the beam is defined in this way to be consistent with the AMP pressure
conditions~\eqref{eq:AMPpressureBCI}-\eqref{eq:AMPpressureBCII}.}
\new{This modeling approximation is valid for small beam deflections which is consistent with the 
use of an EB beam and with the AMP pressure conditions~\eqref{eq:AMPpressureBCI}-\eqref{eq:AMPpressureBCII}.}
Recall that the right-hand-side of
~\eqref{eq:EB_BeamForce} \old{turns into the left hand sides of} \new{becomes the left-hand sides of the AMP conditions}~\eqref{eq:AMPpressureBCI}-\eqref{eq:AMPpressureBCII}.
\old{With this definition, the coefficients of $p_\pm$ on the left hand sides of~\eqref{eq:AMPpressureBCI}-\eqref{eq:AMPpressureBCII}
do not depend on the beam deflection and thus do not need to be changed when used with 
a different beam model that is valid for large deflections.}

\paragraph{Treatment of free ends} \old{For a beam with a free end, 
the end of the beam is usually rounded off a small amount as shown in Figure~\ref{fig:beamGrids}. The flow can
be complex near a sharp corner and by rounding off the corner a higher resolution grid can be
generated to resolve the flow in this region.
% 
The force on the beam is computed using the fluid normal $\nv$ and the approximation $\nv^T\sigmav\nv$. This
approximation is not very good on the rounded tip of the beam since the fluid normal is not nearly parallel
to the normal to the beam reference line. Consequently, in practice, fluid forces on the end of the beam are ignored in the
computation of the force on the beam (in particular, any points on the surface of the beam that extend beyond the length
of the beam reference line are ignored). This can be considered as a modeling assumption. The contributions
from the end points are also ignored when projecting the AMP interface velocity onto the beam.}
\new{For a beam with a free end, the tip of the beam is usually rounded as shown in Figure~\ref{fig:beamGrids}. The flow can
be complex near a sharp corner and by rounding the corner a high resolution grid can be
generated that resolves the flow in this region. In addition, recall that the force on the beam surface 
is computed using the fluid normal $\nv$ and the approximation $\nv^T\sigmav\nv$. Near the rounded tip of a beam 
this is a poor approximation since the fluid normal may be orthogonal to the beam reference line. Consequently, 
in practice, the fluid forces on the beam tip are ignored in computing force on the beam (in particular, any points on 
the surface of the beam that extend beyond the length of the beam reference line are ignored). 
This should be considered a modeling assumption. Similarly, contributions from the end points are also ignored 
when projecting the interface velocity onto the beam.}

%- The AMP conditions simplify for an EB beam of constant width. In this case $\nv_+$ is parallel to, and in the
%- opposite direction of $\nv_-$, i.e. $\nv_+^T\nv_-=-1$. 
%- Whence, taking the inner product of $\nv_\pm$ with equation~\eqref{eq:AMP_CombinedConditionsPressure}
%- gives *CHECK ME*
%- % ---------------------------------------------------------------------------------------------------------------
%- \begin{condition}
%- The AMP interface condition for the fluid pressure for an EB beam of constant width is 
%- \begin{equation}
%-   \pm\Big[ -p_+ +  p_-  \Big] - 
%- \frac{\rhos\hs}{\rho} \frac{\partial}{\partial n_\pm} p_\pm
%-          = \nv_\pm^T\Lsv\bigl(\uvs,\vsv\bigr) + \rhos\hs \nv_\pm^T\partialt \wsv_\pm(\ss,t) - \nv_\pm^T(\tauv\nv)_+ - \nv_\pm^T(\tauv\nv)_- , \qquad \ss\in\Gammas.
%-     \label{eq:AMP_Pressure}
%- \end{equation}
%- where $p_\pm=p(\xsv_\pm(\ss,t),t)$. 
%- \end{condition}
%- % ---------------------------------------------------------------------------------------------------------------
%- Taking the inner product with the tangent vectors $\tv_\pm$, gives
%- an interface condition for the velocity.  *CHECK ME*
%- % ---------------------------------------------------------------------------------------------------------------
%- \begin{condition}
%- The AMP interface condition for the fluid velocity for an EB beam of constant width is 
%- \begin{equation}
%-   \pm\Big[ (\tv^T\tauv\nv)_+ -  (\tv^T\tauv\nv)_- \Big] 
%- + \frac{\rhos\hs}{\rho} \tv_\pm^T\grad p(\xsv_\pm(\ss,t),t)  
%-          = \tv_\pm^T\Lsv\bigl(\uvs,\vsv\bigr) + \rhos\hs \tv_\pm^T\partialt \wsv_\pm(\ss,t) , \qquad \ss\in\Gammas.
%-     \label{eq:AMP_Velocity}
%- \end{equation}
%- \end{condition}
%- 


%- % -------------------------------------------------------
%- \subsection{Details: fluid force on the EB beam}
%- 
%- The fluid force on the EB beam is defined in a particular way to be consistent with the AMP pressure
%- conditions~\eqref{eq:AMPpressureBCI}-\eqref{eq:AMPpressureBCI}. 
%- Consider the EB beam equation for a beam on top of a fluid region, 
%- \begin{equation}
%-  \rhos \As \frac{\partial^2\ww}{\partial t^2} = \Ls_2(\ww,\dot\ww) - \nv^T\sigmav\nv  \label{eq:beamEquationWithForce}
%- \end{equation}
%- Note that we take the fluid force to be $\nv^T\sigmav\nv$ instead of $\hat{y}^T\sigmav\nv$ even though
%- $\ww$ is the motion in the $y$ direction.
%- This is a modeling approximation and is valid for small beam deflections. 
%- One reason we make this approximation is so that the normal component of the AMP condition,
%-  derived from~\eqref{eq:beamEquationWithForce}
%- takes the form 
%- \begin{equation}
%-    \nv^T\sigmav\nv + \frac{\rhos\hs}{\rho} \nv^T(\grad\cdot\sigmav) = \nv^T \Lsv + \rhos\hs\nv^T\partialt \wsv
%-                \label{eq:AMPbeam}
%- \end{equation}
%- and thus the term $\nv^T\sigmav\nv= -p =\nv^T\tauv\nv$ appears as the first term of the left-hand-side.


% NOTE: For~\eqref{eq:AMPbeam} to be consistent with~\eqref{eq:beamEquationWithForce} we should take $\nv^T \Lsv=\Ls_2(\ww,\dot\ww)$


% -------------------------------------------------------
% \subsection{Details: Treatment of a beam with free ends}




==> texFiles/cylBeam.tex <==
\newcommand{\Gccb}{\Gc_{\text{cb}}}
\subsection{Flow past a cylinder with an attached beam} \label{sec:cylBeam}



We consider flow past a rigid cylinder with an attached flexible appendage.


Cylinder with center $(0,0)$ and radius $R_c=0.5$.

Beam of length $\Ls=3$ and thickness $\hs=0.2$ is attached to the right side of the cylinder.

The channel occupies the region $[-2,7]\times[-1,2]$.
The cylinder and beam are placed closer to the lower wall of the channel. 

Composite grid $\Gccb^{(j)}$ with approximate grid spacing $\Delta s^{(j)}=1/(10 j)$. 

Fluid: density $rho=1$, $\mu=??$.

Beam: $\rhos=?$, ...


{% ------ GRIDS ------
\newcommand{\figWidth}{8cm}
\newcommand{\trimfig}[2]{\trimFigb{#1}{#2}{.05}{.05}{.3}{.275}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.0,.5) rectangle (16.,5.5);  % set the bounding box (so we have less surrounding white space)
  \draw(-.1,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/cylBeam2Gridt0p0}{\figWidth}};
  \draw(8.1,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/cylBeam2Gridt49p0}{\figWidth}};
% grid:
% \draw[step=1cm,gray] (0,0) grid (16,5);
\end{tikzpicture}
\end{center}
  \caption{Composite grids for a cylinder with attached beam, coarse grid $\Gccb^{(2)}$ at two times.}
  \label{fig:cylBeamGrids}
\end{figure}
}


==> texFiles/flexibleChannelTableII.tex <==
% --- Parameter Set II  ------------------------------------------------------------------------------------------------
\bogus{% ************************ START BOGUS *******************************************************
% -- from runs/ins/flexibleChannel/compfc.cmd (comp.out)
% 
% ********** MArch 24, 2015
% 
% # --- Case A : Fernandez 2013 + larger nu, smaller Kxxt
% 
% 
% Solutions at times=1.000000e+00, 1.000000e+00, 1.000000e+00, 1.000000e+00, 
% ++++++++++++++ max norm results +++++++++++++                               
%     ee = estimated error from C*h^{rate}                                    
% ++computeRate: there is a constant refinement factor r=2.00: e0=2.60e-02, e1=4.98e-03 rate=2.08e+00
%  component=0,           p, rate= 2.08, ee(0) = 1.17e-01, ee(1) = 2.76e-02, [r= 4.23], ee(2) = 6.52e-03, [r= 4.23], ee(3) = 1.54e-03, [r= 4.23], 
% ++computeRate: there is a constant refinement factor r=2.00: e0=1.25e-02, e1=2.38e-03 rate=2.08e+00                                             
%  component=1,           u, rate= 2.08, ee(0) = 5.58e-02, ee(1) = 1.32e-02, [r= 4.23], ee(2) = 3.12e-03, [r= 4.23], ee(3) = 7.39e-04, [r= 4.23], 
% ++computeRate: there is a constant refinement factor r=2.00: e0=4.98e-03, e1=9.62e-04 rate=2.06e+00                                             
%  component=2,           v, rate= 2.06, ee(0) = 2.21e-02, ee(1) = 5.29e-03, [r= 4.18], ee(2) = 1.27e-03, [r= 4.18], ee(3) = 3.03e-04, [r= 4.18], 
% % -------------- max norm results -------------                                                                                                 
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size                                                         
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.                                                   
% \newcommand{\errFormat}[1]{#1}} % use this command to set the format of the error label.                                                      
\begin{center}                                                                                                                                  
\begin{tabular}{|l|c|c|c|c|c|c|} \hline                                                                                                         
   grid              & \errFormat{p} &  r   & \errFormat{u} &  r   & \errFormat{v} &  r  \\ \hline                                              
 fc2a.show &  \num{1.2}{-1} &      & \num{5.6}{-2} &      & \num{2.2}{-2} &      \\ \hline                                                       
 fc4a.show &  \num{2.8}{-2} &  4.2 & \num{1.3}{-2} &  4.2 & \num{5.3}{-3} &  4.2 \\ \hline                                                       
 fc8a.show &  \num{6.5}{-3} &  4.2 & \num{3.1}{-3} &  4.2 & \num{1.3}{-3} &  4.2 \\ \hline                                                       
 fc16a.show & \num{1.5}{-3} &  4.2 & \num{7.4}{-4} &  4.2 & \num{3.0}{-4} &  4.2 \\ \hline                                                      
            &     2.08      &      &     2.08      &      &     2.06      &     \\ \hline      
\end{tabular}                                                                                                                                   
\caption{CASE A: Fernandez parameters but larger $\nu=0.01$, smaller Kxxt$=10^{-2}$. Max-norm self convergence results, Tue Mar 24 16:38:59 2015. }                                                                         
\label{fig:flexibleChannelII}
\end{center}                                                                                                                                    
\end{table}      
}% ********************************** END BOGUS **********************************************************
%
\newcommand{\tableChannelPSII}{%
\begin{tabular}{|c|c|c|c|c|c|c|} \hline
\multicolumn{7}{|c|}{\strutt Traveling wave pressure-pulse} \\ \hline 
\strutt~~$h_j$~~& $E_j^{(p)}$ & $r$  & $E_j^{(v_1)}$  & $r$    & $E_j^{(v_2)}$   & $r$    \\ \hline 
 1/20        &  \num{1.2}{-1} &      & \num{5.6}{-2} &      & \num{2.2}{-2} &      \\ \hline     
 1/40        &  \num{2.8}{-2} &  4.2 & \num{1.3}{-2} &  4.2 & \num{5.3}{-3} &  4.2 \\ \hline     
 1/80        &  \num{6.5}{-3} &  4.2 & \num{3.1}{-3} &  4.2 & \num{1.3}{-3} &  4.2 \\ \hline     
 1/160       &  \num{1.5}{-3} &  4.2 & \num{7.4}{-4} &  4.2 & \num{3.0}{-4} &  4.2 \\ \hline     
\rateLabel   &      2.08      &      &     2.08      &      &     2.06      &     \\ \hline      
\end{tabular}
}


\begin{figure}[hbt]\tableFontSize
\begin{center}
\tableChannelPSII
\end{center}
\caption{Traveling wave pressure-pulse (parameter set II, adjusted): Maximum errors and 
estimated convergence rates at $t=1.0$ computed using the AMP scheme.
}
\label{fig:flexibleChannelII}
\end{figure}


==> texFiles/flexiblePartition-orig.tex <==
\newcommand{\Gcpc}{\Gc_{\text{fp}}}
% ----------------------------------------------------------------------------------------------
\subsection{Steady-state exact solutions for a pressure-deformed beam} \label{sec:flexibleChannelSS}
% \subsection{A flexible partition separating two fluid chambers - steady state solution} \label{sec:flexibleChannelSS}

To illustrate the effectiveness of the AMP coupling scheme in comparison to the
traditional FSI coupling, we now discuss two cases where a beam deforms as a result of a uniform 
fluid pressure.  The first case involves an EB beam on the top surface of a fluid chamber (similar to the previous
test case), while the second involves a beam separating two fluid chambers.  As before, we assume that the EB
beam has negligible thickness but has finite mass.
% as shown in Figure~\ref{fig:partitionedChambersGrids}. {\bf stopped here}
Exact steady-state solutions can be determined when a constant fluid pressure is specified
at the bottom fluid boundary in the case of a single fluid chamber, and at bottom and top fluid boundaries for the case
of an EB beam separating two fluid chambers.  The steady state is computed numerically by integrating the
time-dependent equations from an initially flat beam. It is found that for {\em light} beams the traditional scheme is unstable, in agreement with the previous stability analysis, while the
AMP scheme remains stable and so that the steady state solution is computed accurately. 
% This is a good test of added-mass effects and a good numerical example since 

% The beam is pinned on both ends (displacement equal to zero).



% Some analytic solutions can be determined for this configuration and these are used to verify the accuracy and
% stability of the AMP solution algorithm.

% ----------------------------------------------------------------------------------------------
\subsubsection{A beam with fluid on one side}
For the case of a beam with fluid on one side, the geometry and grid  
are the same as those discussed in Section~\ref{sec:manufacturedSolutions}.
The material parameters for the fluid are chosen 
as  $\rho=1$ and $\mu=0.2$, while those for the
beam are chosen as $\Ks=0$, $\Ts=5$, $\Es\Is=0$, $\Kt=\Kxxt=0$ and a finite value for $\rhos\hs$.
The boundary conditions on the left and right sides of the fluid domain are given as a no-slip walls ($u=v=0$), 
while a given pressure ($p=P_a=5$) and zero tangential velocity ($u=0$) are assigned on the bottom of the fluid domain.
One boundary condition is required at each end of the beam for the chosen parameters, and these are taken as
$\eta=0$ at each end. 
The initial conditions are given as a flat stationary beam ($\eta=\dot\eta=0$) and 
a fluid at rest. The exact steady-state solution is
\begin{align}
u=v=0, \quad p = P_a,\qquad \eta = \frac{P_a x(1-x)}{2\Ts}.
\end{align} 
As before, $\rhos\hs$ is varied to illustrate the stability of the time-integration of the equations using the AMP coupling scheme for a range of masses of the beam, and also to highlight the instability of the traditional FSI coupling scheme for light beams. 
%
%The problem parameters are chosen as
%$p_a=5$, $\Ts=5$, $\Es=0$, $\rhos\As=1^{-3}$, and $\mu=0.2$. 
%
%In this case the beam is pinned on both ends (displacement equal to zero),
%and the exact steady solution is found as
%\begin{align}
%v_1 = 0,~ v_2=0,~ p = p_a,~ {\rm and }~\eta = -\frac{p_a}{2\Ts}\, x(x-1).
%\end{align} 

\textcolor{red}{(Perhaps we should discuss exactly what results we want to show and discuss here -- moving on for now.)}
Figure~\ref{fig:ParabolicBeam} shows the computed solution for $\rhos\hs=10^{-3}$
at early time, $t=0.1$, and  late time, $t=10$, which is nearly steady state. {\bf Its not clear
what this set of images add to the discussion. I suggest we show one image of the grid at the steady
state and then a second plot with a series of curves (coded by color) indicating the location of the displaced
interface for a number of times.} 
At the steady state, the solution is quadratic in $x$ and $y$ and so we would expect that
the second-order method used here would be exact. The table in Figure~\ref{tab:tableParabolicBeamAmp} 
gives the max-norm errors in the steady state solutions for a light ($\rhos\hs=10^{-3}$), medium ($\rhos\hs=1$), and 
heavy ($\rhos\hs=10$) beam. As expected, the AMP scheme is found to be stable and accurate in all three cases 
with the numerical approximation being exact up to roundoff. Note that the time to reach steady state
increases as the mass of the beam increases, as expected. 
{\bf For this problem the traditional partitioned scheme is found to be unstable 
when $\rhos\hs$ is less than $5$ (approximately). CHECK THIS AND SEE IF WE CAN MATCH WITH THEORY.}



{% ------ Parabolic Beam  ------
\newcommand{\figWidth}{8cm}
\newcommand{\trimfig}[2]{\trimFig{#1}{#2}{.02}{0.02}{.045}{.005}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  %\useasboundingbox (0.0,.75) rectangle (16.,5.5);  % set the bounding box (so we have less surrounding white space)
  \draw(0.0,0.0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/etaCenter.pdf}{\figWidth}};
   \draw(8.0,0.0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/vetaCenter.pdf}{\figWidth}};
% grid:
%  \draw[step=1cm,gray] (0,0) grid (16,5);
\end{tikzpicture}
\end{center}
  \caption{$\mu=0.2$, $\Ks=0$, $\Ts=5$, $\Es\Is=0$, $\Kt=0$, and $\Kxxt=0$.}
  \label{fig:ParabolicBeam}
\end{figure}
}
\tableParabolicBeamAmp


% ----------------------------------------------------------------------------------------------
\subsubsection{A beam with fluid on two sides}
For the case of a beam separating two rectangular fluid domains, 
the beam is assumed to have finite thickness $\hs$, and is chosen to initially lie along the x-axis and
occupy the domain $\Omegas(0)=[x_a,x_b]\times[-\hs/2,\hs/2]$. 
At time $t=0$, the lower fluid domain is the rectangular domain $\OmegaF_L(0)  = [x_a,x_b]\times[y_a,-\hs/2]$,
while the upper fluid domain is $\OmegaF_U(0)  = [x_a,x_b]\times[\hs/2,y_b]$.
The boundary conditions on the fluid domains are given as no-slip walls on the left and right with $\vv=0$, 
and constant pressure with zero tangential velocity on the top and bottom. The applied pressure
for the bottom and top are $p_a$ and $p_b$ respectively.
The initial conditions are zero fluid velocity and a stationary beam.

% The beam is pinned on both ends (displacement equal to zero).

% First consider a beam ({\em string model}) with properties $\Ts\ne 0$, and $\Es=0$, and pinned on both ends (displacement equal to zero).
% If a constant pressure $p_a$ is given on the bottom boundary and a constant pressure $p_b$ 
% is given on the top boundary, the analytic steady state solution for the beam displacement 
% is the parabola, 
% \begin{align}
%    \us_2 & = \frac{p_a-p_b}{2 \Ts} (x-x_a)(x_b-x) .
% \end{align}
% The analytic solution for the fluid in the lower domain consists of 
% a constant pressure state $p(\xv,t)=p_a$ and zero velocity, $\vv(\xv,t)=0$ for $\xv\in\Omega_L(t)$, while
% the upper fluid has a constant pressure $p(\xv,t)=p_b$ and zero velocity, $\vv(\xv,t)=0$ for $\xv\in\Omega_R(t)$.
% 
% For a beam with  $\Ts=0$, and $\Es\ne 0$, and clamped at both ends ($\us_2 $ and $\us_2'$ zero at both ends), the exact solution is a quartic 
% \begin{align}
%    \us_2 & = \frac{p_a-p_b}{24 \Es\Is} (x-x_a)^2 (x-x_b)^2 .
% \end{align}
% 
% % QUESTION: can we work out the time-dependent motion in the case when the beam moves slowly?
% 
% The initial conditions are chosen as $p(\xv,t)=p_a$, and $\vv(\xv,0)=0$ for $\xv\in\Omega_L(0)$ and
% $p(\xv,t)=p_b$, and $\vv(\xv,0)=0$ for $\xv\in\Omega_U(0)$.  (CHECK ME)
% % The coefficient of the linear damping term in the beam equation, $K_t$,  is taken to be a positive value
% % in order to accelerate the convergence to the steady state. 

For this case, and all subsequent cases, we will use the full DCG methodology as discussed in Section~\ref{sec:dcg}. 
The composite grid $\Gcpc^{(j)}$ for the geometry is shown in Figure~\ref{fig:partitionedChambersGrids}
and consists of two background Cartesian grids together with two body fitted grids adjacent to the top
and bottom sides of the interface, These grids are generated independently 
using the hyperbolic grids generator, and each  
has $6$ grids lines in the normal direction (so that this grid becomes thinner as
the composite grid is refined). The grid spacing on all component grids 
is chosen to be approximately $\Delta s^{(j)}=1/(10 j)$. 
% 
{\bf Is the following statement needed? Note that we have used a single fluid solver to advance both fluid domains: this implies there
is a single pressure equation being solved.} 

Here the material parameters for the beam are chosen to highlight two classes of beam models. In the first
case, known as a {\em string model}, the beam operator $L$ is dominated by a Laplacian and so the 
beam motion is governed by a wave equation in second-order form. For this second-order operator the 
steady state will be quadratic in $x$ and $y$ and the second-order accurate 
discretization is expected to yield exact results to machine precision. For the second case, known as a {\em beam model}, the beam
operator $L$ is dominated by a bi-harmonic operator. As a result, the steady state will be quartic in $x$ and $y$
and a second-order accurate operator is not expected to yield exact results.   

%  >>> t =  1.000e+01, dt = 6.85e-03, cpu = 4.54e+01 seconds (1445 steps)
%            p : (min,max)=(-1.165066e-07, 1.000001e+00) 
%            u : (min,max)=(-5.361090e-07, 4.917002e-06) 
%            v : (min,max)=(-4.017208e-06, 3.334336e-06) 
%  Divergence: divMax/vorMax = 1.52e-02 divl2Norm/vorMax=7.55e-04 vorMax=3.35e-05
% -- BM -- beam: Error t=1.000e+01 : uErr=(4.96e-08,6.97e-07)=(max,max/uNorm), vErr=(4.60e-08,4.60e+04)=(max,max/vNorm) (steps=1446)
%  >>> t =  5.000e+01, dt = 6.85e-03, cpu = 2.29e+02 seconds (7245 steps)
%            p : (min,max)=(-2.470246e-15, 1.000000e+00) 
%            u : (min,max)=(-4.385046e-16, 7.038391e-15) 
%            v : (min,max)=(-3.865316e-15, 2.511914e-15) 
%  Divergence: divMax/vorMax = 5.81e-01 divl2Norm/vorMax=1.00e-01 vorMax=3.05e-14
% -- BM -- beam: Error t=5.000e+01 : uErr=(3.89e-16,5.45e-15)=(max,max/uNorm), vErr=(8.72e-16,8.72e-04)=(max,max/vNorm) (steps=7246)


\paragraph{String model} The material and geometric parameters for this case are taken as
 $\hs=.1$, $\Ts=5$, $\Es\Is=0$, $K_t=6$, $\rho=1$, $\mu=.05$, $p_a=1$, $p_b=0$, $x_a=-1$, $x_b=1$, $y_a=-.5-\hs/2$ and $y_b=.5+\hs/2$. 
The beam is assumed pinned at both ends (displacement equal to zero), and the exact solution for the beam is
\begin{align}
   \eta & = \frac{p_a-p_b}{2 \Ts} (x-x_a)(x_b-x) ,
\end{align}
while the fluid velocity is $\vv=0$, and the fluid pressure is $p_a$ in the lower region and $p_b$ in the upper.
% 
The problem is solved for both a range of beam densities with $\rhos\hs=.01, .1, 1, 10$. 
In all cases the AMP scheme is found to be 
stable and the solution convergences to the {\em exact} steady state solution as expected.
On the other hand, the traditional scheme is found to be stable for $\rhos\hs=10$ but unstable for $\rhos\hs=1$. 
As a representative example, Figure~\ref{fig:partitionedChambersGrids} shows the solution at $t=0$ and $t=10$ for this string
model with $\rhos\hs=.1$. In this case 
% $\Ts=5$,  and $\Es\Is=0$, 
% for $\rhos=1$ and damping coefficient $K_t=6$.
the maximum displacement of the beam in the
steady state is $0.1$. 
The maximum error in the beam displacement (compared to the steady state solution) is approximately $5\times 10^{-8}$ at $t=10$,
and reaches round-off errors of $4\times 10^{-16}$ by $t=50$. 
{% ------ STRING GRIDS ------
\newcommand{\figWidth}{8cm}
\newcommand{\trimfig}[2]{\trimFig{#1}{#2}{.02}{0.02}{.285}{.285}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.0,.75) rectangle (16.,5.1);  % set the bounding box (so we have less surrounding white space)
%   \draw(0.0,4.4) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/fc2Gridt0p010}{\figWidth}};
  \draw(0.0,0.0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/flexiblePartition2Gridt00}{\figWidth}};
  \draw(8.0,0.0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/flexiblePartition2Gridt10}{\figWidth}};
% grid:
%  \draw[step=1cm,gray] (0,0) grid (16,5);
\end{tikzpicture}
\end{center}
  \caption{Composite grids for the partitioned chambers with the string model (quadratic steady state), 
    coarse grid $\Gcpc^{(2)}$ at $t=0$ and $t=10$. 
    The figure on the right shows the solution when the beam has nearly reached the steady state solution. 
    The parameters were chosen as $\rhos\hs=.1$ (light beam), $\Ts=5$, $\Es\Is=0$, and $p_a-p_b=1$. 
  }
  \label{fig:partitionedChambersGrids}
\end{figure}
}

\paragraph{Beam model} The material and geometric parameters for this case are taken as 
$\hs=.1$, $\Es\Is=0.2$, $\Ts=0$, $K_t=5$, $\rho=1$, $\mu=.05$, $p_a=1$, $p_b=0$, $x_a=-1$, $x_b=1$, $y_a=-.5-\hs/2$ and $y_b=.5+\hs/2$. 
The beam is clamped at both ends ($\eta $ and $\eta'$ zero) and the exact steady solution for the beam displacement is the fourth-degree polynomial, 
\begin{align}
   \eta & = \frac{p_a-p_b}{24 \Es\Is} (x-x_a)^2 (x-x_b)^2 .
\end{align}
% 
As before the fluid velocity is $\vv=0$, and the fluid pressure is $p_a$ in the lower region and $p_b$ in the upper.
The problem is again solved for a range of beam densities with $\rhos\hs=.01, .1, 1, 10$. 
In all  cases the AMP scheme is found to be 
stable and the solution convergences {\bf this can't be right ... we probably want to do a convergence study for this case
right?} to the {\em exact} steady state solution (the numerical approximation being
able to exactly approximate the true solution up to round-off errors). 
The traditonal scheme is found to be stable for $\rhos\hs=10$ but becomes unstable around $\rhos\hs=1$. 
Figure~\ref{fig:partitionedChambersBeamGrids} shows a representative solution at $t=0$ and $t=10$ with
$\rhos\hs=0.1$. 
%  for the beam $\Es\Is=0.2$, $\Ts=0$,  for $\rhos=1$ and damping coefficient $K_t=5$. For these parameters 
Here maximum displacement of the beam in the steady state is approximately $0.208$. 
The maximum error in the beam displacement (compared to the steady state solution) is approximately $4\times 10^{-7}$  at $t=10$,
and reaches $10^{-15}$ by $t=50$. 



{% ------ BEAM GRIDS ------
\newcommand{\figWidth}{8cm}
\newcommand{\trimfig}[2]{\trimFig{#1}{#2}{.02}{0.02}{.285}{.285}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.0,.75) rectangle (16.,5.1);  % set the bounding box (so we have less surrounding white space)
%   \draw(0.0,4.4) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/fc2Gridt0p010}{\figWidth}};
  \draw(0.0,0.0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{flexibleChannel/flexiblePartition2BeamGridt00}{\figWidth}};
  \draw(8.0,0.0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{flexibleChannel/flexiblePartition2BeamGridt10}{\figWidth}};
% grid:
%  \draw[step=1cm,gray] (0,0) grid (16,5);
\end{tikzpicture}
\end{center}
  \caption{Composite grids for the partitioned chambers with the beam model (quartic steady state), coarse grid $\Gcpc^{(2)}$ at $t=0$ and $t=10$. 
    The figure on the right shows the solution when the beam has nearly reached the steady state solution. 
    The parameters were chosen as $\rhos\hs=.1$ (light beam), $\Ts=0$, $\Es\Is=.2$, and $p_a-p_b=1$. 
  }
  \label{fig:partitionedChambersBeamGrids}
\end{figure}
}

% ----------------------------------------------------------------------------------------------
\subsection{A flexible partition separating two fluid chambers - time dependent solution}  \label{sec:flexibleChannelTD}

Consider the geometry of a beam separating two fluid domains as described in Section~\ref{sec:flexibleChannelSS}. 
Suppose that on the vertical walls, the beam is allowed to slide up and down, and the fluid satisfies
a slip-wall condition, then 
an exact time-dependent solution can be determined which consists of a flat horizontal beam oscillating up and down.
% provided the beam ends are allowed to slide and slip-wall boundarty conditions are used for the fluid.
This solution is used to assess the time accuracy and stability of the AMP scheme. 

% When the beam ends are allowed to slide up and down along the
% left and right walls, and slip conditions are used for the fluid on these vertical walls,
% an exact time-dependent solution can be determined which consists of a flat horizontal beam oscillating up and down. 

% We take slip wall boundary conditions for the fluid domains on the left and right, and free boundary
% conditions on the beam so that the ends are allowed to slide up and down.

{% ------ OSCILLATING BEAM FIGURE ------
\newcommand{\figWidth}{8cm}
\newcommand{\trimfig}[2]{\trimFig{#1}{#2}{.0}{0.0}{.0}{.0}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.0,.75) rectangle (9,8);  % set the bounding box (so we have less surrounding white space)
  \draw(0.0,0.0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{flexibleChannel/oscillatingBeamRhosHs0p1}{\figWidth}};
% grid:
% \draw[step=1cm,gray] (0,0) grid (8,7);
\end{tikzpicture}
\end{center}
\caption{Oscillating beam between two fluids, beam vertical displacement and velocity for $\rhos\hs=0.1$ compared
to the exact solution.}\label{fig:oscillatingBeam}
\end{figure}
}

% An exact time-dependent solution can be determined when the pressures on the bottom and top
Let the pressures on the bottom and top boundaries 
be specified as functions of time but indepdendent of $x$, $p(x,y_a,t)=p_a(t)$ and $p(x,y_b,t)=p_b(t)$. 
In this case the solution is independent of $x$. 
Let $y=\eta(t)$, denote the vertical displacement of the beam.
From the governing equations it follows that $p_{yy}(x,y,t)=0$ with boundary conditions $p(x,y_a,t)=p_a(t)$ on the bottom, 
$p(x,y_b,t)=p_b(t)$ on the top, 
and (compatibility conditions) $p_y(x,\eta\pm\hs/2,t)=\rho \eta_{tt}$ on the beam. Thus 
the fluid pressure is a linear function of $y$ in each domain with $y$-derivative equal to $-\rho\eta_{tt}$,
\begin{align*}
   p(x,y,t) = \begin{cases}
                    p_a(t) -\rho \eta_{tt} (y-y_a) & y\in [y_a,\eta-\hs/2], \\
                    p_b(t) -\rho \eta_{tt} (y-y_b) & y\in [\eta+\hs/2,y_b],
              \end{cases} 
\end{align*}
while the fluid velocity is constant in space with $v_1(x,y,t)=0$ and $v_2(x,y,t)=\eta_t(t)$. 
% For a beam with fluid on the top and bottom 
Whence the equation of motion for the beam is (the terms involving $x$-derivatives drop out)
\begin{align*}
   \rhos\As \eta_{tt} & = - K_0 \eta - \Kt \eta_t + p(x,\eta-\hs/2,t) - p(x,\eta+\hs/2,t) , \\
     %                & = - K_0 \eta - \Kt \eta_t + p_a(t)  + (-\rho\eta_{tt})(\eta-\hs/2-y_a) 
     %                                         - p_b(t) - (-\rho \eta_{tt})(\eta+\hs/2-y_b) , \\
                    & = - K_0 \eta - \Kt \eta_t + p_a(t)- p_b(t)  -\rho\eta_{tt} (y_b-y_a - \hs), 
\end{align*}
which leads to the linear ordinary differential equation governing the vertical displacement of the beam
\begin{align}
   (\rhos\As + \rho H )\eta_{tt} = - K_0 \eta - \Kt \eta_t  + p_a(t) - p_b(t), \label{eq:oscillatingBeam}
\end{align}
where $H=y_b-y_a - \hs$ is the total depth of the two fluid domains. The coefficient, $\rhos\As + \rho H$, of
$\eta_{tt}$ in equation~\eqref{eq:oscillatingBeam} is seen to consist of the mass of the beam, $\rhos\hs$ and
the added mass of the fluid, $\rho H$. 
% 
For a constant pressure difference $\Delta p = p_a-p_b$ and $K_0\ne 0$, $K_t=0$, the solution for
initial conditions $\eta(0)=0$ and $\eta_t(0)=0$ is
\begin{align*}
&   \eta(t) = \frac{\Delta p}{K_0} \Big( 1 - \cos(\omega t) \Big), \qquad
   \omega=\sqrt{\frac{K_0}{\rhos\As + \rho H}}.
\end{align*}
The beam
parameters were taken as $\Es\Is=10^{-4}$ and $\Ts=10^{-2}$ (these values should not play a role, other
than affecting the choice of time-step, since the beam is flat).

% ----- tables ----
\input texFiles/beamPistonTables

Figure~\ref{fig:oscillatingBeam} shows the computed values of $\eta(t)$ and $\eta_t(t)$ compared to
the exact solution for $\rhos\hs=0.1$ and $\Ks_0=10$ on the grid $\Gcpc^{(2)}$. 
The differences between the computed and exact solutions are near indistinguishable.
The tables in Figure~\ref{tab:beamPiston} shows the max-norm errors and estimated convergence rates for a
light beam, $\rhos\hs=10^{-2}$ and a heavy beam $\rhos\hs=10$.  
The maximum errors are converging close to fourth-order accuracy. Recall that the beam solver is 
fourth-order accurate in space and second-order order accurate in time but converges as fourth-order overall
when the time-step scales as $\dt \propto \dx^2$. 
% Note that the global time-step $\dt$ is determined from the maximum allowable time steps for the fluid and beam.
% Since the beam time step is proprotional to $\Es\Is\dx^2$ 






% \input fig/exact.beamPistonRhos10p0.pc.flexiblePartition.ins.order2.ConvTable.tex
% \input fig/exact.beamPistonRhos0p1.pc.flexiblePartition.ins.order2.ConvTable.tex

%- NOTE: For a beam with fluid on the lower side only, and a pressure $p=p_b(t)$ imposed on the top of the
%- beam, the motion of the beam is governed by 
%- \begin{align*}
%-    \rhos\As \ddot \eta & = - K_0 \eta - K_t \dot \eta + p_a(t)  + (-\rho\ddot \eta)(\eta-\hs/2-y_a) 
%-                                              - p_b(t) 
%- \end{align*}
%- which results in the {\em nonlinear} ODE *CHECK ME*
%- \begin{align*}
%-    (\rhos\As + \rho(\eta-\hs/2-y_a) ) \ddot \eta & = - K_0 \eta - K_t \dot \eta + p_a(t) - p_b(t) 
%- \end{align*}




==> texFiles/governingEquations-5-5-15.tex <==

\renewcommand{\sv}{{s}}

\section{Governing equations}\label{sec:governingEquations}

We consider the fluid-structure coupling of an incompressible fluid and a thin deformable structure.  The fluid occupies the domain $\xv\in\OmegaF(t)$ while the structure lies in the domain $\xv\in\OmegaS(t)$, where $\xv$ is position and $t$ is time.  The coupling of the fluid and structure occurs along the interface $\Gamma(t)$, see Figure~\ref{fig:genericBeamCartoon}.  It is assumed that the fluid is governed by the incompressible Navier-Stokes equations, which in an Eulerian frame are given by 
\begin{alignat}{3}
  &  \frac{\partial\vv}{\partial t} + (\vv\cdot\grad)\vv 
                 =  \frac{1}{\rho} \grad\cdot\sigmav  , \qquad&& \xv\in\OmegaF(t) ,  \label{eq:fluidMomentum}  \\
  & \grad\cdot\vv =0,  \quad&& \xv\in\OmegaF\new{(t)} ,  \label{eq:fluidDiv3d}
\end{alignat}
where $\rho$ is the (constant) fluid density and $\vv=\vv(\xv,t)$ is the fluid velocity.  The fluid stress tensor, $\sigmav=\sigmav(\xv,t)$, is given by 
\begin{equation}
  \sigmav = -p \Iv + \tauv,\qquad \tauv = \mu \left[ \grad\vv + (\grad\vv)^T \right],
  \label{eq:fluidStress}
\end{equation}
where $p=p(\xv,t)$ is the pressure, $\Iv$ is the identity tensor, $\tauv$ is the viscous stress tensor, and $\mu$ is the (constant) fluid viscosity. For future reference, the components of a vector such as $\vv$ will be denoted by $v_m$, $m=1,2,3$ (i.e.~$\vv=[v_1, v_2, v_3]^T$), while components of a tensor such as $\sigmav$ will be denoted by $\sigma_{mn}$, $m,n=1,2,3$.  The velocity-divergence form of the equations given by~\eqref{eq:fluidMomentum} and~\eqref{eq:fluidDiv3d} require appropriate initial and boundary conditions, as well as conditions on $\Gamma(t)$ where the behavior of the fluid is coupled to that of the solid (as discussed below).

\input texFiles/genericBeamCartoon.tex

An elliptic equation for the fluid pressure can be derived from~\eqref{eq:fluidMomentum}--\eqref{eq:fluidStress} as
\begin{alignat}{3}
  &  \Delta p &= - \rho \grad\vv:(\grad\vv)^T ,  \qquad&& \xv\in\OmegaF(t) . \label{eq:fluidPressure}
\end{alignat}
In the pressure-velocity form of the incompressible Navier-Stokes equations~\eqref{eq:fluidPressure} is used in place of~\eqref{eq:fluidDiv3d}. This form requires an additional boundary condition, and a natural choice uses $\grad\cdot\vv=0$ for $\xv\in\partial\OmegaF(t)$, see~\cite{ICNS} for example.

The structure is assumed to be thin and governed by a beam model, which describes the evolution of the displacement, $\uvs=\uvs(\sv,t)$, of a reference centerline curve of the beam as a function of a Lagrangian coordinate $\sv\in\OmegaSbar$ and time $t$.  (Overbars are used throughout to denote quantities belonging to the structure.)  The beam model has the form
\begin{alignat}{3}
  \rhos \As \frac{\partial^2 \uvs}{\partial t^2} =& \Lvs(\uvs,\vvs) +\fsv(\sv,t), \qquad && \sv\in\OmegaSbar,
     \label{eq:beamEquation}
\end{alignat}
where $\rhos$ is the (constant) beam density, $\As=\As(\sv)$ is the cross-sectional area of the beam, $\Lvs$ is the internal restoring force per unit length which depends on $\uvs$ and on the velocity, $\vvs=\partial \uvs/\partial t$, of the reference curve (in general), and $\fsv$ is the external force per unit length on the beam from the fluid (defined below).  In physical space, the position of the reference curve is given by
\[
\xv=\xvb(\sv,t)=\xvb(\sv,0)+\uvs(\sv,t),\qquad \sv\in\OmegaSbar,
\]
where $\xvb(\sv,0)$ is the initial position of the reference curve of the beam.  The positions of the upper and lower surfaces of the beam, denoted by $\xsv_+(\sv,t)$ and $\xsv_-(\sv,t)$, respectively, are determined by
\begin{equation}
\xsv_\pm(\sv,t)=\xvb(\sv,t)+\xvz_\pm(\sv,t),\qquad \sv\in\OmegaSbar,
\label{eq:surfaces}
\end{equation}
where $\xvz_\pm$ measures distance from the reference surface to account for the finite thickness of the beam.  The upper and lower surfaces of the beam define the position of the fluid-structure interface $\Gamma(t)$ (see Figure~\ref{fig:genericBeamCartoon}).

At the fluid-structure interface, the velocity of the fluid at a point on the surface of the beam matches the corresponding velocity of the beam surface,
\begin{align}
    \vv(\xsv_\pm(\sv,t),t) &= \frac{\partial}{\partial t}\xsv_{\pm}(\sv,t), \qquad \sv\in\OmegaSbar, \label{eq:kinematicII}
\end{align}
where $\xsv_{\pm}$ is given in~(\ref{eq:surfaces}).  Velocities of the upper and lower surfaces of the beam are thus given by 
\begin{align}
   \vsv_\pm (\sv,t)=  \frac{\partial}{\partial t}\xsv_{\pm}(\sv,t) = \vsv(\sv,t) + \wsv_\pm(\sv,t) ,\label{eq:beamSurfaceVelocity}
\end{align}
where $\wsv_\pm=\partial\xvz_\pm/\partial t$.  Formulas for the finite-thickness corrections, $\xvz_\pm$ and $\wsv_\pm$, are given in Section~\ref{sec:beamModels} for the case of an Euler-Bernoulli beam model.  The dynamic matching condition (balance of forces) defines the force on the beam, $\fsv$, in (\ref{eq:beamEquation}) in terms of the fluid forces on the upper and lower surfaces of the beam,
% WE NEED A DIFFERENT NOTATION to differentiate between $(\sigmav\nv)_+(\ss,t)$ on the reference line and $(\sigmav\nv)_+$ on the surface!
\begin{align}
    \fsv(\sv,t)  &= - \Big[ (\sigmav\nv)_+(\sv,t)+ (\sigmav\nv)_-(\sv,t) \Big], \qquad \sv\in\OmegaSbar , \label{eq:dynamic} 
\end{align} 
where
\begin{align}
    (\sigmav\nv)_\pm(\sv,t) &\equiv \sigmav(\xsv_\pm(\sv,t),t)\,\nv(\xsv_\pm(\sv,t),t).
\end{align} 
Here, $\nv$ denotes the unit normal to the beam surface (outward pointing from the fluid domain). 




==> texFiles/governingEquations-orig.tex <==


\section{Governing equations}\label{sec:governingEquations}


We consider the fluid-stucture coupling on a incompressible fluid on the \new{deforming} domain $\OmegaF(t)$ and a thin structure
on an interface $\Gamma(t)$ of $\OmegaF(t)$.
The fluid is governed by the incompressible Navier-Stokes equations \old{in the domain $\OmegaF$} which in an Eulerian
frame are given by 
\begin{alignat}{3}
  &  \frac{\partial\vv}{\partial t} + (\vv\cdot\grad)\vv 
                 =  \frac{1}{\rho} \grad\cdot\sigmav  , \qquad&& \xv\in\OmegaF(t) ,  \label{eq:fluidMomentum}  \\
  & \grad\cdot\vv =0,  \quad&& \xv\in\OmegaF\new{(t)} ,  \label{eq:fluidDiv3d}
\end{alignat}
where $\xv$ is position, $t$ is time, $\rho$ is the (constant) fluid density, and $\vv=\vv(\xv,t)$ is the fluid velocity.
The fluid stress tensor, $\sigmav=\sigmav(\xv,t)$, is given by 
\begin{equation}
  \sigmav = -p \Iv + \tauv,\qquad \tauv = \mu \left[ \grad\vv + (\grad\vv)^T \right],
  \label{eq:fluidStress}
\end{equation}
where $p$ is the pressure, $\Iv$ is the identity tensor, $\tauv$ is the viscous stress tensor, and $\mu$ is the (constant) fluid viscosity. 
For future reference, 
the components of a vector, such as $\vv$ will be denoted by $v_m$, $m=1,2,3$, (i.e. $\vv=[v_1, v_2, v_3]^T$), while components
of a tensor such as $\sigmav$, will be denoted by $\sigma_{mn}$, $m,n=1,2,3$.
%
\old{The equations~\eqref{eq:fluidMomentum}-\eqref{eq:fluidDiv3d}} \new{Equations~\eqref{eq:fluidMomentum}-\eqref{eq:fluidDiv3d}} are augmented by appropriate initial \old{conditions} and
boundary conditions. 
\old{The pressure satisfies the elliptic equation
\begin{alignat}{3}
  &  \Delta p &= - \rho \grad\vv:\grad\vv ,  \qquad&& \xv\in\OmegaF(t) . \label{eq:fluidPressure}
\end{alignat}
In the pressure-velocity form of the incompressible Navier-Stokes,
one solves~\eqref{eq:fluidMomentum} and~\eqref{eq:fluidPressure} in the interior of the domain and
equation~\eqref{eq:fluidDiv3d} is dropped.  The pressure-velocity system requires an additional boundary
condition and a natural choice is to take $\grad\cdot\vv =0$ to be this boundary condition~\cite{ICNS}.}
\new{From \eqref{eq:fluidMomentum}-\eqref{eq:fluidStress}, one can derive an elliptic equation for the 
fluid pressuree as
\begin{alignat}{3}
  &  \Delta p &= - \rho \grad\vv:\grad\vv ,  \qquad&& \xv\in\OmegaF(t) . \label{eq:fluidPressure}
\end{alignat}
In the pressure-velocity form of the incompressible Navier-Stokes equations~\eqref{eq:fluidPressure}
is used in place of~\eqref{eq:fluidDiv3d}. This pressure-velocity system requires an additional boundary
condition and one natural choice is to take $\grad\cdot\vv =0$ to be this boundary condition~\cite{ICNS}.}


The evolution of the 
thin structure is assumed governed by a beam model, which in a Lagrangian frame
is given by the equations 
\begin{alignat}{3}
  \rhos \As \frac{\partial^2 \uvs}{\partial t^2} =& \Lvs(\uvs,\vvs) +\fsv(s,t), \quad && \ss\in[0,\ls], \quad t\ge 0,
     \label{eq:beamEquation}
\end{alignat}
where $\uvs(\ss,t)$ is the displacement of the beam reference-line (or center-line), 
$\vvs=\partial \uvs/\partial t$ is the corresponding beam velocity, 
$\Lvs$ is the beam operator, $\fsv$ the force on the beam from the fluid (defined below), 
$\As$ is the cross-sectional area of the beam ($\As=\hs\bs$ for a beam of constant thickness, $\hs$ and constant breadth $\bs$ in the z-direction), 
$\rhos$ is the beam density, $\ls$ is the length of the undeformed beam. 

The dynamic matching condition (balance of forces) 
defines the force on the beam in terms of the fluid forces on the upper and lower surfaces of the beam,
% WE NEED A DIFFERENT NOTATION to differentiate between $(\sigmav\nv)_+(\ss,t)$ on the reference line and $(\sigmav\nv)_+$ on the surface!
\begin{align}
    \fsv(\ss,t)  &= - \Big[ (\sigmav\nv)_+(\ss,t)+ (\sigmav\nv)_-(\ss,t) \Big], \qquad \ss\in[0,\ls] , \label{eq:dynamic} 
\end{align} 
where
\begin{align}
    (\sigmav\nv)_\pm(\ss,t) &\equiv \sigmav(\xsv_\pm(\ss,t),t)\,\nv(\xsv_\pm(\ss,t),t).
\end{align} 
Here $\nv$ denotes the unit normal to the beam surface (outward pointing from the fluid domain) while
$\xsv_+(\ss,t)$ and $\xsv_-(\ss,t)$ denote points on the upper and lower surfaces of the beam, respectively. 


The kinematic matching condition at the fluid-structure interface is that the velocity of the fluid at a point on the surface of
the beam matches the corresponding velocity of the beam surface,
\begin{align}
    \vv(\xsv_\pm(\ss,t),t) &= \frac{\partial}{\partial t}\xsv_{\pm}(\ss,t), \qquad\qquad \ss\in[0,\ls]. \label{eq:kinematicII}
\end{align} 
The velocity of the beam {\em surface} is written as the sum of the velocity of the beam reference line
plus a correction due to finite width beams, 
\begin{align}
   \vsv_\pm (\ss,t)=  \frac{\partial}{\partial t}\xsv_{\pm}(\ss,t) = \vsv(\ss,t) + \wsv_\pm(\ss,t) .\label{eq:beamSurfaceVelocity}
\end{align} 
The form of the correction $\wsv_\pm$ for Euler-Bernoulli beams is given in Section~\ref{sec:beamModels}.


==> texFiles/matlabResults-orig.tex <==
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}} % partial derivatives \pd{u}{x}
\newcommand{\pdn}[3]{\frac{\partial^{#3} #1}{\partial #2^{#3}}} % higher partial derivatives \pd{u}{x}{n}
%tables
\newcommand{\tableTZAmp}{%
  \begin{figure}[hbt]\tableFont %
    \begin{center}
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline 
%\multicolumn{11}{|c|}{\strutt  light beam, $\rhos\hs=10^{-3}$} \\ \hline 
%\strutt~~$h_j$~~& $E_j^{(p)}$ & $r$ & $E_j^{(u)}$ & $r$ & $E_j^{(v)}$ & $r$ & $E_j^{(\eta)}$ & $r$   & $E_j^{(\vsv)}$  & $r$  \\ \hline 
%1/20 & 2.49e-02 &   & 1.85e-02  &   & 1.38e-02  &   & 3.06e-04  &   & 7.77e-03  &    \\ \hline
%1/40 & 6.50e-03 & 3.83  & 4.96e-03  & 3.73  & 3.61e-03  & 3.82  & 1.00e-04  & 3.06  & 2.36e-03  & 3.29   \\ \hline
%1/80 & 1.64e-03 & 3.96  & 1.26e-03  & 3.94  & 9.15e-04  & 3.95  & 2.68e-05  & 3.74  & 6.12e-04  & 3.86   \\ \hline
%rate &  1.96 &   &  1.94  &   &  1.96  &   &  1.76  &   &  1.76  &    \\ \hline
%\end{tabular}
%
%
%
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline 
%\multicolumn{11}{|c|}{\strutt  medium beam, $\rhos\hs=1$} \\ \hline 
%\strutt~~$h_j$~~& $E_j^{(p)}$ & $r$ & $E_j^{(u)}$ & $r$ & $E_j^{(v)}$ & $r$ & $E_j^{(\eta)}$ & $r$   & $E_j^{(\vsv)}$  & $r$  \\ \hline 
%1/20 & 5.07e-02 &   & 1.92e-02  &   & 1.49e-02  &   & 8.64e-05  &   & 2.18e-03  &    \\ \hline
%1/40 & 1.41e-02 & 3.60  & 5.16e-03  & 3.73  & 3.99e-03  & 3.75  & 3.10e-05  & 2.79  & 6.94e-04  & 3.14   \\ \hline
%1/80 & 3.68e-03 & 3.83  & 1.31e-03  & 3.94  & 1.01e-03  & 3.93  & 8.44e-06  & 3.68  & 1.86e-04  & 3.74   \\ \hline
%rate &  1.89 &   &  1.94  &   &  1.94  &   &  1.68  &   &  1.68  &    \\ \hline
%\end{tabular}
%
%
%
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline 
%\multicolumn{11}{|c|}{\strutt  heavy beam, $\rhos\hs=10^{3}$} \\ \hline 
%\strutt~~$h_j$~~& $E_j^{(p)}$ & $r$ & $E_j^{(u)}$ & $r$ & $E_j^{(v)}$ & $r$ & $E_j^{(\eta)}$ & $r$   & $E_j^{(\vsv)}$  & $r$  \\ \hline 
%1/20 & 7.81e-02 &   & 1.97e-02  &   & 1.64e-02  &   & 2.83e-05  &   & 9.68e-04  &    \\ \hline
%1/40 & 1.96e-02 & 3.98  & 5.27e-03  & 3.73  & 4.44e-03  & 3.69  & 8.04e-06  & 3.52  & 2.40e-04  & 4.03   \\ \hline
%1/80 & 4.94e-03 & 3.97  & 1.34e-03  & 3.94  & 1.13e-03  & 3.91  & 2.05e-06  & 3.92  & 5.99e-05  & 4.01   \\ \hline
%rate &  1.99 &   &  1.94  &   &  1.93  &   &  1.89  &   &  1.89  &    \\ \hline
%\end{tabular}


\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline 
\multicolumn{11}{|c|}{\strutt  light beam, $\rhos\hs=10\sp{-3}$} \\ \hline 
\strutt~~$h_j$~~& $E_j^{(p)}$ & $r$ & $E_j^{(u)}$ & $r$ & $E_j^{(v)}$ & $r$ & $E_j^{(\eta)}$ & $r$   & $E_j^{(\dot\eta)}$  & $r$  \\ \hline 
1/10 & 6.55e-02 &  0.00  & 2.64e-02  &  0.00  & 2.23e-02 &  0.00  & 9.06e-04  &  0.00  & 2.19e-02  &  0.00   \\ \hline
1/20 & 1.70e-02 &  3.84  & 7.26e-03  &  3.64  & 5.41e-03 &  4.12  & 2.23e-04  &  4.07  & 5.15e-03  &  4.25   \\ \hline
1/40 & 4.45e-03 &  3.83  & 1.86e-03  &  3.91  & 1.39e-03 &  3.90  & 6.03e-05  &  3.69  & 1.31e-03  &  3.94   \\ \hline
1/80 & 1.12e-03 &  3.98  & 4.70e-04  &  3.95  & 3.55e-04 &  3.91  & 1.54e-05  &  3.90  & 3.29e-04  &  3.97   \\ \hline
rate &  1.96 &   &  1.94  &   &  1.99  &   &  1.95  &   &  2.01  &    \\ \hline
\end{tabular}



\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline 
\multicolumn{11}{|c|}{\strutt  medium beam, $\rhos\hs=1$} \\ \hline 
\strutt~~$h_j$~~& $E_j^{(p)}$ & $r$ & $E_j^{(u)}$ & $r$ & $E_j^{(v)}$ & $r$ & $E_j^{(\eta)}$ & $r$   & $E_j^{(\dot\eta)}$  & $r$  \\ \hline 
1/10 & 1.18e-01 &  0.00  & 2.07e-02  &  0.00  & 2.40e-02 &  0.00  & 3.56e-04  &  0.00  & 9.09e-03  &  0.00   \\ \hline
1/20 & 2.53e-02 &  4.69  & 5.86e-03  &  3.53  & 5.80e-03 &  4.14  & 7.70e-05  &  4.63  & 1.89e-03  &  4.80   \\ \hline
1/40 & 6.49e-03 &  3.90  & 1.54e-03  &  3.80  & 1.52e-03 &  3.82  & 2.02e-05  &  3.81  & 4.61e-04  &  4.11   \\ \hline
1/80 & 1.67e-03 &  3.89  & 3.95e-04  &  3.90  & 3.87e-04 &  3.92  & 5.10e-06  &  3.96  & 1.15e-04  &  4.02   \\ \hline
rate &  2.04 &   &  1.91  &   &  1.98  &   &  2.03  &   &  2.10  &    \\ \hline
\end{tabular}



\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline 
\multicolumn{11}{|c|}{\strutt  heavy beam, $\rhos\hs=10\sp{3}$} \\ \hline 
\strutt~~$h_j$~~& $E_j^{(p)}$ & $r$ & $E_j^{(u)}$ & $r$ & $E_j^{(v)}$ & $r$ & $E_j^{(\eta)}$ & $r$   & $E_j^{(\dot\eta)}$  & $r$  \\ \hline 
1/10 & 1.73e-01 &  0.00  & 2.06e-02  &  0.00  & 2.80e-02 &  0.00  & 8.45e-05  &  0.00  & 2.91e-03  &  0.00   \\ \hline
1/20 & 3.33e-02 &  5.20  & 5.63e-03  &  3.66  & 6.68e-03 &  4.20  & 2.25e-05  &  3.76  & 7.72e-04  &  3.77   \\ \hline
1/40 & 8.83e-03 &  3.77  & 1.51e-03  &  3.74  & 1.77e-03 &  3.77  & 6.37e-06  &  3.53  & 1.91e-04  &  4.05   \\ \hline
1/80 & 2.31e-03 &  3.82  & 3.90e-04  &  3.86  & 4.54e-04 &  3.90  & 1.63e-06  &  3.92  & 4.75e-05  &  4.01   \\ \hline
rate &  2.06 &   &  1.91  &   &  1.98  &   &  1.89  &   &  1.98  &    \\ \hline
\end{tabular}

\caption{Maximum-norm errors and estimated convergence rates using manufactured solution. The column labeled ``r'' provides the
  ratio of the errors at the current grid spacing to that on the next coarser grid. }
\label{tab:tableTZAmp}
\end{center}
\end{figure}
}


\newcommand{\tableParabolicBeamAmp}{%
  \begin{figure}[hbt]\tableFont %
    \begin{center}
      \begin{tabular}{|c|c|c|c|c|c|c|} \hline 
          \strutt~~$\bar{\rho}{\bar{h}}$~~& $t$ & $E_j^{(p)}$  & $E_j^{(u)}$  & $E_j^{(v)}$  & $E_j^{(\eta)}$    & $E_j^{(\vsv)}$    \\ \hline
        1e-3 & 30  &  1.50e-12  & 7.06e-14  & 2.25e-13   & 2.00e-15 & 2.25e-13     \\ \hline
        1     &  50  & 4.53e-12  &  3.73e-14   & 7.15e-13   & 1.80e-13 & 7.15e-13     \\ \hline
        10 & 250  & 4.19e-12  & 3.84e-14   & 2.63e-12  & 9.08e-14 &2.63e-12   \\ \hline
      \end{tabular}
\caption{Results of the evolution to steady state.}
\label{tab:tableParabolicBeamAmp}
\end{center}
\end{figure}
}





%- \subsection{Verification for a channel with a flexible wall (Matlab solver)} \label{sec:matlabResults}
%- In this section, we verify the stability and accuracy of the AMP scheme by solving test problems on a deforming domain.
%- We use a relatively simple geometry (a channel with a flexible wall) to represent a beam with fluid on one side. To be specific, the fluid domain at $t$ is $\Omega_{L}(t) =[0,1]\times[0,\eta(x,t)+1]$ with a beam lying on the top, where $\eta(x,t)$ is the displacement of the beam. The computational grid is generated using transfinite interpolation (TFI) as shown in Figure~\ref{fig:TFIgrids}, and  the TFI mapping is given by
%- $$
%- (x,y) = \mathbf{g}(r,s,t):= (r,s(\eta+1)),~(r,s)\in [0,1]\times[0,1].
%- $$
%- As a simplified model, a beam with property $\bar{E}=0$ is considered,  and the interface conditions are applied directly on the centerline rather than on the surface of the beam.  We note that results in this section were implemented in a Matlab based FSI solver and thus repesent an independently developed and verified code for the FSI problem.  
%{% ------ GRIDS ------
%\newcommand{\figWidth}{7cm}
%\newcommand{\trimfig}[2]{\trimFig{#1}{#2}{.02}{0.02}{.085}{.185}}
%\begin{figure}[htb]
%\begin{center}
%\begin{tikzpicture}[scale=1]
%  \useasboundingbox (0.0,.75) rectangle (7.,7.);  % set the bounding box (so we have less surrounding white space)
%  \draw(0.0,0.0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/TFIgrid.pdf}{\figWidth}};
%% grid:
%% \draw[step=1cm,gray] (0,0) grid (14,5);
%\end{tikzpicture}
%\end{center}
%  \caption{Computational grids at $t=0.1$ for the manufactured solution example.}
%  \label{fig:TFIgrids}
%\end{figure}
%}

% ----------------------------------------------------------------------------------------
\subsection{Manufactured Solutions} \label{sec:manufacturedSolutions}

The method of manufactured solutions~\cite{CGNS,Roache1998} can be used to construct exact
solutions of FSI problems by adding forcing functions to the governing
equations. The forcing is specified so that a chosen function becomes an exact solution to the forced equations. Here the approach is used to verify the stability and accuracy of the numerical approach for a nonlinear 
FSI problem consisting of an initially rectangular fluid domain bounded by a flexible beam along its top surface with vertical displacement $\eta(x,t)$. For this simple geometry the fluid domain,
$\OmegaF(t) =[0,1]\times[0,1+\eta(x,t)]$, is represented by a single transfinite interpolation (TFI) grid, as shown in Figure~\ref{fig:lightBeamError}. The TFI mapping is given by
\[
(x,y) = \mathbf{g}(r,s,t)\equiv(r,s(1+\eta)),\qquad (r,s)\in [0,1]\times[0,1].
\]
\textcolor{red}{(Comment: the notation is unfortunate here.  Previously, we used $s$ to be the Lagrangian coordinate measuring distance along the beam.  Now it is a component in the TFI mapping.  I am not sure the best way to remove this possible confusion.  One possibility is to stick with subscripts: $(x_1,x_2)$, $(r_1,r_2)$, $(v_1,v_2)$, etc.)}
 
The parameters for the fluid are chosen to be ({\bf CHECK ME}) $\rho=1$ and $\mu=0.05$.  The thickness of the beam is taken to be zero while the finite mass of the beam given by $\rhos\hs$ is varied to consider the cases of light, medium and heavy beams.  The remaining parameters of the beam are assumed to be $\Ks=1$, $\Ts=\rhos\hs$ and $\Es\Is=\Kt=\Kxxt=0$.  The exact displacement of the beam is chosen to be
\begin{equation}
\eta_e(x,t) = \frac{a}{\pi f_t}\sin(f_x\pi x)\sin(f_t\pi t),
\label{eq:tzsolid}
\end{equation}
where $a=0.5$ is an amplitude and $f_x=f_t=2$ are frequencies.  The exact components of velocity and the pressure in the fluid are taken to be
\begin{equation}
\left.
\begin{array}{l}
\displaystyle{
u_e(x,y,t) = -a\cos(f_x\pi x)\sin(f_x\pi\tilde y)\cos(f_t\pi t)},\medskip\\
\displaystyle{
v_e(x,y,t) = a\sin(f_x\pi x)\cos(f_x\pi\tilde y)\cos(f_t\pi t)-a\pd{\eta_e}{x}\cos(f_x\pi x)\sin(f_x\pi\tilde y)\cos(f_t\pi t)},\medskip\\
\displaystyle{
p_e(x,y,t) = \cos(f_x\pi x)\cos(f_x\pi y)\cos(f_t\pi t)},
\end{array}
\right\}
\label{eq:tzfluid}
\end{equation}
where $\tilde y=y-(1+\eta_e)$.  \textcolor{red}{(Is a factor of $a$ missing in $p_e$ and is it $y$ or $\tilde y$ in $p_e$.)}
The components of velocity have been chosen so that the continuity equation is satisfied in the exact solution, and the vertical velocities of the fluid and the beam match along the interface at $y=\eta_e$.  Forcing functions are added to the equations for the fluid and structure so that the functions in~\eqref{eq:tzsolid} and~\eqref{eq:tzfluid} are exact solutions.


The stability of the AMP scheme for light beams is illustrated in figure~\ref{fig:lightBeamError} for the case $\rhos\hs=10^{-3}$.  The image on the left shows the TFI grid for the fluid domain at $t=0.1$.  The beam lies on the top surface of the domain, while the boundary conditions on the other three sides of the domain are taken to be Dirichlet conditions based on the exact solution for the fluid.  \textcolor{red}{(Is this true?})  The plot in the center of the figure shows the numerical solution for the vertical component of the fluid velocity, $v$, while the plot on the right shows the difference between the computed solution for $v$ and the exact solution given by $v_e$. \textcolor{red}{(We should include colorbars for the center and right plots.)} Here we observe that the error in $v$ is well behaved in that the magnitude is small and it is smooth throughout the domain including the boundaries.  The behavior of the error in the other components of the solution are similar.
 
%
%{\bf wdh: Longfei, can we compute the least squares convergence rate too for the tables?}
%
%
{% ------ TZ errors ------
\newcommand{\figWidth}{6cm}
\newcommand{\trimfig}[2]{\trimFig{#1}{#2}{.1}{0.02}{.4}{.4}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.0,.75) rectangle (18.,6.);  % set the bounding box (so we have less surrounding white space)
  \draw(-0.5,0.0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/TFIgrid}{\figWidth}};
    \draw(0.25,6.2) node[draw,fill=white,anchor=west,xshift=2pt,yshift=-16pt] {\scriptsize grid at $t=0.1$};
  \draw(5.,0.0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/v2Light}{\figWidth}};
      \draw(5.75,6.2) node[draw,fill=white,anchor=west,xshift=2pt,yshift=-16pt] {\scriptsize $v$ at $t=0.1$};
  \draw(10.5,0.0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/v2ErrLight}{\figWidth}};
       \draw(11.25,6.2) node[draw,fill=white,anchor=west,xshift=2pt,yshift=-16pt] {\scriptsize Error $v$ at $t=0.1$};

% grid:
%  \draw[step=1cm,gray] (0,0) grid (16,5);
\end{tikzpicture}
\end{center}
  \caption{Computational results for the manufactured solutions of a light beam ($\rhos\hs=10^{-3}$) using grid spacings $h=1/80$.
% . $f_x=f_t=2,~ a=0.5,~\bar{\rho}\bar{h}=1e-3,~\bar{T} = 1e-3,~\bar{K}=1$
}
  \label{fig:lightBeamError}
\end{figure}
}

%{% ------ TZ solutions ------
%\newcommand{\figWidth}{8cm}
%\newcommand{\trimfig}[2]{\trimFig{#1}{#2}{.02}{0.02}{.045}{.005}}
%\begin{figure}[htb]
%\begin{center}
%\begin{tikzpicture}[scale=1]
%  \useasboundingbox (0.0,.75) rectangle (16.,16.);  % set the bounding box (so we have less surrounding white space)
%   \draw(4.0,8.0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/pLight}{\figWidth}};
%  \draw(0.0,0.0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/v1Light}{\figWidth}};
%  \draw(8.0,0.0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/v2Light}{\figWidth}};
%% grid:
%%  \draw[step=1cm,gray] (0,0) grid (16,5);
%\end{tikzpicture}
%\end{center}
%  \caption{Computational solutions for the manufactured solutions of a light beam ($\rhos\hs=10^{-3}$) using grid spacings $h=1/80$. {\bf Longfei: I have added figures for all errors and solutions. We can decide which ones to be kept.}
%% . $f_x=f_t=2,~ a=0.1,~\bar{\rho}\bar{h}=1e-3,~\bar{T} = 1e-3,~\bar{K}=1$ 
%}
%  \label{fig:lightBeamContours}
%\end{figure}
%}
%

A convergence study is shown in  Table~\ref{tab:tableTZAmp} for light ($\rhos\hs=10^{-3}$), medium ($\rhos\hs=1$) and heavy ($\rhos\hs=10^{3}$) beams using grid spacings $\dx_j=\dy_j=h_j=1/(10j)$,
$j=1,2,\ldots$.  The maximum-norm errors, $E_j^{(q)}$ for solution component $q$ and for grid resolutions $j=1$, 2, 4 and 8, are computed for each value of $\rhos\hs$.  The convergence
rate is estimated by a least squares fit to the logarithm of the error over the grid resolutions. 
%, $\zeta_q$, is estimated by a least squares fit to the logarithm of the error equation, $E_j^{(q)} = C_q h_j^{\zeta_q}$, where
%$C_q$ is approximately constant for small grid spacings.  
%For vector variables, such as $\vv$ or $\usv$, the error denotes the maximum over all components of the vector.
The results in the table for the fluid velocity $(u,v)$ and pressure $p$, and for the beam displacement $\eta$ and velocity $\dot\eta$ show the expected second-order accuracy for all three choices of the beam mass, and in particular for the case of a light beam when added-mass effects are strong.

\tableTZAmp

%
%
%Figure~\ref{fig:lightBeamContours} shows shaded contours of the computed solution at $t=0.1$ for a light beam using
%manufactured solutions. The parameters were chosen as 
%$f_x=f_t=2$, $a=0.1$, $\bar{\rho}\bar{h}=10^{-3}$ , $\Ts =10^{-3}$, and $\Ks_0=1$. 
%Table~\ref{tab:tableTZAmp} gives the maximum-norm errors and estimated convergence rates for a light $\rhos=10^{-3}$, (CHECK ME)
%medium $\rhos=1$, and heavy $\rhos=10^3$ beam. 
%The AMP scheme is stable in all cases and
%the solutions are seen to converge at close to second-order accuracy. 

% Convergence results $f_x=f_t=2,~ a=0.1,~\bar{\rho}\bar{h}=1e-3,~\bar{T} = 1e-3,~\bar{K}=1$
%\tableTZAmp

% 
% % ---------------------------------------------------------------------------------------------------
% \subsection{Fluid chamber with a flexible top - parabolic beam steady solution}
% 
% An exact steady state solution can be determined for a rectangular fluid domain with a 
% flexible beam on the top when the fluid pressure on the bottom of the domain is a specified
% constant.
% 
% The geometry of the problem is ....
% 
% The grid is ...
% 
% 
% The steady state solution for ... is 
% \begin{align}
% u = 0,~ v=0,~ p = p_b,~ {\rm and }~\eta = -\frac{p_b}{2\bar{T}}x(x-1)
% \end{align}








==> texFiles/old.tex <==
\section{Old stuff -- keep here for now}


% 
% The EB beam is generally consider valid for thin beams and small slopes,  $|\uvs_x| \ll 1$.

QUESTION: DO WE RESTRICT THE DISCUSSION TO AN EB BEAM?

\input texFiles/beamCartoon

Let $\xbv(\ss,t)$ denote the position of the reference-line 
of the beam (sometimes this will be the centerline or {\em neutral-axis}) at time $t$
which is given by 
\begin{align*}
  \xbv(\ss,t)= \xbv(\ss,0) + \usv(s,t), 
\end{align*}
% where $\xsv(s)=\xbv(\ss,0)$ is the initial position of the reference-line and 
where $\usv(s,t)$ is the beam displacement.
Let $\xsv_+(\ss,t)$ and $\xsv_+(\ss,t)$ denote the points
on the upper and lower surfaces of the beam, respectively.
The geometry for EB beam is illustrated in Figure~\ref{fig:beamCartoon}. 
In this case, lines normal to the mid-line remain straight and 
we have  
\begin{align}
  \xsv_{\pm}(\ss,t)=\xbv(\ss,t)\pm \frac{\hs(\ss)}{2} \nsv(\ss,t), \label{eq:EBsurface}
\end{align}
where $\hs$ is the thickness of the beam and $\nsv(\ss,t)$ is the unit normal to the {\em reference-line} 
($\nsv$ is sometimes called the pseudo-normal or director~\cite{Belytschko2005}). 
% Note that in some circumstances we use the simplied approximation $\xsv_{\pm}(\ss,t)=\xbv(\ss,t)$, 
% which is a good approximation for very thin beams. 
The dynamic matching condition (balance of forces) 
defines the force on the beam in terms of the fluid forces on the upper and lower surfaces of the beam.
For our purposes here let us assume that this force can be written in the form 
\begin{align}
    \fsv(\ss,t)  &= - \Big[ (\sigmav\nv)_+(\ss,t)+ (\sigmav\nv)_-(\ss,t) \Big] + \deltafsv(\ss,t), \qquad \ss\in[0,\ls] , \label{eq:dynamic} 
%              &=  - \Big[ (\sigmav\nv)(\xsv_+(\ss,t),t) + (\sigmav\nv)(\xsv_-(\ss,t),t) \Big], \qquad \ss\in[0,\ls] , \\
%             &= - \Big[ (\sigmav\nv)_+(\ss,t)+ (\sigmav\nv)_-(\ss,t) \Big],   
\end{align} 
where
\begin{align}
    (\sigmav\nv)_\pm(\ss,t) &\equiv \sigmav(\xsv_\pm(\ss,t),t)\,\nv(\xsv_\pm(\ss,t),t), 
%     (\sigmav\nv)_-(\ss,t) &\equiv \sigmav(\xsv_+(\ss,t),t)\,\nv(\xsv_-(\ss,t),t), 
\end{align} 
and where $\deltafsv$ is assumed to be some small correction term.  
Here $\nv$ is the unit normal to the fluid-beam interface (outward pointing from the fluid domain). 
In general the force $\fsv(\ss,t)$ may depend on the fluid tractions in neighbourhoods of the points $\xsv_-(\ss,t)$ and $\xsv_+(\ss,t)$ but 
for the stability of the resulting AMP algorithm we will only need some reasonable approximation to the dependence of this
force on the fluid traction, which we suppose is the form of~\eqref{eq:dynamic}.
Other approximations could be used and these would alter the form and perhaps the stability of the AMP conditions but not the overall accuracy. 
% and the traction $\sigmav\nv$ is evaluated at the the point
% $\xv=\xv_\Gamma(s)$ on the interface.
% where we note that the normal $\nv$ differs on the upper and lower surfaces. 


The kinematic matching condition at the fluid-structure interface is that the velocity of the fluid at a point on the surface of
the beam matches the corresponding velocity of the beam surface,
\begin{align}
    \vv(\xsv_\pm(\ss,t),t) &= \frac{\partial}{\partial t}\xsv_{\pm}(\ss,t), \qquad\qquad \ss\in[0,\ls]  , \nonumber \\
                           &=\vsv(\ss,t) + \wsv_\pm(\ss,t),\label{eq:kinematicII}
\end{align} 
where $\wsv_\pm$, defined by~\eqref{eq:kinematicII}, is assumed to be an $O(\hs)$ correction to $\vsv(\ss,t)$. 
In the case of an EB beam we have 
 \begin{align}
    \vv(\xsv_\pm(\ss,t),t) &= \vsv(\ss,t) \pm \frac{\hs(\ss)}{2} \partialt \nsv(\ss,t),  \qquad \ss\in[0,\ls] ,   \label{eq:kinematicEB}
\end{align} 
and thus $\wsv_\pm(\ss,t) = \pm \frac{\hs(\ss)}{2} \partialt \nsv(\ss,t)$ for an EB beam. 
Note that the velocity of points on the beam surface will have primary contributions from the velocity of the beam reference-line
together with smaller ($O(\hs)$) contributions from the bending of the beam due to time variations in the beam normal $\nsv(\ss,t)$.
% as seen from~\eqref{eq:EBsurface} for an EB beam.
% where $\xsv=\xsv_\Gamma(\ss)$ denotes the coordinates of the interface. FIX ME FOR TWO SIDES 

MAYBE REMOVE THIS NEXT PARAGRAPH and refer to the subsection on  beams ??

In this paper the displacement of the beam is restricted to be in one direction relative to a flat undeformed state.
When the undeformed beam is parallel to the $x$-direction and the beam moves in the $y$-direction
we take $\Lvs=[\Ls_1,\Ls_2,\Ls_3]$ with $\Ls_1=\Ls_3=0$ and
\begin{alignat}{3}
    \Ls_2(\us_2,\vs_2) \equiv&        -\Ks_0 \us_2 +
                   \frac{\partial}{\partial \ss}\left( \Ts \frac{\partial \us_2}{\partial \ss}\right)
                   - \frac{\partial^2}{\partial \ss^2}\left( \Es\Is \frac{\partial^2 \us_2}{\partial \ss^2}\right) 
                  - \Ks_{t} \vs_2
                   + \Ks_{xxt} \frac{\partial^2 \vs_2}{\partial \ss^2}, \label{eq:EBbeamEquations}
\end{alignat}
where 
$\Es$ is Young's modulus, $\Is$ is the area-moment of inertial (e.g. $\Is=\frac{1}{12} \hs^3 \bs$ for a rectangular beam),
$\Ts$ is the {\em tension} coefficient and $\Ks_0$ is the linear stiffiness coefficient.
The factor involving $\Ks_t$ is a linear damping term while the factor with 
coefficient $\Ks_{xxt}$ is a {\em visco-elastic} damping term. 

% 
% \bigskip
% Old: 
% \begin{alignat}{3}
%     \Lvs(\uvs,\vvs) \equiv&        -K_0 \uvs +
%                    \frac{\partial}{\partial \ss}\left( T \frac{\partial \uvs}{\partial \ss}\right)
%                    - \frac{\partial^2}{\partial \ss^2}\left( E I \frac{\partial^2 \uvs}{\partial \ss^2}\right) 
%                   - K_{t} \vvs
%                    + K_{xxt} \frac{\partial^2 \vvs}{\partial \ss^2}, 
% \end{alignat}

% -----------------------------------
\subsection{EB Beam of constant thickness.}

**CHECK ME**

The AMP conditions simplify for a very thin EB beam of constant thickness.
In this case the normal vectors $\nv_+$ and $\nv_-$ are {\em nearly} parallel to centerline normal $\nsv$.
We can make the approximation $\nsv=\nv_-$ and then $\nv_+ = -\nsv$.
It follows that
\begin{align}
  \nv_\pm^T (\sigmav\nv)_+ = \pm p(\xsv_+(\ss,t),t), \\
  \nv_\pm^T (\sigmav\nv)_- = \mp p(\xsv_-(\ss,t),t). 
\end{align}
WE SHOULD JUST DROP THE LAST TERMin~\eqref{eq:AMP1a}.

The last term in~\eqref{eq:AMP1a} can be evaulated using
\begin{align*}
     \nsv^T\nsv = 1  ~\implies~ \partialt(\nsv^T\nsv)=0 ~\implies~ \nsv^T\partialt\nsv=0 , \\
  \implies   \partialt( \nsv^T\partialt\nsv ) =  \nsv^T\partialt^2\nsv + \partialt\nsv^T\partialt\nsv =0 , \\
  \implies \nsv^T\partialt^2\nsv = - \| \partialt\nsv \|^2, 
\end{align*}
and thus 
\begin{equation}
\rhos\hs \nv_\pm^T \partialt \wsv(\ss,t) = \rhos\frac{\hs^2}{2} \nv_\pm^T\partialt\nsv 
    = \mp  \rhos\frac{\hs^2}{2}  \nsv^T\partialt\nsv 
    = \pm \rhos\frac{\hs^2}{2} \| \partialt\nsv \|^2, 
\end{equation}
which represents a centripetal acceleration due to the rotation of the beam. 
Whence, INCLUDE VISCOUS STRESS HERE:
% ---------------------------------------------------------------------------------------------------------------
\begin{condition}
The AMP interface condition for the pressure for a very thin  EB beam of constant thickness is
% which, using $\nv_+=-\nv_-$ for an EB beam, leads to (multiplying both sides by minus 1)
% The normal component of~\eqref{eq:continuousversionI} defines a Robin condition on the pressure,
\begin{equation}
  \pm \Big[  p(\xsv_+(\ss,t),t) - p(\xsv_-(\ss,t),t) \Big] + 
\frac{\rhos\hs}{\rho}\frac{\partial}{\partial n_\pm} p(\xsv_\pm(\ss,t),t)  = -\nv_\pm ^T \Lsv\bigl(\uvs,\vsv\bigr) 
           - \rhos\frac{\hs^2}{2} \| \partialt\nsv \|^2  ,  \qquad \ss\in\Gammas.
    \label{eq:continuousversionIp}
\end{equation}
\end{condition}
% ---------------------------------------------------------------------------------------------------------------
% where we have used $\nsv_\pm^T\partial\nsv_\pm/\partial t=0$ (since $\nsv_\pm^T\nsv_\pm=1$) to eliminate the term involving $\wsv$. 
Note that 
equation~\eqref{eq:continuousversionIp} defines a mixed condition for the pressure at a point on the beam in terms
of the pressure on the opposite side of the beam and the beam operator $\Lsv$.


Taking the sum of the two equations in~\eqref{eq:continuousversionIp} for the upper and lower sides gives
%  and using $\nv_+=-\nv_-$  we find that
\begin{equation}
  \frac{\rhos\hs}{\rho}\frac{\partial}{\partial n_+} p(\xsv_+(\ss,t),t) 
+ \frac{\rhos\hs}{\rho}\frac{\partial}{\partial n_-} p(\xsv_-(\ss,t),t) = - \rhos\hs^2 \| \partialt\nsv \|^2, 
    \label{eq:pressureGradientCondition}
\end{equation}
% Thus, although the pressure can have a largejump across the beam, the normal derivative of the pressure, 
Therefore, when adjusted for the sign of the normals, the jump is the normal derivative of the pressure across the beam
is generally small for thin beams, being of order $O(\rhos\hs^2)$.
Condition~\eqref{eq:pressureGradientConditionII} could be used to in place of one of the equations in~\eqref{eq:continuousversionIp}.
This  might have some numerical advantages when $\rhos\hs/\rho$ becomes very small since the two 
equations in~\eqref{eq:continuousversionIp} become nearly linearly dependent in this limit.
% Conditions~\eqref{eq:pressureGradientConditionII}-\eqref{eq:pressureJump} are alternative forms of the interface conditions. 

\clearpage
\bigskip CHECK ME: 
The AMP condition~\eqref{eq:continuousversionIp} is somewhat awkward to implement as it is a nonlocal condition on $p$ (involving
$p$ on opposite sides of the beam)
and it would be convenient to have a local condition that had the same stability and accuracy properties.
To this end we propose the alternative local AMP condition, derived from~\eqref{eq:AMPconditionSigma} by adding
$\sigmav(\xsv_\pm(\ss,t),t)\nv$ to both sides, 
\begin{equation}
 \sigmav(\xsv_\pm(\ss,t),t)\nv +  \frac{\rhos\hs}{\rho}\grad\cdot\sigmav(\xsv_\pm(\ss,t),t)  = \Lsv\bigl(\uvs,\vsv\bigr) \mp \rhos\hs \partialt \wsv(\ss,t)  + \fsv + \sigmav(\xsv_\pm(\ss,t),t)\nv    \qquad \ss\in\Gammas.
    \label{eq:AMPconditionSigmaII}
\end{equation}
We have removed the primary dependence of $\fsv$ on $\sigmav(\xsv_\pm(\ss,t),t)\nv$ by taking 
$\fsv + \sigmav(\xsv_\pm(\ss,t),t)\nv$.
Given accurate {\em predicted} values $\fsv^{p}$ and  $\sigmav^{p}(\xsv_\pm(\ss,t),t)\nv$ we define the AMP condition
to be
 \begin{equation}
 \sigmav(\xsv_\pm(\ss,t),t)\nv +  \frac{\rhos\hs}{\rho}\grad\cdot\sigmav(\xsv_\pm(\ss,t),t)  = \Lsv\bigl(\uvs,\vsv\bigr) \mp \rhos\hs \partialt \wsv(\ss,t)  + \fsv^{p} + \sigmav^{p}(\xsv_\pm(\ss,t),t)\nv    \qquad \ss\in\Gammas,
    \label{eq:AMPconditionSigmaIII}
\end{equation}
where we have used the predicted traction on the right-hand-side of~\eqref{eq:AMPconditionSigmaIII}. 
The normal component of~\eqref{eq:AMPconditionSigmaIII} is the local Robin condition
\begin{equation}
   p(\xsv_{\pm}(\ss,t),t) + 
\frac{\rhos\hs}{\rho}\frac{\partial}{\partial n} p(\xsv_\pm(\ss,t),t)  =
         - \nv^T \Lsv\bigl(\uvs,\vsv\bigr) +  \nv^T\fsv^{p} + p^{p}(\xsv_{\pm}(\ss,t),t) \qquad \ss\in\Gammas,
    \label{eq:continuousversionII}
\end{equation}
where $p^{p}(\xsv_{\pm}(\ss,t),t)$ is an accurate {\em predicted} value for the pressure on the beam surface. 
It remains to show that~\eqref{eq:continuousversionII} defines a stable scheme for light beams. THIS MAY REQUIRE
SOME ITERATION or ACCELERATION TECHNIQUE.


\clearpage
% ================================================================
The dynamic matching condition (balance of forces) 
defines the force on the beam in terms of the fluid forces on the upper and lower surfaces of the beam.
For our purposes here let us assume that this force can be written in the form 
\begin{align}
    \fsv(\ss,t)  &= - \Big[ (\sigmav\nv)_+(\ss,t)+ (\sigmav\nv)_-(\ss,t) \Big] + \deltafsv(\ss,t), \qquad \ss\in[0,\ls] , \label{eq:dynamic} 
%              &=  - \Big[ (\sigmav\nv)(\xsv_+(\ss,t),t) + (\sigmav\nv)(\xsv_-(\ss,t),t) \Big], \qquad \ss\in[0,\ls] , \\
%             &= - \Big[ (\sigmav\nv)_+(\ss,t)+ (\sigmav\nv)_-(\ss,t) \Big],   
\end{align} 
where
\begin{align}
    (\sigmav\nv)_\pm(\ss,t) &\equiv \sigmav(\xsv_\pm(\ss,t),t)\,\nv(\xsv_\pm(\ss,t),t), 
%     (\sigmav\nv)_-(\ss,t) &\equiv \sigmav(\xsv_+(\ss,t),t)\,\nv(\xsv_-(\ss,t),t), 
\end{align} 
and where $\deltafsv$ is assumed to be some small correction term.  
Here $\nv$ is the unit normal to the fluid-beam interface (outward pointing from the fluid domain). 
In general the force $\fsv(\ss,t)$ may depend on the fluid tractions in neighbourhoods of the points $\xsv_-(\ss,t)$ and $\xsv_+(\ss,t)$ but 
for the stability of the resulting AMP algorithm we will only need some reasonable approximation to the dependence of this
force on the fluid traction, which we suppose is the form of~\eqref{eq:dynamic}.
Other approximations could be used and these would alter the form and perhaps the stability of the AMP conditions but not the overall accuracy. 
% and the traction $\sigmav\nv$ is evaluated at the the point
% $\xv=\xv_\Gamma(s)$ on the interface.
% where we note that the normal $\nv$ differs on the upper and lower surfaces. 


The kinematic matching condition at the fluid-structure interface is that the velocity of the fluid at a point on the surface of
the beam matches the corresponding velocity of the beam surface,
\begin{align}
    \vv(\xsv_\pm(\ss,t),t) &= \frac{\partial}{\partial t}\xsv_{\pm}(\ss,t), \qquad\qquad \ss\in[0,\ls]  , \nonumber \\
                           &=\vsv(\ss,t) + \wsv_\pm(\ss,t),\label{eq:kinematicII}
\end{align} 
where $\wsv_\pm$, defined by~\eqref{eq:kinematicII}, is assumed to be an $O(\hs)$ correction to $\vsv(\ss,t)$. 
In the case of an EB beam we have 
 \begin{align}
    \vv(\xsv_\pm(\ss,t),t) &= \vsv(\ss,t) \pm \frac{\hs(\ss)}{2} \partialt \nsv(\ss,t),  \qquad \ss\in[0,\ls] ,   \label{eq:kinematicEB}
\end{align} 
and thus $\wsv_\pm(\ss,t) = \pm \frac{\hs(\ss)}{2} \partialt \nsv(\ss,t)$ for an EB beam. 
Note that the velocity of points on the beam surface will have primary contributions from the velocity of the beam reference-line
together with smaller ($O(\hs)$) contributions from the bending of the beam due to time variations 
in the beam normal $\nsv(\ss,t)$.


\section{Beams}

MAYBE just forward reference in ``governing'' and put beam equations here?

% The beam equations~\eqref{eq:EBbeamEquations} 
A generalized Euler-Bernoulli beam model is
\begin{align}
  \rhos \As \frac{\partial^2\ww}{\partial t^2} = 
                    & -\Ks_0\ww +
                   \frac{\partial}{\partial x}\left( \Ts \frac{\partial\ww}{\partial x}\right)
                   - \frac{\partial^2}{\partial x^2}\left( \Es \Is \frac{\partial^2\ww}{\partial x^2}\right) \nonumber \\
              &    - \Ks_{t} \wt
                   + \Ks_{xxt} \frac{\partial^2 \wt}{\partial x^2}
                   + f(x,t), 
                  \qquad\qquad x\in[0,\Ls], \quad t\ge 0,  \label{eq:BeamModelOld}
\end{align}
where $y=w(x,t)$ is the displacement of the beam, $\wt=\partial\ww/\partial t$ is the beam velocity,  
$\As$ is the cross-sectional area of the beam ($\As=\hs\bs$ for a beam of constant thickness, $\hs$ and constant breadth $\bs$ in the z-direction), 
$\rhos$ is the beam density, $\Ls$ is the length of the beam, 
$\Es$ is Young's modulus, $\Is$ is the area-moment of inertial (e.g. $\Is=\frac{1}{12} h^3 b$ for a rectangular beam),
 $\Ts$ is the {\em tension} coefficient and $\Ks_0$ is the linear stiffiness coefficient.
The term with coefficient $\Ks_{xxt}$ is a {\em visco-elastic} damping term. 
% 
The force $f(x,t)$ on the beam centerline is determined from the fluid tractions $\sigmav\nv$ on the beam
surface.


%--------------------
\vskip3\baselineskip



{\bf AMP-ADJ:}
Multiplying~\eqref{eq:discreteBeam} by $M^{-1}$ gives the spatially discrete beam equation, 
\begin{align}
   \rhos\As \ddot\wvh &= - M^{-1}K \wvh - M^{-1} B \dot\wvh + M^{-1}\fvh,   \\ \label{eq:discreteBeamII}
                     &= \Lsv^h(\wvh,\dot\wvh) + \Fv^h , 
\end{align}
where $\Fv^h\equiv M^{-1}\fvh$. 
Equation~\eqref{eq:discreteBeamII} can be used to compute the discrete forms of the beam operator $\Lsv(\usv,\vsv)$ and
forcing, $\fsv$ that appear in the AMP scheme.
% 
In particular, entries in the term $\Fv^h$ are linear functions of the pressure and viscous stress $\tauv\nv$ on the beam surfaces, 
\begin{align}
   \Fv^h = A_p \pv^h + A_\tau \tauv^h
\end{align}
where $\pv^h$ and $\tauv^h$ are vectors of the pressures and viscous tractions on the beam surface, 
and $A_p$ and $A_\tau$ are matrices (non square in general since the number of fluid grid points on the beam surface will
be different from the number of beam nodes). 

The spatially discrete form of the AMP condition~\eqref{eq:AMPconditionSigma}: 
\begin{equation}
  \frac{\rhos\hs}{\rho}\grad\cdot\sigmav(\xsv_\pm(\ss,t),t)  = \Lsv\bigl(\uvs,\vv\bigr) + \rhos\hs \partialt \wsv_\pm(\ss,t)  + \fsv(\ss,t)
          \qquad \ss\in\Gammas.
    \label{eq:AMPconditionSigmaII}
\end{equation}
 will thus be of the form (this is not really true as we need to transfer the beam unknowns onto the fluid grid). 
\begin{equation}
  \frac{\rhos\hs}{\rho}\grad_h\cdot\sigmav^h_\pm  = 
     \Lsv^h\bigl(\uvs^h,\vsv^h\bigr) + \rhos\hs \partialt \wsv_\pm^h  + A_p \pv^h + A_\tau \tauv^h
    \label{eq:AMPconditionSigmaDiscrete}
\end{equation}
or
\begin{equation}
  -A_p \pv^h  + \frac{\rhos\hs}{\rho}\grad_h\pv^h_\pm    = 
     \Lsv^h\bigl(\uvs^h,\vsv^h\bigr) + \rhos\hs \partialt \wsv_\pm^h +  A_\tau \tauv^h -\frac{\rhos\hs}{\rho}\grad_h\cdot\tauv^h_\pm
    \label{eq:AMPconditionSigmaDiscreteII}
\end{equation}
% or
% \begin{equation}
%   -A_p \pv^h -  A_\tau \tauv^h + \frac{\rhos\hs}{\rho}\grad_h\cdot\sigmav^h_\pm  = 
%      \Lsv^h\bigl(\uvs^h,\vsv^h\bigr) + \rhos\hs \partialt \wsv_\pm^h 
%     \label{eq:AMPconditionSigmaDiscreteIII}
% \end{equation}
The discrete AMP condition~~\eqref{eq:AMPconditionSigmaDiscreteII} thus defines a generalized Robin
condition that involves the pressure and velocity on the interface. 
The {\em normal component} of these condition will define a discrete Robin condition for the
pressure of the form
\begin{equation}
  B_p \pv^h  + \frac{\rhos\hs}{\rho}(\nv_h\cdot\grad_h)\pv^h_\pm    = \gv^h  \label{eq:AMPdiscrete}
\end{equation}
For a beam with fluid on two sides one might expect that 
\begin{align}
   B_p \pv^h  \approx \pv_- - \pv_+ . \label{eq:AMPapproximation}
\end{align}
From the derivation given above, it can be seen, however, that the actual dependence will be more complicated due
to the fluid-solid transfer operators, the effect of the mass matrix and the implicit dependence on the
beam boundary conditions. 
As a means to simplify the implementation we rewrite~\eqref{eq:AMPdiscrete} in the form
\begin{equation}
 \pv_- - \pv_+ + \frac{\rhos\hs}{\rho}(\nv_h\cdot\grad_h)\pv^h_\pm    = \gv^h + \Big[\pv_- - \pv_+  -B_p \pv^h  \Big] 
                 \label{eq:AMPdiscreteII}
\end{equation}
where we have added $\pv_- - \pv_+$ to both sides and moved $B_p \pv^h$ to the right-hand side.

\paragraph{Force and velocity transfers} Forces and velocities need to be transfered between the fluid grid
and the beam FEM representation. 


The FEM representation for the beam as Hermite polynomials can be used to compute 
values of the displacement and velocity at any point on the beam surface. FINISH ME.

\bigskip
BEAM VERIFICATION -- should be add convergence tables for the beam solver?

% 
% \vskip3\baselineskip
% and the form of this dependence will provide the form of the pressure term in the Robin AMP condition. 
% For example, for a beam with fluid on two sides one might expect that 
% \begin{align}
%    (M^{-1}\fvh)_i^{\phi} \approx p(\xv_-(s_i),t) - p(\xv_+(s_i),t). \label{eq:beamForce}
% \end{align}
% From ~\eqref{eq:discreteBeamII} it can be seen that the actual dependence will be more complicated due
% to the fluid-solid transfer operators, the effect of the mass matrix and the implicit dependence on the
% beam boundary conditions. 
% 
% NOTE that~\eqref{eq:discreteBeamII} incorporates the boundary conditions of the beam. 
% Thus the beam force approximation~\eqref{eq:dynamic} may not be very good near clamped/pinned beam boundaries. 
% For example,  for a clamped beam, with $\ww(a,t)=0$, the acceleration of the
% beam will be zero on the end and this condition will be incoporated into the equations~\eqref{eq:discreteBeam}. 
% 
% Conceptually, the local added mass effect near a clamped/pinned boundary is generally 
% smaller than in the middle of the beam since the beam is restricted in motion and thus restricted in
% the amount of fluid that is put in motion when the beam accelerates (IS THIS ARGUMENT VALID?). 

